Sparse grids vs. random points for high-dimensional polynomial approximation

We study polynomial approximation on a $d$-cube, where $d$ is large, and compare interpolation on sparse grids, aka Smolyak's algorithm (SA), with a simple least squares method based on randomly generated points (LS) using standard benchmark functions. Our main motivation is the influential paper [Barthelmann, Novak, Ritter: High dimensional polynomial interpolation on sparse grids, Adv. Comput. Math. 12, 2000]. We repeat and extend their theoretical analysis and numerical experiments for SA and compare to LS in dimensions up to 100. Our extensive experiments demonstrate that LS, even with only slight oversampling, consistently matches the accuracy of SA in low dimensions. In high dimensions, however, LS shows clear superiority.

==> tables/CONTINUOUS.tex <==
% Created with Python on 2025-06-22 19:31:18
% ..\results\final_results\low_dim\results_numerical_experiments.csv, function = CONTINUOUS, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\textbf{Dim 2}\\$Q=50$}} & Smolyak & \first{4.40e-02} & \first{1.49e-02}  & 2.22e-02 & 5.15e-03  & 1.10e-02 & 1.58e-03  & 5.23e-03 & 6.18e-04  & 2.68e-03 & 2.17e-04  & 1.46e-03 & 8.93e-05  & 7.65e-04 & 2.95e-05\\
 & LS-Uniform & 2.66e-01 & 7.08e-02  & 5.19e-01 & 7.51e-02  & 3.64e-01 & 3.24e-02  & 6.88e-01 & 6.27e-02  & 5.86e+02 & 2.69e+01  & 7.77e+02 & 3.19e+01  & 8.46e+08 & 1.50e+07\\
 & LS-Chebyshev & 4.80e-02 & 2.21e-02  & \first{1.84e-02} & \first{4.06e-03}  & \first{9.43e-03} & \first{1.45e-03}  & \first{4.69e-03} & \first{4.91e-04}  & \first{2.08e-03} & \first{1.85e-04}  & \first{1.20e-03} & \first{6.72e-05}  & \first{6.47e-04} & \first{2.71e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 3}\\$Q=50$}} & Smolyak & 4.54e-02 & 1.16e-02  & \first{1.57e-02} & \first{3.66e-03}  & 1.17e-02 & 1.68e-03  & \first{4.17e-03} & \first{4.94e-04}  & 3.22e-03 & 1.92e-04  & 1.32e-03 & 6.54e-05  & 6.66e-04 & 2.43e-05\\
 & LS-Uniform & 9.00e-02 & 1.51e-02  & 2.57e-02 & 4.94e-03  & 3.90e-02 & 2.89e-03  & 5.98e-02 & 2.11e-03  & 5.33e-02 & 1.49e-03  & 2.74e-01 & 4.00e-03  & 3.04e+01 & 3.14e-01\\
 & LS-Chebyshev & \first{3.30e-02} & \first{9.08e-03}  & 1.90e-02 & 4.16e-03  & \first{7.98e-03} & \first{1.43e-03}  & 5.42e-03 & 5.28e-04  & \first{2.11e-03} & \first{1.81e-04}  & \first{1.04e-03} & \first{6.09e-05}  & \first{5.69e-04} & \first{2.19e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 4}\\$Q=50$}} & Smolyak & 3.06e-02 & \first{7.22e-03}  & 1.51e-02 & 3.07e-03  & 9.36e-03 & 1.03e-03  & 4.98e-03 & 4.84e-04  & 2.80e-03 & 1.64e-04  & 1.13e-03 & 5.73e-05  & 6.76e-04 & 1.81e-05\\
 & LS-Uniform & 6.82e-02 & 8.94e-03  & 3.20e-02 & 3.45e-03  & 1.81e-02 & 1.67e-03  & 1.81e-02 & 7.44e-04  & 1.05e-02 & 3.41e-04  & 2.03e-02 & 2.56e-04  & 2.02e-01 & 1.17e-03\\
 & LS-Chebyshev & \first{2.80e-02} & 7.87e-03  & \first{1.33e-02} & \first{2.72e-03}  & \first{7.72e-03} & \first{9.94e-04}  & \first{3.78e-03} & \first{3.61e-04}  & \first{2.23e-03} & \first{1.29e-04}  & \first{8.58e-04} & \first{4.69e-05}  & \first{4.37e-04} & \first{1.74e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 5}\\$Q=50$}} & Smolyak & 3.24e-02 & \first{6.00e-03}  & 1.60e-02 & 2.55e-03  & 8.41e-03 & 8.77e-04  & 3.68e-03 & 3.27e-04  & 2.18e-03 & 1.31e-04  & 8.40e-04 & 4.66e-05  &  & \\
 & LS-Uniform & 3.47e-02 & 7.08e-03  & 2.26e-02 & 3.14e-03  & 1.63e-02 & 1.17e-03  & 1.36e-02 & 4.58e-04  & 6.62e-03 & 2.06e-04  & 7.40e-03 & 1.04e-04  &  & \\
 & LS-Chebyshev & \first{2.80e-02} & 6.25e-03  & \first{1.45e-02} & \first{2.23e-03}  & \first{6.89e-03} & \first{7.64e-04}  & \first{3.13e-03} & \first{2.85e-04}  & \first{1.42e-03} & \first{1.02e-04}  & \first{7.27e-04} & \first{3.74e-05}  &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 6}\\$Q=50$}} & Smolyak & \first{2.46e-02} & \first{5.14e-03}  & \first{1.37e-02} & \first{1.90e-03}  & 7.75e-03 & 7.71e-04  & \first{3.31e-03} & 3.30e-04  & 1.78e-03 & 1.10e-04  &  &   &  & \\
 & LS-Uniform & 3.23e-02 & 5.40e-03  & 1.68e-02 & 2.30e-03  & 1.09e-02 & 9.02e-04  & 1.16e-02 & 3.73e-04  & 5.36e-03 & 1.60e-04  &  &   &  & \\
 & LS-Chebyshev & 2.47e-02 & 5.55e-03  & 1.38e-02 & 2.15e-03  & \first{6.24e-03} & \first{7.46e-04}  & 3.75e-03 & \first{2.59e-04}  & \first{1.58e-03} & \first{9.33e-05}  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 7}\\$Q=50$}} & Smolyak & 3.05e-02 & 6.08e-03  & 1.22e-02 & 1.95e-03  & 7.33e-03 & 7.47e-04  & 4.32e-03 & 2.83e-04  & 1.78e-03 & 1.08e-04  &  &   &  & \\
 & LS-Uniform & 3.32e-02 & \first{5.12e-03}  & 1.91e-02 & 1.94e-03  & 1.35e-02 & 8.28e-04  & 1.17e-02 & 3.24e-04  & 6.02e-03 & 1.35e-04  &  &   &  & \\
 & LS-Chebyshev & \first{2.13e-02} & 5.31e-03  & \first{1.13e-02} & \first{1.78e-03}  & \first{5.84e-03} & \first{6.34e-04}  & \first{2.99e-03} & \first{2.35e-04}  & \first{1.74e-03} & \first{8.47e-05}  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 8}\\$Q=50$}} & Smolyak & 2.35e-02 & 4.67e-03  & \first{1.13e-02} & 1.89e-03  & 6.45e-03 & 6.21e-04  & 3.25e-03 & 2.40e-04  &  &   &  &   &  & \\
 & LS-Uniform & 2.41e-02 & \first{4.44e-03}  & 1.40e-02 & 1.80e-03  & 9.09e-03 & 7.09e-04  & 5.86e-03 & 2.80e-04  &  &   &  &   &  & \\
 & LS-Chebyshev & \first{2.22e-02} & 4.75e-03  & 1.26e-02 & \first{1.65e-03}  & \first{5.08e-03} & \first{6.01e-04}  & \first{2.85e-03} & \first{2.17e-04}  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 9}\\$Q=50$}} & Smolyak & \first{2.08e-02} & \first{4.22e-03}  & 1.26e-02 & \first{1.74e-03}  & \first{4.71e-03} & 7.08e-04  & 3.44e-03 & 2.55e-04  &  &   &  &   &  & \\
 & LS-Uniform & 2.26e-02 & 4.27e-03  & 1.56e-02 & 1.86e-03  & 1.33e-02 & 7.18e-04  & 9.70e-03 & 2.93e-04  &  &   &  &   &  & \\
 & LS-Chebyshev & 2.09e-02 & 4.60e-03  & \first{9.93e-03} & 1.86e-03  & 5.37e-03 & \first{6.31e-04}  & \first{2.60e-03} & \first{2.33e-04}  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 10}\\$Q=50$}} & Smolyak & 2.33e-02 & 4.16e-03  & \first{9.30e-03} & 1.55e-03  & \first{5.37e-03} & 6.20e-04  & 2.79e-03 & \first{1.92e-04}  &  &   &  &   &  & \\
 & LS-Uniform & 2.36e-02 & \first{3.73e-03}  & 1.20e-02 & 1.48e-03  & 1.07e-02 & 6.01e-04  & 6.48e-03 & 2.37e-04  &  &   &  &   &  & \\
 & LS-Chebyshev & \first{2.23e-02} & 4.08e-03  & 1.03e-02 & \first{1.45e-03}  & 5.61e-03 & \first{5.39e-04}  & \first{2.34e-03} & 1.95e-04  &  &   &  &   &  & \\
\bottomrule
\end{tabular}


==> tables/CORNER_PEAK.tex <==
% Created with Python on 2025-06-22 19:31:18
% ..\results\final_results\low_dim\results_numerical_experiments.csv, function = CORNER_PEAK, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\textbf{Dim 2}\\$Q=50$}} & Smolyak & \first{8.78e-03} & 4.52e-03  & 1.48e-03 & 5.81e-04  & 1.04e-04 & 3.31e-05  & 8.90e-07 & 2.61e-07  & \first{6.08e-09} & 1.75e-09  & \first{2.77e-13} & 8.54e-14  & \first{6.99e-15} & \first{9.35e-16}\\
 & LS-Uniform & 1.54e-02 & 3.24e-03  & 3.50e-03 & 5.50e-04  & 4.92e-04 & 5.98e-05  & 2.30e-04 & 2.04e-05  & 6.80e-04 & 3.05e-05  & 7.93e-08 & 2.70e-09  & 1.66e-02 & 2.92e-04\\
 & LS-Chebyshev & 8.88e-03 & \first{3.12e-03}  & \first{1.42e-03} & \first{4.44e-04}  & \first{8.77e-05} & \first{2.65e-05}  & \first{6.13e-07} & \first{1.70e-07}  & 6.32e-09 & \first{1.30e-09}  & 2.79e-13 & \first{5.98e-14}  & 1.39e-14 & 1.17e-15\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 3}\\$Q=50$}} & Smolyak & 5.78e-02 & 1.58e-02  & 3.03e-02 & 5.80e-03  & 7.48e-03 & 1.46e-03  & 1.44e-03 & 2.55e-04  & 1.98e-04 & 2.96e-05  & 1.35e-05 & 2.06e-06  & 3.16e-07 & 4.17e-08\\
 & LS-Uniform & 7.11e-02 & \first{1.33e-02}  & \first{8.54e-03} & \first{1.65e-03}  & 6.77e-03 & \first{3.90e-04}  & 2.03e-03 & 1.02e-04  & 1.40e-03 & 3.23e-05  & 6.45e-04 & 1.13e-05  & 5.31e-03 & 5.72e-05\\
 & LS-Chebyshev & \first{3.38e-02} & 1.34e-02  & 9.19e-03 & 2.33e-03  & \first{2.31e-03} & 4.72e-04  & \first{3.68e-04} & \first{8.59e-05}  & \first{6.43e-05} & \first{1.07e-05}  & \first{5.24e-06} & \first{9.96e-07}  & \first{1.16e-07} & \first{2.05e-08}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 4}\\$Q=50$}} & Smolyak & 1.62e-01 & 2.46e-02  & 8.14e-02 & 1.29e-02  & 5.39e-02 & 5.69e-03  & 1.89e-02 & 2.32e-03  & 6.42e-03 & 6.42e-04  & 1.60e-03 & 1.37e-04  & 3.10e-04 & 2.20e-05\\
 & LS-Uniform & \first{9.45e-02} & \first{1.05e-02}  & 6.71e-02 & \first{4.08e-03}  & 2.02e-02 & \first{1.08e-03}  & 8.63e-03 & \first{2.20e-04}  & 6.64e-03 & \first{8.51e-05}  & 1.53e-03 & \first{2.20e-05}  & 3.41e-03 & 2.36e-05\\
 & LS-Chebyshev & 1.14e-01 & 2.12e-02  & \first{4.08e-02} & 7.06e-03  & \first{1.23e-02} & 2.09e-03  & \first{2.51e-03} & 4.46e-04  & \first{7.63e-04} & 1.16e-04  & \first{1.81e-04} & 2.37e-05  & \first{3.76e-05} & \first{4.59e-06}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 5}\\$Q=50$}} & Smolyak & 1.56e-01 & 2.07e-02  & 2.47e-01 & 1.57e-02  & 1.25e-01 & 1.07e-02  & 7.94e-02 & 5.60e-03  & 3.98e-02 & 2.24e-03  & 1.65e-02 & 1.01e-03  &  & \\
 & LS-Uniform & \first{4.36e-02} & \first{5.32e-03}  & 1.21e-01 & \first{4.43e-03}  & 6.88e-02 & \first{1.49e-03}  & 1.91e-02 & \first{4.54e-04}  & 1.51e-02 & \first{1.62e-04}  & 1.39e-02 & \first{6.86e-05}  &  & \\
 & LS-Chebyshev & 1.51e-01 & 3.78e-02  & \first{5.15e-02} & 1.30e-02  & \first{2.44e-02} & 4.49e-03  & \first{8.78e-03} & 1.20e-03  & \first{2.72e-03} & 3.57e-04  & \first{1.25e-03} & 1.15e-04  &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 6}\\$Q=50$}} & Smolyak & 2.46e-02 & 2.99e-03  & 1.80e-01 & 8.18e-03  & 2.53e-01 & 8.59e-03  & 1.44e-01 & 5.65e-03  & 1.07e-01 & 4.41e-03  &  &   &  & \\
 & LS-Uniform & \first{2.41e-02} & \first{2.87e-03}  & 1.03e-01 & \first{2.87e-03}  & 7.82e-02 & \first{1.19e-03}  & 7.77e-02 & \first{6.63e-04}  & 2.75e-02 & \first{1.54e-04}  &  &   &  & \\
 & LS-Chebyshev & 7.62e-02 & 2.10e-02  & \first{6.89e-02} & 9.41e-03  & \first{2.50e-02} & 4.35e-03  & \first{1.75e-02} & 2.11e-03  & \first{8.05e-03} & 7.55e-04  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 7}\\$Q=50$}} & Smolyak & 1.68e-02 & 1.40e-03  & 3.63e-02 & 2.11e-03  & 1.06e-01 & 3.14e-03  & 1.36e-01 & 3.50e-03  & 1.45e-01 & 3.08e-03  &  &   &  & \\
 & LS-Uniform & \first{1.49e-02} & \first{7.53e-04}  & \first{2.17e-02} & \first{4.91e-04}  & 3.75e-02 & \first{4.28e-04}  & 6.35e-02 & \first{4.00e-04}  & 4.31e-02 & \first{1.72e-04}  &  &   &  & \\
 & LS-Chebyshev & 3.82e-02 & 1.26e-02  & 2.98e-02 & 4.26e-03  & \first{2.76e-02} & 3.68e-03  & \first{1.62e-02} & 1.41e-03  & \first{9.84e-03} & 6.83e-04  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 8}\\$Q=50$}} & Smolyak & 1.40e-03 & \first{6.37e-05}  & 7.79e-03 & 5.32e-04  & 4.59e-02 & 9.43e-04  & 4.68e-02 & 1.34e-03  &  &   &  &   &  & \\
 & LS-Uniform & \first{1.29e-03} & 8.69e-05  & \first{1.43e-03} & \first{9.33e-05}  & \first{9.09e-03} & \first{7.55e-05}  & \first{7.43e-03} & \first{7.63e-05}  &  &   &  &   &  & \\
 & LS-Chebyshev & 1.52e-02 & 3.77e-03  & 2.64e-02 & 3.62e-03  & 2.40e-02 & 2.21e-03  & 1.56e-02 & 9.77e-04  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 9}\\$Q=50$}} & Smolyak & \first{1.30e-03} & \first{4.80e-05}  & 1.49e-02 & 4.24e-04  & 3.07e-02 & 6.85e-04  & 4.38e-02 & 8.63e-04  &  &   &  &   &  & \\
 & LS-Uniform & 1.46e-03 & 5.45e-05  & \first{6.29e-03} & \first{8.21e-05}  & \first{5.84e-03} & \first{3.80e-05}  & 2.55e-02 & \first{8.50e-05}  &  &   &  &   &  & \\
 & LS-Chebyshev & 3.56e-02 & 8.37e-03  & 2.21e-02 & 3.34e-03  & 1.46e-02 & 1.54e-03  & \first{1.97e-02} & 1.03e-03  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 10}\\$Q=50$}} & Smolyak & 4.08e-04 & \first{1.11e-05}  & 5.66e-04 & \first{1.08e-05}  & 1.16e-02 & 1.67e-04  & 2.88e-02 & 4.11e-04  &  &   &  &   &  & \\
 & LS-Uniform & \first{3.87e-04} & 2.09e-05  & \first{5.40e-04} & 1.26e-05  & \first{9.89e-04} & \first{9.84e-06}  & \first{2.38e-03} & \first{8.90e-06}  &  &   &  &   &  & \\
 & LS-Chebyshev & 1.62e-03 & 2.92e-04  & 1.33e-03 & 2.53e-04  & 4.98e-03 & 3.72e-04  & 6.19e-03 & 3.31e-04  &  &   &  &   &  & \\
\bottomrule
\end{tabular}


==> tables/DISCONTINUOUS.tex <==
% Created with Python on 2025-06-22 19:31:18
% ..\results\final_results\low_dim\results_numerical_experiments.csv, function = DISCONTINUOUS, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\textbf{Dim 2}\\$Q=50$}} & Smolyak & 4.73e+00 & \first{1.26e+00}  & 3.82e+00 & 1.08e+00  & 4.82e+00 & 8.42e-01  & 4.56e+00 & 6.75e-01  & 4.07e+00 & 4.26e-01  & 3.57e+00 & 3.28e-01  & 4.70e+00 & 2.16e-01\\
 & LS-Uniform & 3.46e+01 & 8.99e+00  & 7.48e+01 & 1.09e+01  & 6.02e+01 & 6.33e+00  & 3.07e+02 & 2.72e+01  & 6.62e+05 & 2.77e+04  & 1.79e+06 & 6.20e+04  & 6.27e+12 & 1.10e+11\\
 & LS-Chebyshev & \first{3.47e+00} & 1.27e+00  & \first{3.59e+00} & \first{7.15e-01}  & \first{4.24e+00} & \first{6.58e-01}  & \first{3.44e+00} & \first{4.35e-01}  & \first{3.25e+00} & \first{2.92e-01}  & \first{2.36e+00} & \first{2.04e-01}  & \first{2.92e+00} & \first{1.46e-01}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 3}\\$Q=50$}} & Smolyak & 7.08e+00 & \first{1.73e+00}  & 1.11e+01 & \first{1.33e+00}  & 7.35e+00 & \first{1.03e+00}  & 9.26e+00 & 8.10e-01  & 9.99e+00 & 5.76e-01  & 8.40e+00 & 4.81e-01  & 1.07e+01 & 3.28e-01\\
 & LS-Uniform & 1.70e+01 & 3.87e+00  & 1.11e+01 & 1.66e+00  & 2.38e+01 & 1.67e+00  & 6.09e+01 & 2.57e+00  & 2.28e+02 & 5.88e+00  & 1.29e+03 & 2.70e+01  & 4.47e+05 & 4.45e+03\\
 & LS-Chebyshev & \first{6.97e+00} & 1.75e+00  & \first{6.09e+00} & 1.37e+00  & \first{5.86e+00} & 1.04e+00  & \first{7.10e+00} & \first{7.63e-01}  & \first{9.30e+00} & \first{5.30e-01}  & \first{6.44e+00} & \first{3.77e-01}  & \first{6.29e+00} & \first{2.59e-01}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 4}\\$Q=50$}} & Smolyak & 2.40e+01 & \first{3.96e+00}  & 3.61e+01 & 3.29e+00  & 3.36e+01 & 2.59e+00  & 2.92e+01 & 1.96e+00  & 2.90e+01 & 1.40e+00  & 3.14e+01 & \first{1.04e+00}  & 3.13e+01 & 7.74e-01\\
 & LS-Uniform & \first{2.27e+01} & 4.40e+00  & \first{2.68e+01} & \first{3.24e+00}  & 5.96e+01 & 3.33e+00  & 4.40e+01 & 3.05e+00  & 1.19e+02 & 2.99e+00  & 5.04e+02 & 5.85e+00  & 1.13e+04 & 6.19e+01\\
 & LS-Chebyshev & 2.49e+01 & 5.10e+00  & 2.99e+01 & 3.74e+00  & \first{2.35e+01} & \first{2.33e+00}  & \first{2.49e+01} & \first{1.78e+00}  & \first{1.98e+01} & \first{1.33e+00}  & \first{1.92e+01} & 1.07e+00  & \first{1.81e+01} & \first{7.73e-01}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 5}\\$Q=50$}} & Smolyak & \first{4.92e+01} & 7.98e+00  & \first{5.33e+01} & \first{5.79e+00}  & 5.18e+01 & \first{4.33e+00}  & 6.96e+01 & \first{3.59e+00}  & 7.05e+01 & \first{2.61e+00}  & 7.93e+01 & \first{1.92e+00}  &  & \\
 & LS-Uniform & 5.05e+01 & 9.25e+00  & 6.57e+01 & 7.68e+00  & 7.06e+01 & 5.40e+00  & 1.27e+02 & 4.79e+00  & 1.84e+02 & 5.00e+00  & 3.20e+02 & 4.61e+00  &  & \\
 & LS-Chebyshev & 4.93e+01 & \first{7.89e+00}  & 6.37e+01 & 6.57e+00  & \first{5.03e+01} & 4.62e+00  & \first{5.36e+01} & 3.66e+00  & \first{4.26e+01} & 2.71e+00  & \first{4.79e+01} & 2.04e+00  &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 6}\\$Q=50$}} & Smolyak & 1.19e+02 & \first{1.29e+01}  & 1.67e+02 & 1.14e+01  & 1.38e+02 & \first{7.79e+00}  & 1.31e+02 & \first{5.95e+00}  & 1.75e+02 & \first{4.24e+00}  &  &   &  & \\
 & LS-Uniform & \first{1.12e+02} & 1.38e+01  & \first{1.27e+02} & \first{1.13e+01}  & 1.42e+02 & 9.37e+00  & 2.74e+02 & 8.39e+00  & 3.37e+02 & 7.03e+00  &  &   &  & \\
 & LS-Chebyshev & 1.45e+02 & 4.46e+01  & 1.37e+02 & 2.16e+01  & \first{1.01e+02} & 1.07e+01  & \first{1.08e+02} & 7.36e+00  & \first{1.01e+02} & 5.33e+00  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 7}\\$Q=50$}} & Smolyak & 3.16e+02 & \first{3.26e+01}  & 3.15e+02 & \first{2.22e+01}  & 3.21e+02 & \first{1.78e+01}  & 2.93e+02 & \first{1.29e+01}  & 3.78e+02 & \first{9.44e+00}  &  &   &  & \\
 & LS-Uniform & 5.30e+02 & 3.27e+01  & 3.72e+02 & 2.34e+01  & 4.73e+02 & 1.82e+01  & 3.96e+02 & 1.51e+01  & 7.70e+02 & 1.33e+01  &  &   &  & \\
 & LS-Chebyshev & \first{2.55e+02} & 5.16e+01  & \first{2.21e+02} & 4.58e+01  & \first{2.45e+02} & 2.90e+01  & \first{2.71e+02} & 2.14e+01  & \first{3.10e+02} & 1.54e+01  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 8}\\$Q=50$}} & Smolyak & 6.16e+02 & \first{4.12e+01}  & 4.69e+02 & \first{3.33e+01}  & 1.00e+03 & \first{2.78e+01}  & 8.55e+02 & \first{2.15e+01}  &  &   &  &   &  & \\
 & LS-Uniform & \first{4.39e+02} & 4.64e+01  & 5.24e+02 & 4.03e+01  & \first{7.67e+02} & 3.26e+01  & 8.95e+02 & 2.75e+01  &  &   &  &   &  & \\
 & LS-Chebyshev & 5.56e+02 & 8.63e+01  & \first{4.46e+02} & 6.56e+01  & 8.71e+02 & 4.60e+01  & \first{8.14e+02} & 3.56e+01  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 9}\\$Q=50$}} & Smolyak & 1.11e+03 & \first{7.78e+01}  & 1.84e+03 & \first{5.96e+01}  & 1.62e+03 & \first{4.44e+01}  & 2.28e+03 & \first{3.75e+01}  &  &   &  &   &  & \\
 & LS-Uniform & 1.25e+03 & 9.28e+01  & \first{1.59e+03} & 7.37e+01  & \first{1.57e+03} & 5.85e+01  & \first{1.85e+03} & 4.80e+01  &  &   &  &   &  & \\
 & LS-Chebyshev & \first{1.06e+03} & 1.61e+02  & 1.98e+03 & 1.45e+02  & 1.73e+03 & 9.91e+01  & 2.05e+03 & 7.17e+01  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 10}\\$Q=50$}} & Smolyak & 4.14e+03 & 2.24e+02  & 4.14e+03 & \first{1.37e+02}  & 2.92e+03 & \first{1.00e+02}  & 5.01e+03 & \first{7.81e+01}  &  &   &  &   &  & \\
 & LS-Uniform & \first{3.36e+03} & \first{1.93e+02}  & \first{2.89e+03} & 1.43e+02  & 2.62e+03 & 1.13e+02  & 4.37e+03 & 9.03e+01  &  &   &  &   &  & \\
 & LS-Chebyshev & 3.79e+03 & 4.90e+02  & 3.60e+03 & 3.37e+02  & \first{2.60e+03} & 2.30e+02  & \first{3.39e+03} & 1.75e+02  &  &   &  &   &  & \\
\bottomrule
\end{tabular}


==> tables/GAUSSIAN.tex <==
% Created with Python on 2025-06-22 19:31:18
% ..\results\final_results\low_dim\results_numerical_experiments.csv, function = GAUSSIAN, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\textbf{Dim 2}\\$Q=50$}} & Smolyak & 5.81e-01 & 2.39e-01  & 3.51e-01 & 9.72e-02  & 1.18e-01 & 3.11e-02  & 2.17e-02 & 5.03e-03  & 1.93e-03 & 4.27e-04  & 7.40e-06 & 1.88e-06  & 6.31e-09 & 1.51e-09\\
 & LS-Uniform & 3.13e+00 & 7.97e-01  & 3.83e+00 & 5.77e-01  & 3.44e+00 & 2.92e-01  & 7.53e+00 & 6.71e-01  & 2.27e+02 & 1.11e+01  & 2.62e+00 & 8.97e-02  & 1.88e+04 & 3.30e+02\\
 & LS-Chebyshev & \first{4.84e-01} & \first{1.75e-01}  & \first{3.40e-01} & \first{8.12e-02}  & \first{6.74e-02} & \first{1.90e-02}  & \first{1.67e-02} & \first{3.37e-03}  & \first{1.19e-03} & \first{2.87e-04}  & \first{5.39e-06} & \first{1.22e-06}  & \first{5.51e-09} & \first{1.08e-09}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 3}\\$Q=50$}} & Smolyak & 6.32e-01 & 2.17e-01  & 4.54e-01 & 9.92e-02  & \first{2.21e-01} & 3.99e-02  & 1.20e-01 & 1.72e-02  & 3.31e-02 & 5.10e-03  & 7.56e-03 & 8.69e-04  & 9.87e-04 & 1.01e-04\\
 & LS-Uniform & 1.66e+00 & 2.82e-01  & 7.59e-01 & 9.70e-02  & 7.69e-01 & 6.15e-02  & 6.03e-01 & 3.04e-02  & 6.14e-01 & 1.82e-02  & 9.04e-01 & 1.65e-02  & 5.56e+01 & 5.23e-01\\
 & LS-Chebyshev & \first{4.91e-01} & \first{1.28e-01}  & \first{3.66e-01} & \first{7.08e-02}  & 2.59e-01 & \first{2.74e-02}  & \first{9.23e-02} & \first{8.81e-03}  & \first{1.72e-02} & \first{2.09e-03}  & \first{2.88e-03} & \first{3.73e-04}  & \first{3.26e-04} & \first{4.46e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 4}\\$Q=50$}} & Smolyak & 6.42e-01 & 1.75e-01  & 4.80e-01 & 8.93e-02  & 3.24e-01 & 4.70e-02  & 1.98e-01 & 2.07e-02  & 1.04e-01 & 7.66e-03  & 3.94e-02 & 3.36e-03  & 9.55e-03 & 9.78e-04\\
 & LS-Uniform & 8.28e-01 & 1.35e-01  & 1.03e+00 & 7.53e-02  & 1.01e+00 & 5.19e-02  & 1.30e+00 & 2.99e-02  & 3.52e-01 & 9.70e-03  & 3.41e-01 & 4.48e-03  & 1.31e+00 & 7.83e-03\\
 & LS-Chebyshev & \first{5.90e-01} & \first{9.71e-02}  & \first{4.10e-01} & \first{5.53e-02}  & \first{2.14e-01} & \first{2.71e-02}  & \first{1.08e-01} & \first{1.13e-02}  & \first{3.82e-02} & \first{3.73e-03}  & \first{1.68e-02} & \first{1.06e-03}  & \first{5.26e-03} & \first{2.87e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 5}\\$Q=50$}} & Smolyak & 6.92e-01 & 1.18e-01  & 5.59e-01 & 7.81e-02  & 4.13e-01 & 6.14e-02  & 2.36e-01 & 2.39e-02  & 1.11e-01 & 8.48e-03  & 4.50e-02 & 3.53e-03  &  & \\
 & LS-Uniform & \first{5.93e-01} & 9.65e-02  & 1.05e+00 & 8.73e-02  & 1.11e+00 & 3.93e-02  & 6.08e-01 & 1.70e-02  & 7.12e-01 & 1.01e-02  & 8.05e-01 & 4.63e-03  &  & \\
 & LS-Chebyshev & 6.71e-01 & \first{8.36e-02}  & \first{4.57e-01} & \first{5.40e-02}  & \first{2.64e-01} & \first{2.75e-02}  & \first{1.49e-01} & \first{1.25e-02}  & \first{7.31e-02} & \first{4.62e-03}  & \first{2.69e-02} & \first{1.46e-03}  &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 6}\\$Q=50$}} & Smolyak & \first{5.74e-01} & 1.63e-01  & 5.92e-01 & 8.11e-02  & 4.88e-01 & 4.00e-02  & 3.05e-01 & 2.13e-02  & 1.95e-01 & 8.53e-03  &  &   &  & \\
 & LS-Uniform & 7.27e-01 & 1.11e-01  & 6.73e-01 & 5.92e-02  & 9.13e-01 & 3.42e-02  & 1.40e+00 & 1.85e-02  & 8.09e-01 & 8.80e-03  &  &   &  & \\
 & LS-Chebyshev & 6.30e-01 & \first{9.58e-02}  & \first{5.16e-01} & \first{5.49e-02}  & \first{3.05e-01} & \first{2.89e-02}  & \first{1.69e-01} & \first{1.34e-02}  & \first{9.95e-02} & \first{5.00e-03}  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 7}\\$Q=50$}} & Smolyak & 8.19e-01 & 8.12e-02  & 6.49e-01 & 9.23e-02  & 5.66e-01 & 3.82e-02  & 4.27e-01 & 1.90e-02  & 2.89e-01 & 1.24e-02  &  &   &  & \\
 & LS-Uniform & \first{6.16e-01} & \first{6.05e-02}  & 6.97e-01 & 3.99e-02  & 9.40e-01 & 2.56e-02  & 1.90e+00 & 1.90e-02  & 1.08e+00 & 9.96e-03  &  &   &  & \\
 & LS-Chebyshev & 6.45e-01 & 7.00e-02  & \first{5.18e-01} & \first{3.70e-02}  & \first{3.33e-01} & \first{2.22e-02}  & \first{2.45e-01} & \first{1.22e-02}  & \first{1.38e-01} & \first{6.03e-03}  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 8}\\$Q=50$}} & Smolyak & \first{5.52e-01} & 1.32e-01  & 6.66e-01 & 7.20e-02  & 5.10e-01 & 4.32e-02  & 3.42e-01 & 2.35e-02  &  &   &  &   &  & \\
 & LS-Uniform & 5.90e-01 & \first{5.49e-02}  & 9.57e-01 & \first{3.33e-02}  & 7.75e-01 & 2.12e-02  & 8.86e-01 & 1.30e-02  &  &   &  &   &  & \\
 & LS-Chebyshev & 6.10e-01 & 7.08e-02  & \first{5.32e-01} & 3.60e-02  & \first{4.23e-01} & \first{2.02e-02}  & \first{2.45e-01} & \first{1.11e-02}  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 9}\\$Q=50$}} & Smolyak & 5.85e-01 & 1.46e-01  & 9.05e-01 & 8.47e-02  & 5.07e-01 & 4.52e-02  & 3.81e-01 & 2.74e-02  &  &   &  &   &  & \\
 & LS-Uniform & \first{5.43e-01} & 4.69e-02  & 8.32e-01 & 3.36e-02  & 8.26e-01 & 2.38e-02  & 1.39e+00 & 1.49e-02  &  &   &  &   &  & \\
 & LS-Chebyshev & 5.99e-01 & \first{4.31e-02}  & \first{5.93e-01} & \first{3.13e-02}  & \first{4.24e-01} & \first{2.10e-02}  & \first{2.95e-01} & \first{1.27e-02}  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 10}\\$Q=50$}} & Smolyak & 7.29e-01 & 8.59e-02  & 6.10e-01 & 5.78e-02  & 5.69e-01 & 3.47e-02  & 4.24e-01 & 2.04e-02  &  &   &  &   &  & \\
 & LS-Uniform & \first{5.32e-01} & \first{4.63e-02}  & \first{5.28e-01} & \first{2.98e-02}  & 1.01e+00 & \first{1.82e-02}  & 9.98e-01 & 1.08e-02  &  &   &  &   &  & \\
 & LS-Chebyshev & 7.05e-01 & 5.57e-02  & 5.66e-01 & 3.15e-02  & \first{4.67e-01} & 1.96e-02  & \first{3.04e-01} & \first{1.07e-02}  &  &   &  &   &  & \\
\bottomrule
\end{tabular}


==> tables/G_FUNCTION.tex <==
% Created with Python on 2025-06-22 19:31:18
% ..\results\final_results\low_dim\results_numerical_experiments.csv, function = G_FUNCTION, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\textbf{Dim 2}\\$Q=50$}} & Smolyak & 2.48e-01 & 1.05e-01  & \first{1.14e-01} & \first{3.85e-02}  & \first{6.89e-02} & 1.54e-02  & \first{3.42e-02} & 5.39e-03  & \first{2.39e-02} & 2.13e-03  & 1.18e-02 & 9.11e-04  & 7.14e-03 & 3.33e-04\\
 & LS-Uniform & 1.29e+00 & 3.18e-01  & 2.37e+00 & 3.45e-01  & 1.61e+00 & 1.67e-01  & 9.01e+00 & 7.85e-01  & 6.36e+03 & 2.86e+02  & 5.10e+03 & 1.54e+02  & 1.57e+10 & 2.75e+08\\
 & LS-Chebyshev & \first{1.94e-01} & \first{6.80e-02}  & 1.17e-01 & 4.08e-02  & 8.27e-02 & \first{1.14e-02}  & 4.75e-02 & \first{4.39e-03}  & 2.72e-02 & \first{1.68e-03}  & \first{1.14e-02} & \first{6.19e-04}  & \first{5.41e-03} & \first{2.38e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 3}\\$Q=50$}} & Smolyak & 6.03e-01 & 1.98e-01  & 4.75e-01 & 8.99e-02  & 2.08e-01 & 4.03e-02  & 1.18e-01 & 1.54e-02  & 7.33e-02 & 6.44e-03  & \first{3.25e-02} & 2.47e-03  & 3.06e-02 & 9.64e-04\\
 & LS-Uniform & 1.09e+00 & 2.25e-01  & 4.55e-01 & 9.45e-02  & 4.46e-01 & 4.71e-02  & 9.80e-01 & 3.95e-02  & 2.31e+00 & 5.32e-02  & 1.25e+01 & 2.04e-01  & 2.03e+03 & 1.87e+01\\
 & LS-Chebyshev & \first{5.43e-01} & \first{1.53e-01}  & \first{3.43e-01} & \first{7.47e-02}  & \first{1.98e-01} & \first{3.08e-02}  & \first{9.31e-02} & \first{1.15e-02}  & \first{4.65e-02} & \first{4.66e-03}  & 3.39e-02 & \first{1.74e-03}  & \first{1.99e-02} & \first{6.82e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 4}\\$Q=50$}} & Smolyak & 1.70e+00 & 3.83e-01  & 1.30e+00 & 2.05e-01  & 7.02e-01 & 8.54e-02  & 3.40e-01 & 3.77e-02  & 2.32e-01 & 1.58e-02  & 1.24e-01 & 6.54e-03  & 4.96e-02 & 2.72e-03\\
 & LS-Uniform & 2.06e+00 & \first{2.88e-01}  & 1.16e+00 & 1.47e-01  & 1.02e+00 & 9.01e-02  & 1.02e+00 & 3.59e-02  & 6.19e-01 & 2.10e-02  & 2.03e+00 & 2.22e-02  & 1.28e+01 & 8.16e-02\\
 & LS-Chebyshev & \first{9.88e-01} & 3.53e-01  & \first{5.30e-01} & \first{1.27e-01}  & \first{2.94e-01} & \first{5.48e-02}  & \first{2.30e-01} & \first{2.59e-02}  & \first{1.19e-01} & \first{9.61e-03}  & \first{6.77e-02} & \first{3.92e-03}  & \first{4.23e-02} & \first{1.60e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 5}\\$Q=50$}} & Smolyak & 2.92e+00 & 6.22e-01  & 2.40e+00 & 3.19e-01  & 1.80e+00 & 1.67e-01  & 8.60e-01 & 8.16e-02  & 4.45e-01 & 3.77e-02  & 3.11e-01 & 1.70e-02  &  & \\
 & LS-Uniform & 2.32e+00 & \first{4.64e-01}  & 2.05e+00 & \first{2.24e-01}  & 1.88e+00 & 1.10e-01  & 1.40e+00 & 5.16e-02  & 9.51e-01 & 2.92e-02  & 1.43e+00 & 1.86e-02  &  & \\
 & LS-Chebyshev & \first{2.23e+00} & 6.17e-01  & \first{1.26e+00} & 2.63e-01  & \first{9.49e-01} & \first{1.02e-01}  & \first{3.85e-01} & \first{4.24e-02}  & \first{1.92e-01} & \first{1.79e-02}  & \first{1.58e-01} & \first{7.57e-03}  &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 6}\\$Q=50$}} & Smolyak & 6.46e+00 & 9.21e-01  & 6.57e+00 & 5.98e-01  & 4.06e+00 & 3.12e-01  & 1.86e+00 & 1.60e-01  & 1.18e+00 & 7.76e-02  &  &   &  & \\
 & LS-Uniform & \first{3.24e+00} & \first{5.50e-01}  & 4.09e+00 & \first{2.63e-01}  & 2.21e+00 & \first{1.33e-01}  & 1.91e+00 & \first{7.53e-02}  & 1.10e+00 & 3.85e-02  &  &   &  & \\
 & LS-Chebyshev & 3.78e+00 & 8.72e-01  & \first{3.10e+00} & 3.98e-01  & \first{1.66e+00} & 1.80e-01  & \first{7.14e-01} & 7.62e-02  & \first{4.85e-01} & \first{3.25e-02}  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 7}\\$Q=50$}} & Smolyak & 1.64e+01 & 1.22e+00  & 1.34e+01 & 8.31e-01  & 9.61e+00 & 4.93e-01  & 5.26e+00 & 2.66e-01  & 3.23e+00 & 1.35e-01  &  &   &  & \\
 & LS-Uniform & 7.44e+00 & \first{7.64e-01}  & 5.69e+00 & \first{4.08e-01}  & 3.73e+00 & \first{2.25e-01}  & 3.20e+00 & \first{1.20e-01}  & 2.14e+00 & \first{6.46e-02}  &  &   &  & \\
 & LS-Chebyshev & \first{6.29e+00} & 1.45e+00  & \first{3.24e+00} & 7.89e-01  & \first{2.17e+00} & 3.60e-01  & \first{1.98e+00} & 1.62e-01  & \first{9.39e-01} & 7.06e-02  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 8}\\$Q=50$}} & Smolyak & 2.29e+01 & 1.85e+00  & 2.60e+01 & 1.40e+00  & 1.89e+01 & 9.00e-01  & 1.10e+01 & 5.33e-01  &  &   &  &   &  & \\
 & LS-Uniform & \first{7.92e+00} & \first{1.30e+00}  & \first{6.54e+00} & \first{7.10e-01}  & 5.65e+00 & \first{3.95e-01}  & 5.08e+00 & \first{2.09e-01}  &  &   &  &   &  & \\
 & LS-Chebyshev & 9.91e+00 & 2.75e+00  & 6.68e+00 & 1.61e+00  & \first{4.08e+00} & 7.55e-01  & \first{2.58e+00} & 3.53e-01  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 9}\\$Q=50$}} & Smolyak & 4.61e+01 & 2.46e+00  & 4.11e+01 & 1.85e+00  & 3.73e+01 & 1.30e+00  & 2.35e+01 & 7.50e-01  &  &   &  &   &  & \\
 & LS-Uniform & 1.93e+01 & \first{1.52e+00}  & 1.51e+01 & \first{8.92e-01}  & 1.48e+01 & \first{4.86e-01}  & 8.80e+00 & \first{2.75e-01}  &  &   &  &   &  & \\
 & LS-Chebyshev & \first{1.54e+01} & 4.25e+00  & \first{1.39e+01} & 2.17e+00  & \first{8.35e+00} & 1.18e+00  & \first{4.76e+00} & 5.52e-01  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 10}\\$Q=50$}} & Smolyak & 4.96e+01 & 2.83e+00  & 6.16e+01 & 2.16e+00  & 4.62e+01 & 1.64e+00  & 5.71e+01 & 1.08e+00  &  &   &  &   &  & \\
 & LS-Uniform & \first{1.98e+01} & \first{1.64e+00}  & \first{1.61e+01} & \first{9.34e-01}  & 1.40e+01 & \first{5.31e-01}  & 1.15e+01 & \first{2.94e-01}  &  &   &  &   &  & \\
 & LS-Chebyshev & 2.68e+01 & 6.33e+00  & 1.98e+01 & 3.37e+00  & \first{1.00e+01} & 1.63e+00  & \first{7.43e+00} & 7.75e-01  &  &   &  &   &  & \\
\bottomrule
\end{tabular}


==> tables/MOROKOFF_CALFISCH_1.tex <==
% Created with Python on 2025-06-22 19:31:19
% ..\results\final_results\low_dim\results_numerical_experiments.csv, function = MOROKOFF_CALFISCH_1, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\textbf{Dim 2}\\$Q=50$}} & Smolyak & 1.09e-02 & 5.50e-03  & 2.80e-03 & \first{7.19e-04}  & \first{3.70e-04} & \first{7.25e-05}  & 4.84e-05 & 8.72e-06  & 3.65e-06 & 6.94e-07  & 1.36e-07 & 2.22e-08  & 2.19e-09 & 3.61e-10\\
 & LS-Uniform & \first{7.18e-03} & \first{1.52e-03}  & 5.70e-03 & 1.08e-03  & 1.33e-03 & 1.36e-04  & 3.29e-03 & 2.95e-04  & 1.07e-01 & 4.54e-03  & 3.88e-03 & 1.23e-04  & 2.26e+02 & 3.95e+00\\
 & LS-Chebyshev & 9.32e-03 & 4.52e-03  & \first{2.45e-03} & 9.90e-04  & 5.63e-04 & 9.85e-05  & \first{3.23e-05} & \first{7.11e-06}  & \first{3.08e-06} & \first{5.99e-07}  & \first{9.87e-08} & \first{2.00e-08}  & \first{2.06e-09} & \first{3.03e-10}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 3}\\$Q=50$}} & Smolyak & 2.27e-02 & 7.18e-03  & \first{3.20e-03} & 8.34e-04  & 3.76e-04 & 6.70e-05  & 2.58e-05 & 4.08e-06  & 2.11e-06 & 2.89e-07  & 1.44e-07 & 1.55e-08  & 6.94e-09 & 7.03e-10\\
 & LS-Uniform & 4.56e-02 & \first{6.02e-03}  & 4.19e-03 & \first{5.11e-04}  & 5.38e-04 & \first{4.27e-05}  & 5.83e-05 & 3.24e-06  & 3.39e-05 & 9.23e-07  & 1.81e-06 & 4.77e-08  & 6.44e-05 & 6.38e-07\\
 & LS-Chebyshev & \first{2.22e-02} & 6.15e-03  & 3.75e-03 & 1.06e-03  & \first{2.48e-04} & 7.25e-05  & \first{1.39e-05} & \first{3.05e-06}  & \first{9.97e-07} & \first{1.49e-07}  & \first{4.43e-08} & \first{6.60e-09}  & \first{2.38e-09} & \first{3.29e-10}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 4}\\$Q=50$}} & Smolyak & \first{8.36e-02} & 2.25e-02  & 3.02e-02 & 5.43e-03  & 9.51e-03 & 1.15e-03  & 2.33e-03 & 2.05e-04  & 5.75e-04 & 3.13e-05  & 9.34e-05 & 4.02e-06  & 1.07e-05 & 4.43e-07\\
 & LS-Uniform & 1.03e-01 & \first{1.27e-02}  & \first{2.90e-02} & \first{2.50e-03}  & 1.35e-02 & \first{5.94e-04}  & 5.62e-03 & \first{1.27e-04}  & 8.25e-04 & \first{1.35e-05}  & 1.25e-04 & \first{2.09e-06}  & 1.18e-04 & 9.63e-07\\
 & LS-Chebyshev & 1.03e-01 & 3.31e-02  & 2.91e-02 & 7.40e-03  & \first{5.91e-03} & 1.19e-03  & \first{8.35e-04} & 2.12e-04  & \first{1.92e-04} & 2.86e-05  & \first{1.68e-05} & 2.98e-06  & \first{3.13e-06} & \first{2.92e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 5}\\$Q=50$}} & Smolyak & \first{2.20e-02} & 5.62e-03  & 5.79e-03 & 9.61e-04  & 1.28e-03 & 1.42e-04  & 1.84e-04 & 1.79e-05  & 3.08e-05 & 1.64e-06  & 3.21e-06 & 1.30e-07  &  & \\
 & LS-Uniform & 3.12e-02 & \first{4.22e-03}  & 6.55e-03 & \first{5.47e-04}  & 1.46e-03 & \first{6.65e-05}  & 3.74e-04 & \first{8.14e-06}  & 5.12e-05 & \first{9.06e-07}  & 4.22e-06 & \first{6.83e-08}  &  & \\
 & LS-Chebyshev & 2.24e-02 & 8.09e-03  & \first{4.78e-03} & 7.64e-04  & \first{5.93e-04} & 1.02e-04  & \first{6.03e-05} & 1.21e-05  & \first{1.06e-05} & 1.30e-06  & \first{1.13e-06} & 1.03e-07  &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 6}\\$Q=50$}} & Smolyak & \first{9.67e-02} & 2.23e-02  & 3.33e-02 & 4.40e-03  & 6.61e-03 & 6.20e-04  & 1.20e-03 & 1.12e-04  & 3.06e-04 & 1.70e-05  &  &   &  & \\
 & LS-Uniform & 1.24e-01 & \first{1.62e-02}  & 2.86e-02 & \first{3.13e-03}  & 8.01e-03 & \first{3.48e-04}  & 4.62e-03 & \first{5.96e-05}  & 5.21e-04 & \first{8.06e-06}  &  &   &  & \\
 & LS-Chebyshev & 1.04e-01 & 2.51e-02  & \first{2.43e-02} & 5.71e-03  & \first{5.20e-03} & 9.03e-04  & \first{7.05e-04} & 9.40e-05  & \first{1.05e-04} & 1.40e-05  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 7}\\$Q=50$}} & Smolyak & 2.12e-01 & 3.39e-02  & \first{5.98e-02} & 9.17e-03  & 1.69e-02 & 1.66e-03  & 5.02e-03 & 3.01e-04  & 1.22e-03 & 5.36e-05  &  &   &  & \\
 & LS-Uniform & 2.46e-01 & \first{1.96e-02}  & 6.28e-02 & \first{5.51e-03}  & 2.67e-02 & \first{9.99e-04}  & 5.91e-03 & \first{1.25e-04}  & 1.96e-03 & \first{1.69e-05}  &  &   &  & \\
 & LS-Chebyshev & \first{1.69e-01} & 4.66e-02  & 7.30e-02 & 1.61e-02  & \first{1.53e-02} & 2.97e-03  & \first{2.32e-03} & 3.96e-04  & \first{4.64e-04} & 5.06e-05  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 8}\\$Q=50$}} & Smolyak & \first{7.50e-02} & 1.68e-02  & 2.32e-02 & 3.01e-03  & 6.07e-03 & 5.67e-04  & 1.60e-03 & 1.05e-04  &  &   &  &   &  & \\
 & LS-Uniform & 8.86e-02 & \first{1.09e-02}  & 2.59e-02 & \first{1.87e-03}  & \first{3.50e-03} & \first{2.15e-04}  & 1.94e-03 & \first{2.84e-05}  &  &   &  &   &  & \\
 & LS-Chebyshev & 1.03e-01 & 2.53e-02  & \first{2.16e-02} & 4.55e-03  & 4.17e-03 & 5.71e-04  & \first{3.78e-04} & 6.69e-05  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 9}\\$Q=50$}} & Smolyak & 1.54e-01 & 3.18e-02  & \first{5.70e-02} & 8.03e-03  & \first{1.56e-02} & 1.37e-03  & 3.57e-03 & 1.52e-04  &  &   &  &   &  & \\
 & LS-Uniform & \first{1.28e-01} & \first{1.48e-02}  & 7.95e-02 & \first{4.52e-03}  & 2.44e-02 & \first{8.86e-04}  & 4.25e-03 & \first{8.22e-05}  &  &   &  &   &  & \\
 & LS-Chebyshev & 1.58e-01 & 4.58e-02  & 6.94e-02 & 1.42e-02  & 1.70e-02 & 2.74e-03  & \first{2.24e-03} & 2.98e-04  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 10}\\$Q=50$}} & Smolyak & 2.11e-01 & 3.30e-02  & 1.24e-01 & 1.11e-02  & 5.30e-02 & 3.61e-03  & 1.45e-02 & 1.10e-03  &  &   &  &   &  & \\
 & LS-Uniform & \first{1.33e-01} & \first{1.46e-02}  & 7.36e-02 & \first{4.07e-03}  & 2.87e-02 & \first{8.66e-04}  & 1.27e-02 & \first{1.82e-04}  &  &   &  &   &  & \\
 & LS-Chebyshev & 1.70e-01 & 3.77e-02  & \first{5.84e-02} & 1.26e-02  & \first{1.60e-02} & 2.92e-03  & \first{7.23e-03} & 8.24e-04  &  &   &  &   &  & \\
\bottomrule
\end{tabular}


==> tables/NOISE.tex <==
% Created with Python on 2025-06-22 19:31:19
% ..\results\final_results\low_dim\results_numerical_experiments.csv, function = NOISE, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\textbf{Dim 2}\\$Q=50$}} & Smolyak & 6.00e-07 & 3.07e-07  & 6.46e-07 & 2.64e-07  & 7.78e-07 & 2.43e-07  & \first{8.85e-07} & 2.38e-07  & 9.21e-07 & 2.39e-07  & 1.21e-06 & 2.51e-07  & 1.25e-06 & 2.57e-07\\
 & LS-Uniform & 4.11e-06 & 1.04e-06  & 2.12e-05 & 3.07e-06  & 1.98e-05 & 2.30e-06  & 2.21e-04 & 2.00e-05  & 5.97e-01 & 2.69e-02  & 1.65e+00 & 5.52e-02  & 1.05e+07 & 1.84e+05\\
 & LS-Chebyshev & \first{5.59e-07} & \first{2.36e-07}  & \first{5.80e-07} & \first{1.97e-07}  & \first{7.30e-07} & \first{1.51e-07}  & 1.13e-06 & \first{1.47e-07}  & \first{8.96e-07} & \first{1.35e-07}  & \first{7.56e-07} & \first{1.28e-07}  & \first{7.61e-07} & \first{1.27e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 3}\\$Q=50$}} & Smolyak & 9.86e-07 & 3.43e-07  & 1.25e-06 & 3.48e-07  & 1.44e-06 & 4.06e-07  & 1.80e-06 & 4.04e-07  & 2.24e-06 & 4.56e-07  & 2.73e-06 & 4.96e-07  & 3.06e-06 & 5.57e-07\\
 & LS-Uniform & 1.75e-06 & 3.59e-07  & 1.39e-06 & 2.47e-07  & 3.84e-06 & 3.29e-07  & 2.20e-05 & 8.19e-07  & 6.91e-05 & 1.80e-06  & 6.26e-04 & 1.09e-05  & 2.51e-01 & 2.57e-03\\
 & LS-Chebyshev & \first{6.16e-07} & \first{1.70e-07}  & \first{6.21e-07} & \first{1.59e-07}  & \first{6.35e-07} & \first{1.49e-07}  & \first{8.77e-07} & \first{1.46e-07}  & \first{9.05e-07} & \first{1.43e-07}  & \first{7.14e-07} & \first{1.38e-07}  & \first{7.36e-07} & \first{1.31e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 4}\\$Q=50$}} & Smolyak & 1.65e-06 & 4.23e-07  & 2.09e-06 & 5.18e-07  & 2.63e-06 & 5.34e-07  & 4.27e-06 & 6.76e-07  & 4.65e-06 & 7.53e-07  & 5.81e-06 & 9.02e-07  & 6.78e-06 & 1.02e-06\\
 & LS-Uniform & 1.45e-06 & 1.96e-07  & 1.48e-06 & 1.88e-07  & 3.94e-06 & 2.58e-07  & 6.85e-06 & 2.78e-07  & 1.39e-05 & 4.01e-07  & 7.98e-05 & 9.71e-07  & 2.00e-03 & 1.32e-05\\
 & LS-Chebyshev & \first{6.18e-07} & \first{1.75e-07}  & \first{7.31e-07} & \first{1.71e-07}  & \first{7.82e-07} & \first{1.49e-07}  & \first{8.05e-07} & \first{1.38e-07}  & \first{7.41e-07} & \first{1.39e-07}  & \first{7.44e-07} & \first{1.37e-07}  & \first{7.95e-07} & \first{1.37e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 5}\\$Q=50$}} & Smolyak & 1.86e-06 & 5.11e-07  & 2.72e-06 & 6.52e-07  & 4.71e-06 & 7.87e-07  & 6.50e-06 & 9.68e-07  & 9.92e-06 & 1.21e-06  & 1.06e-05 & 1.47e-06  &  & \\
 & LS-Uniform & 1.13e-06 & \first{1.76e-07}  & 1.67e-06 & 1.92e-07  & 3.03e-06 & 1.90e-07  & 7.35e-06 & 2.27e-07  & 1.06e-05 & 2.99e-07  & 3.63e-05 & 4.34e-07  &  & \\
 & LS-Chebyshev & \first{8.94e-07} & 1.77e-07  & \first{7.39e-07} & \first{1.51e-07}  & \first{7.12e-07} & \first{1.48e-07}  & \first{8.82e-07} & \first{1.48e-07}  & \first{7.43e-07} & \first{1.42e-07}  & \first{8.45e-07} & \first{1.43e-07}  &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 6}\\$Q=50$}} & Smolyak & 2.98e-06 & 6.30e-07  & 4.34e-06 & 9.47e-07  & 8.13e-06 & 1.08e-06  & 1.08e-05 & 1.42e-06  & 1.53e-05 & 1.84e-06  &  &   &  & \\
 & LS-Uniform & 1.09e-06 & \first{1.62e-07}  & 2.38e-06 & \first{1.61e-07}  & 2.97e-06 & 1.74e-07  & 8.25e-06 & 2.14e-07  & 1.15e-05 & 2.52e-07  &  &   &  & \\
 & LS-Chebyshev & \first{7.27e-07} & 1.73e-07  & \first{7.92e-07} & 1.63e-07  & \first{7.93e-07} & \first{1.57e-07}  & \first{8.30e-07} & \first{1.49e-07}  & \first{9.26e-07} & \first{1.49e-07}  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 7}\\$Q=50$}} & Smolyak & 3.89e-06 & 7.36e-07  & 7.43e-06 & 1.18e-06  & 1.29e-05 & 1.44e-06  & 1.83e-05 & 1.99e-06  & 2.80e-05 & 2.59e-06  &  &   &  & \\
 & LS-Uniform & 1.03e-06 & \first{1.40e-07}  & 2.18e-06 & \first{1.50e-07}  & 4.86e-06 & 1.72e-07  & 7.99e-06 & 1.94e-07  & 1.59e-05 & 2.34e-07  &  &   &  & \\
 & LS-Chebyshev & \first{6.94e-07} & 1.70e-07  & \first{8.48e-07} & 1.70e-07  & \first{9.50e-07} & \first{1.58e-07}  & \first{1.07e-06} & \first{1.55e-07}  & \first{1.12e-06} & \first{1.56e-07}  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 8}\\$Q=50$}} & Smolyak & 5.30e-06 & 8.86e-07  & 1.10e-05 & 1.46e-06  & 1.77e-05 & 1.94e-06  & 2.64e-05 & 2.67e-06  &  &   &  &   &  & \\
 & LS-Uniform & 9.18e-07 & \first{1.34e-07}  & 1.41e-06 & \first{1.42e-07}  & 3.08e-06 & \first{1.58e-07}  & 6.80e-06 & 1.81e-07  &  &   &  &   &  & \\
 & LS-Chebyshev & \first{7.69e-07} & 1.75e-07  & \first{8.40e-07} & 1.63e-07  & \first{9.82e-07} & 1.61e-07  & \first{1.08e-06} & \first{1.61e-07}  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 9}\\$Q=50$}} & Smolyak & 5.41e-06 & 1.18e-06  & 1.23e-05 & 1.76e-06  & 2.59e-05 & 2.62e-06  & 3.88e-05 & 3.57e-06  &  &   &  &   &  & \\
 & LS-Uniform & 1.03e-06 & \first{1.31e-07}  & 1.69e-06 & \first{1.39e-07}  & 3.67e-06 & \first{1.53e-07}  & 1.05e-05 & 1.74e-07  &  &   &  &   &  & \\
 & LS-Chebyshev & \first{7.20e-07} & 1.85e-07  & \first{9.39e-07} & 1.73e-07  & \first{1.14e-06} & 1.65e-07  & \first{1.33e-06} & \first{1.65e-07}  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 10}\\$Q=50$}} & Smolyak & 1.06e-05 & 1.74e-06  & 2.09e-05 & 2.14e-06  & 3.98e-05 & 3.22e-06  & 6.21e-05 & 4.71e-06  &  &   &  &   &  & \\
 & LS-Uniform & 7.99e-07 & \first{1.25e-07}  & 1.42e-06 & \first{1.31e-07}  & 3.67e-06 & \first{1.47e-07}  & 5.65e-06 & \first{1.65e-07}  &  &   &  &   &  & \\
 & LS-Chebyshev & \first{7.85e-07} & 1.77e-07  & \first{1.01e-06} & 1.76e-07  & \first{1.15e-06} & 1.70e-07  & \first{1.29e-06} & 1.68e-07  &  &   &  &   &  & \\
\bottomrule
\end{tabular}


==> tables/OSCILLATORY.tex <==
% Created with Python on 2025-06-22 19:31:19
% ..\results\final_results\low_dim\results_numerical_experiments.csv, function = OSCILLATORY, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\textbf{Dim 2}\\$Q=50$}} & Smolyak & \first{3.97e-02} & 2.52e-02  & \first{2.12e-03} & 1.06e-03  & \first{4.48e-05} & 1.87e-05  & 9.42e-09 & 3.35e-09  & 5.70e-13 & 1.95e-13  & \first{9.44e-15} & \first{2.26e-15}  & \first{1.97e-14} & 3.65e-15\\
 & LS-Uniform & 1.69e-01 & 3.71e-02  & 9.31e-03 & 1.42e-03  & 1.97e-04 & 3.00e-05  & 2.71e-06 & 2.40e-07  & 7.01e-08 & 3.60e-09  & 7.54e-09 & 2.53e-10  & 5.83e-02 & 1.02e-03\\
 & LS-Chebyshev & 4.57e-02 & \first{1.78e-02}  & 2.53e-03 & \first{8.35e-04}  & 5.56e-05 & \first{1.33e-05}  & \first{7.69e-09} & \first{2.20e-09}  & \first{5.26e-13} & \first{1.40e-13}  & 3.43e-14 & 2.88e-15  & 2.81e-14 & \first{2.41e-15}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 3}\\$Q=50$}} & Smolyak & \first{4.60e-01} & \first{1.54e-01}  & \first{8.77e-02} & 3.12e-02  & 9.48e-03 & 3.25e-03  & 5.94e-04 & 1.77e-04  & 2.01e-05 & 4.99e-06  & 2.82e-07 & 6.29e-08  & 7.89e-11 & 1.71e-11\\
 & LS-Uniform & 1.12e+00 & 2.40e-01  & 1.43e-01 & \first{1.71e-02}  & 2.46e-02 & 1.93e-03  & 2.61e-03 & 1.24e-04  & 2.75e-04 & 7.39e-06  & 4.31e-05 & 7.63e-07  & 4.07e-06 & 3.67e-08\\
 & LS-Chebyshev & 6.95e-01 & 1.94e-01  & 9.86e-02 & 2.25e-02  & \first{8.00e-03} & \first{1.65e-03}  & \first{3.41e-04} & \first{7.41e-05}  & \first{1.38e-05} & \first{2.08e-06}  & \first{1.45e-07} & \first{2.87e-08}  & \first{4.98e-11} & \first{7.59e-12}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 4}\\$Q=50$}} & Smolyak & \first{1.73e+00} & \first{3.71e-01}  & \first{6.40e-01} & 1.27e-01  & 1.47e-01 & 3.57e-02  & 2.27e-02 & 5.91e-03  & 2.29e-03 & 5.81e-04  & 1.65e-04 & 3.36e-05  & 6.86e-06 & 1.18e-06\\
 & LS-Uniform & 2.57e+00 & 4.73e-01  & 1.12e+00 & \first{1.18e-01}  & 3.74e-01 & \first{2.14e-02}  & 8.01e-02 & \first{2.14e-03}  & 6.46e-03 & 1.75e-04  & 8.88e-04 & 1.58e-05  & 4.14e-04 & 3.25e-06\\
 & LS-Chebyshev & 2.99e+00 & 6.38e-01  & 1.04e+00 & 2.00e-01  & \first{1.19e-01} & 2.60e-02  & \first{1.21e-02} & 2.29e-03  & \first{1.06e-03} & \first{1.60e-04}  & \first{6.54e-05} & \first{8.09e-06}  & \first{2.32e-06} & \first{2.84e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 5}\\$Q=50$}} & Smolyak & \first{3.16e+00} & \first{6.35e-01}  & \first{1.96e+00} & \first{3.25e-01}  & 8.12e-01 & 1.37e-01  & 1.98e-01 & 3.66e-02  & 3.98e-02 & 8.11e-03  & 5.71e-03 & 1.11e-03  &  & \\
 & LS-Uniform & 7.47e+00 & 8.13e-01  & 3.53e+00 & 3.44e-01  & 1.87e+00 & \first{8.95e-02}  & 1.44e+00 & \first{2.34e-02}  & 2.71e-01 & 3.65e-03  & 3.33e-02 & 3.65e-04  &  & \\
 & LS-Chebyshev & 3.93e+00 & 1.02e+00  & 2.23e+00 & 5.68e-01  & \first{7.15e-01} & 1.66e-01  & \first{1.56e-01} & 3.08e-02  & \first{2.59e-02} & \first{3.41e-03}  & \first{2.31e-03} & \first{2.90e-04}  &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 6}\\$Q=50$}} & Smolyak & 8.22e+00 & \first{9.31e-01}  & 5.60e+00 & \first{5.52e-01}  & 2.34e+00 & 2.79e-01  & 9.08e-01 & 1.15e-01  & 2.67e-01 & 3.63e-02  &  &   &  & \\
 & LS-Uniform & 7.38e+00 & 9.44e-01  & 7.51e+00 & 6.52e-01  & 6.52e+00 & \first{2.55e-01}  & 4.17e+00 & \first{8.02e-02}  & 1.47e+00 & \first{1.98e-02}  &  &   &  & \\
 & LS-Chebyshev & \first{5.68e+00} & 1.28e+00  & \first{3.63e+00} & 9.07e-01  & \first{2.31e+00} & 4.57e-01  & \first{7.52e-01} & 1.33e-01  & \first{1.63e-01} & 2.75e-02  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 7}\\$Q=50$}} & Smolyak & 1.07e+01 & 1.22e+00  & 9.41e+00 & 9.07e-01  & 5.95e+00 & 5.23e-01  & 3.24e+00 & 2.56e-01  & 1.26e+00 & 1.05e-01  &  &   &  & \\
 & LS-Uniform & 1.10e+01 & \first{1.12e+00}  & 1.37e+01 & \first{7.95e-01}  & 2.03e+01 & \first{4.98e-01}  & 1.55e+01 & \first{2.40e-01}  & 8.97e+00 & \first{7.95e-02}  &  &   &  & \\
 & LS-Chebyshev & \first{6.02e+00} & 1.39e+00  & \first{4.89e+00} & 1.17e+00  & \first{4.09e+00} & 7.94e-01  & \first{2.75e+00} & 4.25e-01  & \first{8.34e-01} & 1.35e-01  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 8}\\$Q=50$}} & Smolyak & 1.74e+01 & 1.53e+00  & 1.66e+01 & 1.13e+00  & 1.42e+01 & 7.29e-01  & 1.29e+01 & 4.34e-01  &  &   &  &   &  & \\
 & LS-Uniform & 1.07e+01 & \first{1.20e+00}  & 1.22e+01 & \first{9.90e-01}  & 1.71e+01 & \first{7.00e-01}  & 2.00e+01 & \first{4.00e-01}  &  &   &  &   &  & \\
 & LS-Chebyshev & \first{5.75e+00} & 1.45e+00  & \first{5.84e+00} & 1.27e+00  & \first{5.79e+00} & 1.09e+00  & \first{4.52e+00} & 7.55e-01  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 9}\\$Q=50$}} & Smolyak & 2.42e+01 & 2.27e+00  & 3.33e+01 & 1.48e+00  & 2.19e+01 & 1.12e+00  & 2.13e+01 & 7.17e-01  &  &   &  &   &  & \\
 & LS-Uniform & 8.54e+00 & \first{1.15e+00}  & 1.69e+01 & \first{1.07e+00}  & 3.41e+01 & \first{8.90e-01}  & 4.13e+01 & \first{6.09e-01}  &  &   &  &   &  & \\
 & LS-Chebyshev & \first{6.95e+00} & 1.52e+00  & \first{6.84e+00} & 1.41e+00  & \first{6.82e+00} & 1.24e+00  & \first{6.29e+00} & 9.71e-01  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 10}\\$Q=50$}} & Smolyak & 4.10e+01 & 3.10e+00  & 4.89e+01 & 2.10e+00  & 4.38e+01 & 1.44e+00  & 4.67e+01 & 9.71e-01  &  &   &  &   &  & \\
 & LS-Uniform & 6.72e+00 & \first{1.12e+00}  & 1.70e+01 & \first{1.13e+00}  & 4.13e+01 & \first{1.09e+00}  & 6.83e+01 & \first{8.65e-01}  &  &   &  &   &  & \\
 & LS-Chebyshev & \first{6.05e+00} & 1.46e+00  & \first{7.55e+00} & 1.44e+00  & \first{7.39e+00} & 1.34e+00  & \first{8.18e+00} & 1.20e+00  &  &   &  &   &  & \\
\bottomrule
\end{tabular}


==> tables/PRODUCT_PEAK.tex <==
% Created with Python on 2025-06-22 19:31:19
% ..\results\final_results\low_dim\results_numerical_experiments.csv, function = PRODUCT_PEAK, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\textbf{Dim 2}\\$Q=50$}} & Smolyak & \first{1.04e-03} & 6.17e-04  & \first{8.63e-05} & 3.77e-05  & 3.51e-06 & 1.24e-06  & 2.27e-08 & 7.41e-09  & 3.03e-11 & 8.55e-12  & \first{7.77e-15} & 2.15e-15  & \first{1.80e-14} & 3.63e-15\\
 & LS-Uniform & 4.27e-03 & 9.86e-04  & 4.65e-04 & 7.06e-05  & 1.99e-05 & 2.55e-06  & 7.28e-06 & 6.43e-07  & 3.65e-06 & 1.54e-07  & 3.19e-09 & 1.14e-10  & 2.16e-02 & 3.83e-04\\
 & LS-Chebyshev & 1.05e-03 & \first{5.03e-04}  & 1.01e-04 & \first{3.20e-05}  & \first{3.45e-06} & \first{8.70e-07}  & \first{1.81e-08} & \first{4.66e-09}  & \first{2.75e-11} & \first{6.14e-12}  & 1.55e-14 & \first{1.79e-15}  & 2.56e-14 & \first{1.73e-15}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 3}\\$Q=50$}} & Smolyak & 3.13e-03 & 1.28e-03  & 4.30e-04 & 1.57e-04  & 4.39e-05 & 1.56e-05  & 3.80e-06 & 1.11e-06  & 2.04e-07 & 4.59e-08  & 5.45e-09 & 9.51e-10  & 4.20e-11 & 7.27e-12\\
 & LS-Uniform & 9.12e-03 & 1.56e-03  & 5.74e-04 & \first{7.52e-05}  & 8.01e-05 & \first{8.11e-06}  & 1.44e-05 & 7.00e-07  & 2.28e-06 & 6.98e-08  & 9.92e-07 & 1.61e-08  & 1.46e-06 & 1.47e-08\\
 & LS-Chebyshev & \first{2.53e-03} & \first{1.04e-03}  & \first{4.28e-04} & 1.07e-04  & \first{3.82e-05} & 8.14e-06  & \first{2.77e-06} & \first{5.03e-07}  & \first{1.50e-07} & \first{2.05e-08}  & \first{2.57e-09} & \first{4.36e-10}  & \first{2.47e-11} & \first{3.23e-12}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 4}\\$Q=50$}} & Smolyak & 7.49e-03 & 1.86e-03  & 1.17e-03 & 2.97e-04  & 1.95e-04 & 4.47e-05  & 2.37e-05 & 5.74e-06  & 2.36e-06 & 5.40e-07  & 2.12e-07 & 3.75e-08  & 1.43e-08 & 1.83e-09\\
 & LS-Uniform & 7.81e-03 & \first{1.60e-03}  & 3.43e-03 & \first{1.92e-04}  & 3.59e-04 & \first{2.02e-05}  & 7.85e-05 & 2.11e-06  & 5.35e-06 & \first{1.28e-07}  & 9.85e-07 & 1.64e-08  & 8.28e-07 & 5.47e-09\\
 & LS-Chebyshev & \first{6.16e-03} & 2.04e-03  & \first{1.13e-03} & 2.97e-04  & \first{1.08e-04} & 2.55e-05  & \first{1.09e-05} & \first{2.09e-06}  & \first{1.10e-06} & 1.52e-07  & \first{7.08e-08} & \first{9.16e-09}  & \first{4.38e-09} & \first{4.44e-10}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 5}\\$Q=50$}} & Smolyak & 9.44e-03 & 1.67e-03  & \first{1.51e-03} & 3.14e-04  & \first{3.04e-04} & 5.54e-05  & 4.84e-05 & 8.17e-06  & 6.45e-06 & 1.09e-06  & 8.07e-07 & 1.28e-07  &  & \\
 & LS-Uniform & \first{7.66e-03} & \first{1.25e-03}  & 2.88e-03 & \first{2.89e-04}  & 1.22e-03 & \first{3.95e-05}  & 2.85e-04 & 5.28e-06  & 2.59e-05 & 4.58e-07  & 5.06e-06 & 4.72e-08  &  & \\
 & LS-Chebyshev & 9.17e-03 & 2.19e-03  & 2.11e-03 & 3.67e-04  & 3.62e-04 & 4.76e-05  & \first{4.66e-05} & \first{4.97e-06}  & \first{4.87e-06} & \first{4.37e-07}  & \first{3.99e-07} & \first{3.50e-08}  &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 6}\\$Q=50$}} & Smolyak & \first{9.11e-03} & \first{1.58e-03}  & \first{2.55e-03} & 2.81e-04  & \first{3.29e-04} & 4.74e-05  & \first{5.42e-05} & 7.37e-06  & \first{8.00e-06} & 1.14e-06  &  &   &  & \\
 & LS-Uniform & 1.96e-02 & 1.84e-03  & 4.56e-03 & \first{2.72e-04}  & 7.60e-04 & \first{2.89e-05}  & 3.73e-04 & \first{4.33e-06}  & 8.31e-05 & \first{6.08e-07}  &  &   &  & \\
 & LS-Chebyshev & 1.50e-02 & 2.60e-03  & 3.33e-03 & 3.93e-04  & 4.72e-04 & 4.64e-05  & 8.14e-05 & 5.99e-06  & 1.09e-05 & 6.35e-07  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 7}\\$Q=50$}} & Smolyak & \first{8.35e-03} & \first{1.62e-03}  & \first{2.36e-03} & 3.25e-04  & \first{5.73e-04} & 6.41e-05  & \first{1.18e-04} & 1.13e-05  & \first{2.85e-05} & 1.87e-06  &  &   &  & \\
 & LS-Uniform & 1.49e-02 & 1.82e-03  & 4.91e-03 & \first{3.00e-04}  & 8.68e-04 & \first{4.60e-05}  & 3.77e-04 & \first{6.61e-06}  & 1.35e-04 & \first{1.14e-06}  &  &   &  & \\
 & LS-Chebyshev & 1.38e-02 & 2.93e-03  & 4.36e-03 & 5.51e-04  & 7.29e-04 & 7.56e-05  & 1.61e-04 & 1.14e-05  & 2.90e-05 & 1.40e-06  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 8}\\$Q=50$}} & Smolyak & \first{1.07e-02} & 1.34e-03  & \first{3.01e-03} & 2.86e-04  & \first{1.05e-03} & 6.48e-05  & \first{2.19e-04} & 1.16e-05  &  &   &  &   &  & \\
 & LS-Uniform & 1.70e-02 & \first{1.32e-03}  & 4.71e-03 & \first{2.49e-04}  & 1.48e-03 & \first{4.39e-05}  & 1.19e-03 & \first{7.35e-06}  &  &   &  &   &  & \\
 & LS-Chebyshev & 1.87e-02 & 2.34e-03  & 5.39e-03 & 4.65e-04  & 1.11e-03 & 8.02e-05  & 2.30e-04 & 1.16e-05  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 9}\\$Q=50$}} & Smolyak & \first{1.05e-02} & 1.84e-03  & \first{3.58e-03} & 3.43e-04  & \first{9.39e-04} & 6.33e-05  & \first{1.40e-04} & 1.04e-05  &  &   &  &   &  & \\
 & LS-Uniform & 1.62e-02 & \first{1.52e-03}  & 8.66e-03 & \first{3.02e-04}  & 2.92e-03 & \first{4.69e-05}  & 9.15e-04 & \first{7.01e-06}  &  &   &  &   &  & \\
 & LS-Chebyshev & 2.39e-02 & 3.22e-03  & 6.19e-03 & 5.25e-04  & 1.35e-03 & 8.90e-05  & 2.73e-04 & 1.25e-05  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 10}\\$Q=50$}} & Smolyak & \first{1.53e-02} & 1.89e-03  & \first{4.83e-03} & 4.05e-04  & \first{1.79e-03} & 6.80e-05  & \first{2.96e-04} & 1.34e-05  &  &   &  &   &  & \\
 & LS-Uniform & 3.22e-02 & \first{1.41e-03}  & 8.72e-03 & \first{2.71e-04}  & 3.74e-03 & \first{5.71e-05}  & 1.61e-03 & \first{1.08e-05}  &  &   &  &   &  & \\
 & LS-Chebyshev & 1.99e-02 & 2.59e-03  & 8.62e-03 & 5.31e-04  & 2.12e-03 & 9.73e-05  & 5.25e-04 & 1.85e-05  &  &   &  &   &  & \\
\bottomrule
\end{tabular}


==> tables/ZHOU.tex <==
% Created with Python on 2025-06-22 19:31:19
% ..\results\final_results\low_dim\results_numerical_experiments.csv, function = ZHOU, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\textbf{Dim 2}\\$Q=50$}} & Smolyak & \first{5.71e-01} & \first{2.69e-01}  & \first{3.66e-01} & 1.55e-01  & 1.91e-01 & 7.14e-02  & 3.33e-02 & 9.39e-03  & 2.47e-03 & 6.16e-04  & 8.96e-06 & 2.44e-06  & 7.95e-09 & 2.19e-09\\
 & LS-Uniform & 3.51e+00 & 8.16e-01  & 5.12e+00 & 7.82e-01  & 3.56e+00 & 3.27e-01  & 8.19e+00 & 7.13e-01  & 3.15e+02 & 1.41e+01  & 1.93e+00 & 6.95e-02  & 3.03e+04 & 5.31e+02\\
 & LS-Chebyshev & 7.40e-01 & 2.89e-01  & 4.20e-01 & \first{1.35e-01}  & \first{1.87e-01} & \first{4.82e-02}  & \first{2.24e-02} & \first{6.11e-03}  & \first{1.52e-03} & \first{4.10e-04}  & \first{6.78e-06} & \first{1.50e-06}  & \first{7.27e-09} & \first{1.52e-09}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 3}\\$Q=50$}} & Smolyak & 7.17e-01 & 2.93e-01  & \first{4.04e-01} & 1.43e-01  & 2.98e-01 & 8.74e-02  & 1.06e-01 & 2.28e-02  & 2.71e-02 & 5.99e-03  & 5.82e-03 & 9.34e-04  & 6.64e-04 & 1.12e-04\\
 & LS-Uniform & 2.47e+00 & 4.44e-01  & 1.33e+00 & 2.13e-01  & 8.83e-01 & 1.27e-01  & 1.37e+00 & 6.60e-02  & 7.62e-01 & 2.36e-02  & 1.42e+00 & 2.36e-02  & 4.05e+01 & 4.14e-01\\
 & LS-Chebyshev & \first{6.04e-01} & \first{1.77e-01}  & 5.85e-01 & \first{1.25e-01}  & \first{2.25e-01} & \first{5.65e-02}  & \first{7.17e-02} & \first{1.27e-02}  & \first{2.26e-02} & \first{2.86e-03}  & \first{3.83e-03} & \first{4.99e-04}  & \first{3.65e-04} & \first{5.14e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 4}\\$Q=50$}} & Smolyak & \first{6.34e-01} & 1.76e-01  & 6.14e-01 & 1.27e-01  & 3.43e-01 & 8.48e-02  & 1.77e-01 & 4.25e-02  & 1.01e-01 & 1.36e-02  & 3.60e-02 & 3.18e-03  & 9.18e-03 & 8.39e-04\\
 & LS-Uniform & 1.40e+00 & 1.86e-01  & 1.15e+00 & 1.23e-01  & 1.10e+00 & 9.00e-02  & 7.49e-01 & 3.09e-02  & 4.71e-01 & 1.36e-02  & 3.80e-01 & 5.27e-03  & 1.39e+00 & 7.92e-03\\
 & LS-Chebyshev & 7.14e-01 & \first{1.56e-01}  & \first{5.03e-01} & \first{8.22e-02}  & \first{2.35e-01} & \first{4.60e-02}  & \first{1.18e-01} & \first{1.95e-02}  & \first{4.77e-02} & \first{6.20e-03}  & \first{1.29e-02} & \first{1.29e-03}  & \first{3.03e-03} & \first{2.47e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 5}\\$Q=50$}} & Smolyak & 6.58e-01 & 2.19e-01  & 6.01e-01 & 9.79e-02  & 3.44e-01 & 6.83e-02  & 2.10e-01 & 3.35e-02  & 1.14e-01 & 1.41e-02  & 5.70e-02 & 5.97e-03  &  & \\
 & LS-Uniform & 9.73e-01 & 1.46e-01  & 1.01e+00 & 8.20e-02  & 1.05e+00 & 5.14e-02  & 1.27e+00 & 2.76e-02  & 1.21e+00 & 1.35e-02  & 8.27e-01 & 5.01e-03  &  & \\
 & LS-Chebyshev & \first{5.92e-01} & \first{1.11e-01}  & \first{4.63e-01} & \first{6.17e-02}  & \first{2.71e-01} & \first{3.30e-02}  & \first{1.56e-01} & \first{1.79e-02}  & \first{6.91e-02} & \first{7.30e-03}  & \first{2.88e-02} & \first{2.14e-03}  &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 6}\\$Q=50$}} & Smolyak & 7.63e-01 & 1.60e-01  & 5.55e-01 & 1.10e-01  & 4.59e-01 & 6.18e-02  & 3.38e-01 & 2.96e-02  & 1.88e-01 & 1.22e-02  &  &   &  & \\
 & LS-Uniform & 9.79e-01 & \first{1.16e-01}  & 1.28e+00 & 7.12e-02  & 7.96e-01 & 3.72e-02  & 8.97e-01 & 2.03e-02  & 7.20e-01 & 1.21e-02  &  &   &  & \\
 & LS-Chebyshev & \first{7.01e-01} & 1.23e-01  & \first{5.40e-01} & \first{6.15e-02}  & \first{4.19e-01} & \first{3.47e-02}  & \first{2.04e-01} & \first{1.63e-02}  & \first{1.18e-01} & \first{7.75e-03}  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 7}\\$Q=50$}} & Smolyak & \first{5.74e-01} & 9.52e-02  & 5.51e-01 & 6.38e-02  & 5.00e-01 & 4.12e-02  & 3.37e-01 & 2.24e-02  & 2.08e-01 & 1.29e-02  &  &   &  & \\
 & LS-Uniform & 6.72e-01 & \first{7.97e-02}  & 7.04e-01 & 4.92e-02  & 2.33e+00 & 3.49e-02  & 1.17e+00 & 2.44e-02  & 1.85e+00 & 1.71e-02  &  &   &  & \\
 & LS-Chebyshev & 6.09e-01 & 8.44e-02  & \first{5.50e-01} & \first{4.78e-02}  & \first{4.07e-01} & \first{2.92e-02}  & \first{2.38e-01} & \first{1.64e-02}  & \first{1.49e-01} & \first{9.16e-03}  &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 8}\\$Q=50$}} & Smolyak & 1.27e+00 & 3.51e-01  & 9.95e-01 & 1.66e-01  & 4.83e-01 & 7.72e-02  & 3.37e-01 & 3.80e-02  &  &   &  &   &  & \\
 & LS-Uniform & \first{6.17e-01} & \first{5.79e-02}  & 6.54e-01 & \first{4.06e-02}  & 8.87e-01 & \first{2.64e-02}  & 1.06e+00 & 1.82e-02  &  &   &  &   &  & \\
 & LS-Chebyshev & 6.28e-01 & 6.48e-02  & \first{5.80e-01} & 5.10e-02  & \first{4.61e-01} & 2.74e-02  & \first{2.74e-01} & \first{1.46e-02}  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 9}\\$Q=50$}} & Smolyak & 8.64e-01 & 2.63e-01  & 8.49e-01 & 1.23e-01  & 7.20e-01 & 5.77e-02  & 3.17e-01 & 2.91e-02  &  &   &  &   &  & \\
 & LS-Uniform & \first{5.65e-01} & \first{6.83e-02}  & 1.42e+00 & \first{4.23e-02}  & 1.13e+00 & 2.90e-02  & 1.43e+00 & 1.83e-02  &  &   &  &   &  & \\
 & LS-Chebyshev & 6.50e-01 & 7.35e-02  & \first{5.48e-01} & 4.42e-02  & \first{4.36e-01} & \first{2.71e-02}  & \first{2.98e-01} & \first{1.59e-02}  &  &   &  &   &  & \\
\midrule
\multirow{3}{*}{\thead[l]{\textbf{Dim 10}\\$Q=50$}} & Smolyak & 1.21e+00 & 2.73e-01  & 9.42e-01 & 1.45e-01  & 8.41e-01 & 6.38e-02  & 4.33e-01 & 4.68e-02  &  &   &  &   &  & \\
 & LS-Uniform & \first{5.24e-01} & \first{6.01e-02}  & \first{4.85e-01} & \first{4.17e-02}  & 1.13e+00 & 2.66e-02  & 1.52e+00 & 1.71e-02  &  &   &  &   &  & \\
 & LS-Chebyshev & 6.88e-01 & 6.53e-02  & 5.97e-01 & 4.47e-02  & \first{4.92e-01} & \first{2.57e-02}  & \first{3.66e-01} & \first{1.55e-02}  &  &   &  &   &  & \\
\bottomrule
\end{tabular}


==> tables/dim2.tex <==
% Created with Python on 2025-06-22 19:31:16
% ..\results\final_results\low_dim\results_numerical_experiments.csv, dim=2, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & \first{5.71e-01} & \first{2.69e-01}  & \first{3.66e-01} & 1.55e-01  & 1.91e-01 & 7.14e-02  & 3.33e-02 & 9.39e-03  & 2.47e-03 & 6.16e-04  & 8.96e-06 & 2.44e-06  & 7.95e-09 & 2.19e-09\\
 & LS-Uniform & 3.51e+00 & 8.16e-01  & 5.12e+00 & 7.82e-01  & 3.56e+00 & 3.27e-01  & 8.19e+00 & 7.13e-01  & 3.15e+02 & 1.41e+01  & 1.93e+00 & 6.95e-02  & 3.03e+04 & 5.31e+02\\
 & LS-Chebyshev & 7.40e-01 & 2.89e-01  & 4.20e-01 & \first{1.35e-01}  & \first{1.87e-01} & \first{4.82e-02}  & \first{2.24e-02} & \first{6.11e-03}  & \first{1.52e-03} & \first{4.10e-04}  & \first{6.78e-06} & \first{1.50e-06}  & \first{7.27e-09} & \first{1.52e-09}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & \first{4.40e-02} & \first{1.49e-02}  & 2.22e-02 & 5.15e-03  & 1.10e-02 & 1.58e-03  & 5.23e-03 & 6.18e-04  & 2.68e-03 & 2.17e-04  & 1.46e-03 & 8.93e-05  & 7.65e-04 & 2.95e-05\\
 & LS-Uniform & 2.66e-01 & 7.08e-02  & 5.19e-01 & 7.51e-02  & 3.64e-01 & 3.24e-02  & 6.88e-01 & 6.27e-02  & 5.86e+02 & 2.69e+01  & 7.77e+02 & 3.19e+01  & 8.46e+08 & 1.50e+07\\
 & LS-Chebyshev & 4.80e-02 & 2.21e-02  & \first{1.84e-02} & \first{4.06e-03}  & \first{9.43e-03} & \first{1.45e-03}  & \first{4.69e-03} & \first{4.91e-04}  & \first{2.08e-03} & \first{1.85e-04}  & \first{1.20e-03} & \first{6.72e-05}  & \first{6.47e-04} & \first{2.71e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & \first{8.78e-03} & 4.52e-03  & 1.48e-03 & 5.81e-04  & 1.04e-04 & 3.31e-05  & 8.90e-07 & 2.61e-07  & \first{6.08e-09} & 1.75e-09  & \first{2.77e-13} & 8.54e-14  & \first{6.99e-15} & \first{9.35e-16}\\
 & LS-Uniform & 1.54e-02 & 3.24e-03  & 3.50e-03 & 5.50e-04  & 4.92e-04 & 5.98e-05  & 2.30e-04 & 2.04e-05  & 6.80e-04 & 3.05e-05  & 7.93e-08 & 2.70e-09  & 1.66e-02 & 2.92e-04\\
 & LS-Chebyshev & 8.88e-03 & \first{3.12e-03}  & \first{1.42e-03} & \first{4.44e-04}  & \first{8.77e-05} & \first{2.65e-05}  & \first{6.13e-07} & \first{1.70e-07}  & 6.32e-09 & \first{1.30e-09}  & 2.79e-13 & \first{5.98e-14}  & 1.39e-14 & 1.17e-15\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 4.73e+00 & \first{1.26e+00}  & 3.82e+00 & 1.08e+00  & 4.82e+00 & 8.42e-01  & 4.56e+00 & 6.75e-01  & 4.07e+00 & 4.26e-01  & 3.57e+00 & 3.28e-01  & 4.70e+00 & 2.16e-01\\
 & LS-Uniform & 3.46e+01 & 8.99e+00  & 7.48e+01 & 1.09e+01  & 6.02e+01 & 6.33e+00  & 3.07e+02 & 2.72e+01  & 6.62e+05 & 2.77e+04  & 1.79e+06 & 6.20e+04  & 6.27e+12 & 1.10e+11\\
 & LS-Chebyshev & \first{3.47e+00} & 1.27e+00  & \first{3.59e+00} & \first{7.15e-01}  & \first{4.24e+00} & \first{6.58e-01}  & \first{3.44e+00} & \first{4.35e-01}  & \first{3.25e+00} & \first{2.92e-01}  & \first{2.36e+00} & \first{2.04e-01}  & \first{2.92e+00} & \first{1.46e-01}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 5.81e-01 & 2.39e-01  & 3.51e-01 & 9.72e-02  & 1.18e-01 & 3.11e-02  & 2.17e-02 & 5.03e-03  & 1.93e-03 & 4.27e-04  & 7.40e-06 & 1.88e-06  & 6.31e-09 & 1.51e-09\\
 & LS-Uniform & 3.13e+00 & 7.97e-01  & 3.83e+00 & 5.77e-01  & 3.44e+00 & 2.92e-01  & 7.53e+00 & 6.71e-01  & 2.27e+02 & 1.11e+01  & 2.62e+00 & 8.97e-02  & 1.88e+04 & 3.30e+02\\
 & LS-Chebyshev & \first{4.84e-01} & \first{1.75e-01}  & \first{3.40e-01} & \first{8.12e-02}  & \first{6.74e-02} & \first{1.90e-02}  & \first{1.67e-02} & \first{3.37e-03}  & \first{1.19e-03} & \first{2.87e-04}  & \first{5.39e-06} & \first{1.22e-06}  & \first{5.51e-09} & \first{1.08e-09}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 1.09e-02 & 5.50e-03  & 2.80e-03 & \first{7.19e-04}  & \first{3.70e-04} & \first{7.25e-05}  & 4.84e-05 & 8.72e-06  & 3.65e-06 & 6.94e-07  & 1.36e-07 & 2.22e-08  & 2.19e-09 & 3.61e-10\\
 & LS-Uniform & \first{7.18e-03} & \first{1.52e-03}  & 5.70e-03 & 1.08e-03  & 1.33e-03 & 1.36e-04  & 3.29e-03 & 2.95e-04  & 1.07e-01 & 4.54e-03  & 3.88e-03 & 1.23e-04  & 2.26e+02 & 3.95e+00\\
 & LS-Chebyshev & 9.32e-03 & 4.52e-03  & \first{2.45e-03} & 9.90e-04  & 5.63e-04 & 9.85e-05  & \first{3.23e-05} & \first{7.11e-06}  & \first{3.08e-06} & \first{5.99e-07}  & \first{9.87e-08} & \first{2.00e-08}  & \first{2.06e-09} & \first{3.03e-10}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 6.00e-07 & 3.07e-07  & 6.46e-07 & 2.64e-07  & 7.78e-07 & 2.43e-07  & \first{8.85e-07} & 2.38e-07  & 9.21e-07 & 2.39e-07  & 1.21e-06 & 2.51e-07  & 1.25e-06 & 2.57e-07\\
 & LS-Uniform & 4.11e-06 & 1.04e-06  & 2.12e-05 & 3.07e-06  & 1.98e-05 & 2.30e-06  & 2.21e-04 & 2.00e-05  & 5.97e-01 & 2.69e-02  & 1.65e+00 & 5.52e-02  & 1.05e+07 & 1.84e+05\\
 & LS-Chebyshev & \first{5.59e-07} & \first{2.36e-07}  & \first{5.80e-07} & \first{1.97e-07}  & \first{7.30e-07} & \first{1.51e-07}  & 1.13e-06 & \first{1.47e-07}  & \first{8.96e-07} & \first{1.35e-07}  & \first{7.56e-07} & \first{1.28e-07}  & \first{7.61e-07} & \first{1.27e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & \first{3.97e-02} & 2.52e-02  & \first{2.12e-03} & 1.06e-03  & \first{4.48e-05} & 1.87e-05  & 9.42e-09 & 3.35e-09  & 5.70e-13 & 1.95e-13  & \first{9.44e-15} & \first{2.26e-15}  & \first{1.97e-14} & 3.65e-15\\
 & LS-Uniform & 1.69e-01 & 3.71e-02  & 9.31e-03 & 1.42e-03  & 1.97e-04 & 3.00e-05  & 2.71e-06 & 2.40e-07  & 7.01e-08 & 3.60e-09  & 7.54e-09 & 2.53e-10  & 5.83e-02 & 1.02e-03\\
 & LS-Chebyshev & 4.57e-02 & \first{1.78e-02}  & 2.53e-03 & \first{8.35e-04}  & 5.56e-05 & \first{1.33e-05}  & \first{7.69e-09} & \first{2.20e-09}  & \first{5.26e-13} & \first{1.40e-13}  & 3.43e-14 & 2.88e-15  & 2.81e-14 & \first{2.41e-15}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & \first{1.04e-03} & 6.17e-04  & \first{8.63e-05} & 3.77e-05  & 3.51e-06 & 1.24e-06  & 2.27e-08 & 7.41e-09  & 3.03e-11 & 8.55e-12  & \first{7.77e-15} & 2.15e-15  & \first{1.80e-14} & 3.63e-15\\
 & LS-Uniform & 4.27e-03 & 9.86e-04  & 4.65e-04 & 7.06e-05  & 1.99e-05 & 2.55e-06  & 7.28e-06 & 6.43e-07  & 3.65e-06 & 1.54e-07  & 3.19e-09 & 1.14e-10  & 2.16e-02 & 3.83e-04\\
 & LS-Chebyshev & 1.05e-03 & \first{5.03e-04}  & 1.01e-04 & \first{3.20e-05}  & \first{3.45e-06} & \first{8.70e-07}  & \first{1.81e-08} & \first{4.66e-09}  & \first{2.75e-11} & \first{6.14e-12}  & 1.55e-14 & \first{1.79e-15}  & 2.56e-14 & \first{1.73e-15}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 2.48e-01 & 1.05e-01  & \first{1.14e-01} & \first{3.85e-02}  & \first{6.89e-02} & 1.54e-02  & \first{3.42e-02} & 5.39e-03  & \first{2.39e-02} & 2.13e-03  & 1.18e-02 & 9.11e-04  & 7.14e-03 & 3.33e-04\\
 & LS-Uniform & 1.29e+00 & 3.18e-01  & 2.37e+00 & 3.45e-01  & 1.61e+00 & 1.67e-01  & 9.01e+00 & 7.85e-01  & 6.36e+03 & 2.86e+02  & 5.10e+03 & 1.54e+02  & 1.57e+10 & 2.75e+08\\
 & LS-Chebyshev & \first{1.94e-01} & \first{6.80e-02}  & 1.17e-01 & 4.08e-02  & 8.27e-02 & \first{1.14e-02}  & 4.75e-02 & \first{4.39e-03}  & 2.72e-02 & \first{1.68e-03}  & \first{1.14e-02} & \first{6.19e-04}  & \first{5.41e-03} & \first{2.38e-04}\\
\bottomrule
\end{tabular}


==> tables/dim3.tex <==
% Created with Python on 2025-06-22 19:31:16
% ..\results\final_results\low_dim\results_numerical_experiments.csv, dim=3, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 7.17e-01 & 2.93e-01  & \first{4.04e-01} & 1.43e-01  & 2.98e-01 & 8.74e-02  & 1.06e-01 & 2.28e-02  & 2.71e-02 & 5.99e-03  & 5.82e-03 & 9.34e-04  & 6.64e-04 & 1.12e-04\\
 & LS-Uniform & 2.47e+00 & 4.44e-01  & 1.33e+00 & 2.13e-01  & 8.83e-01 & 1.27e-01  & 1.37e+00 & 6.60e-02  & 7.62e-01 & 2.36e-02  & 1.42e+00 & 2.36e-02  & 4.05e+01 & 4.14e-01\\
 & LS-Chebyshev & \first{6.04e-01} & \first{1.77e-01}  & 5.85e-01 & \first{1.25e-01}  & \first{2.25e-01} & \first{5.65e-02}  & \first{7.17e-02} & \first{1.27e-02}  & \first{2.26e-02} & \first{2.86e-03}  & \first{3.83e-03} & \first{4.99e-04}  & \first{3.65e-04} & \first{5.14e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 4.54e-02 & 1.16e-02  & \first{1.57e-02} & \first{3.66e-03}  & 1.17e-02 & 1.68e-03  & \first{4.17e-03} & \first{4.94e-04}  & 3.22e-03 & 1.92e-04  & 1.32e-03 & 6.54e-05  & 6.66e-04 & 2.43e-05\\
 & LS-Uniform & 9.00e-02 & 1.51e-02  & 2.57e-02 & 4.94e-03  & 3.90e-02 & 2.89e-03  & 5.98e-02 & 2.11e-03  & 5.33e-02 & 1.49e-03  & 2.74e-01 & 4.00e-03  & 3.04e+01 & 3.14e-01\\
 & LS-Chebyshev & \first{3.30e-02} & \first{9.08e-03}  & 1.90e-02 & 4.16e-03  & \first{7.98e-03} & \first{1.43e-03}  & 5.42e-03 & 5.28e-04  & \first{2.11e-03} & \first{1.81e-04}  & \first{1.04e-03} & \first{6.09e-05}  & \first{5.69e-04} & \first{2.19e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 5.78e-02 & 1.58e-02  & 3.03e-02 & 5.80e-03  & 7.48e-03 & 1.46e-03  & 1.44e-03 & 2.55e-04  & 1.98e-04 & 2.96e-05  & 1.35e-05 & 2.06e-06  & 3.16e-07 & 4.17e-08\\
 & LS-Uniform & 7.11e-02 & \first{1.33e-02}  & \first{8.54e-03} & \first{1.65e-03}  & 6.77e-03 & \first{3.90e-04}  & 2.03e-03 & 1.02e-04  & 1.40e-03 & 3.23e-05  & 6.45e-04 & 1.13e-05  & 5.31e-03 & 5.72e-05\\
 & LS-Chebyshev & \first{3.38e-02} & 1.34e-02  & 9.19e-03 & 2.33e-03  & \first{2.31e-03} & 4.72e-04  & \first{3.68e-04} & \first{8.59e-05}  & \first{6.43e-05} & \first{1.07e-05}  & \first{5.24e-06} & \first{9.96e-07}  & \first{1.16e-07} & \first{2.05e-08}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 7.08e+00 & \first{1.73e+00}  & 1.11e+01 & \first{1.33e+00}  & 7.35e+00 & \first{1.03e+00}  & 9.26e+00 & 8.10e-01  & 9.99e+00 & 5.76e-01  & 8.40e+00 & 4.81e-01  & 1.07e+01 & 3.28e-01\\
 & LS-Uniform & 1.70e+01 & 3.87e+00  & 1.11e+01 & 1.66e+00  & 2.38e+01 & 1.67e+00  & 6.09e+01 & 2.57e+00  & 2.28e+02 & 5.88e+00  & 1.29e+03 & 2.70e+01  & 4.47e+05 & 4.45e+03\\
 & LS-Chebyshev & \first{6.97e+00} & 1.75e+00  & \first{6.09e+00} & 1.37e+00  & \first{5.86e+00} & 1.04e+00  & \first{7.10e+00} & \first{7.63e-01}  & \first{9.30e+00} & \first{5.30e-01}  & \first{6.44e+00} & \first{3.77e-01}  & \first{6.29e+00} & \first{2.59e-01}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 6.32e-01 & 2.17e-01  & 4.54e-01 & 9.92e-02  & \first{2.21e-01} & 3.99e-02  & 1.20e-01 & 1.72e-02  & 3.31e-02 & 5.10e-03  & 7.56e-03 & 8.69e-04  & 9.87e-04 & 1.01e-04\\
 & LS-Uniform & 1.66e+00 & 2.82e-01  & 7.59e-01 & 9.70e-02  & 7.69e-01 & 6.15e-02  & 6.03e-01 & 3.04e-02  & 6.14e-01 & 1.82e-02  & 9.04e-01 & 1.65e-02  & 5.56e+01 & 5.23e-01\\
 & LS-Chebyshev & \first{4.91e-01} & \first{1.28e-01}  & \first{3.66e-01} & \first{7.08e-02}  & 2.59e-01 & \first{2.74e-02}  & \first{9.23e-02} & \first{8.81e-03}  & \first{1.72e-02} & \first{2.09e-03}  & \first{2.88e-03} & \first{3.73e-04}  & \first{3.26e-04} & \first{4.46e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 2.27e-02 & 7.18e-03  & \first{3.20e-03} & 8.34e-04  & 3.76e-04 & 6.70e-05  & 2.58e-05 & 4.08e-06  & 2.11e-06 & 2.89e-07  & 1.44e-07 & 1.55e-08  & 6.94e-09 & 7.03e-10\\
 & LS-Uniform & 4.56e-02 & \first{6.02e-03}  & 4.19e-03 & \first{5.11e-04}  & 5.38e-04 & \first{4.27e-05}  & 5.83e-05 & 3.24e-06  & 3.39e-05 & 9.23e-07  & 1.81e-06 & 4.77e-08  & 6.44e-05 & 6.38e-07\\
 & LS-Chebyshev & \first{2.22e-02} & 6.15e-03  & 3.75e-03 & 1.06e-03  & \first{2.48e-04} & 7.25e-05  & \first{1.39e-05} & \first{3.05e-06}  & \first{9.97e-07} & \first{1.49e-07}  & \first{4.43e-08} & \first{6.60e-09}  & \first{2.38e-09} & \first{3.29e-10}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 9.86e-07 & 3.43e-07  & 1.25e-06 & 3.48e-07  & 1.44e-06 & 4.06e-07  & 1.80e-06 & 4.04e-07  & 2.24e-06 & 4.56e-07  & 2.73e-06 & 4.96e-07  & 3.06e-06 & 5.57e-07\\
 & LS-Uniform & 1.75e-06 & 3.59e-07  & 1.39e-06 & 2.47e-07  & 3.84e-06 & 3.29e-07  & 2.20e-05 & 8.19e-07  & 6.91e-05 & 1.80e-06  & 6.26e-04 & 1.09e-05  & 2.51e-01 & 2.57e-03\\
 & LS-Chebyshev & \first{6.16e-07} & \first{1.70e-07}  & \first{6.21e-07} & \first{1.59e-07}  & \first{6.35e-07} & \first{1.49e-07}  & \first{8.77e-07} & \first{1.46e-07}  & \first{9.05e-07} & \first{1.43e-07}  & \first{7.14e-07} & \first{1.38e-07}  & \first{7.36e-07} & \first{1.31e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & \first{4.60e-01} & \first{1.54e-01}  & \first{8.77e-02} & 3.12e-02  & 9.48e-03 & 3.25e-03  & 5.94e-04 & 1.77e-04  & 2.01e-05 & 4.99e-06  & 2.82e-07 & 6.29e-08  & 7.89e-11 & 1.71e-11\\
 & LS-Uniform & 1.12e+00 & 2.40e-01  & 1.43e-01 & \first{1.71e-02}  & 2.46e-02 & 1.93e-03  & 2.61e-03 & 1.24e-04  & 2.75e-04 & 7.39e-06  & 4.31e-05 & 7.63e-07  & 4.07e-06 & 3.67e-08\\
 & LS-Chebyshev & 6.95e-01 & 1.94e-01  & 9.86e-02 & 2.25e-02  & \first{8.00e-03} & \first{1.65e-03}  & \first{3.41e-04} & \first{7.41e-05}  & \first{1.38e-05} & \first{2.08e-06}  & \first{1.45e-07} & \first{2.87e-08}  & \first{4.98e-11} & \first{7.59e-12}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & 3.13e-03 & 1.28e-03  & 4.30e-04 & 1.57e-04  & 4.39e-05 & 1.56e-05  & 3.80e-06 & 1.11e-06  & 2.04e-07 & 4.59e-08  & 5.45e-09 & 9.51e-10  & 4.20e-11 & 7.27e-12\\
 & LS-Uniform & 9.12e-03 & 1.56e-03  & 5.74e-04 & \first{7.52e-05}  & 8.01e-05 & \first{8.11e-06}  & 1.44e-05 & 7.00e-07  & 2.28e-06 & 6.98e-08  & 9.92e-07 & 1.61e-08  & 1.46e-06 & 1.47e-08\\
 & LS-Chebyshev & \first{2.53e-03} & \first{1.04e-03}  & \first{4.28e-04} & 1.07e-04  & \first{3.82e-05} & 8.14e-06  & \first{2.77e-06} & \first{5.03e-07}  & \first{1.50e-07} & \first{2.05e-08}  & \first{2.57e-09} & \first{4.36e-10}  & \first{2.47e-11} & \first{3.23e-12}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 6.03e-01 & 1.98e-01  & 4.75e-01 & 8.99e-02  & 2.08e-01 & 4.03e-02  & 1.18e-01 & 1.54e-02  & 7.33e-02 & 6.44e-03  & \first{3.25e-02} & 2.47e-03  & 3.06e-02 & 9.64e-04\\
 & LS-Uniform & 1.09e+00 & 2.25e-01  & 4.55e-01 & 9.45e-02  & 4.46e-01 & 4.71e-02  & 9.80e-01 & 3.95e-02  & 2.31e+00 & 5.32e-02  & 1.25e+01 & 2.04e-01  & 2.03e+03 & 1.87e+01\\
 & LS-Chebyshev & \first{5.43e-01} & \first{1.53e-01}  & \first{3.43e-01} & \first{7.47e-02}  & \first{1.98e-01} & \first{3.08e-02}  & \first{9.31e-02} & \first{1.15e-02}  & \first{4.65e-02} & \first{4.66e-03}  & 3.39e-02 & \first{1.74e-03}  & \first{1.99e-02} & \first{6.82e-04}\\
\bottomrule
\end{tabular}


==> tables/dim4.tex <==
% Created with Python on 2025-06-22 19:31:16
% ..\results\final_results\low_dim\results_numerical_experiments.csv, dim=4, scales = [3, 4, 5, 6, 7, 8, 9]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8} & \multicolumn{2}{c}{Scale 9}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & \first{6.34e-01} & 1.76e-01  & 6.14e-01 & 1.27e-01  & 3.43e-01 & 8.48e-02  & 1.77e-01 & 4.25e-02  & 1.01e-01 & 1.36e-02  & 3.60e-02 & 3.18e-03  & 9.18e-03 & 8.39e-04\\
 & LS-Uniform & 1.40e+00 & 1.86e-01  & 1.15e+00 & 1.23e-01  & 1.10e+00 & 9.00e-02  & 7.49e-01 & 3.09e-02  & 4.71e-01 & 1.36e-02  & 3.80e-01 & 5.27e-03  & 1.39e+00 & 7.92e-03\\
 & LS-Chebyshev & 7.14e-01 & \first{1.56e-01}  & \first{5.03e-01} & \first{8.22e-02}  & \first{2.35e-01} & \first{4.60e-02}  & \first{1.18e-01} & \first{1.95e-02}  & \first{4.77e-02} & \first{6.20e-03}  & \first{1.29e-02} & \first{1.29e-03}  & \first{3.03e-03} & \first{2.47e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 3.06e-02 & \first{7.22e-03}  & 1.51e-02 & 3.07e-03  & 9.36e-03 & 1.03e-03  & 4.98e-03 & 4.84e-04  & 2.80e-03 & 1.64e-04  & 1.13e-03 & 5.73e-05  & 6.76e-04 & 1.81e-05\\
 & LS-Uniform & 6.82e-02 & 8.94e-03  & 3.20e-02 & 3.45e-03  & 1.81e-02 & 1.67e-03  & 1.81e-02 & 7.44e-04  & 1.05e-02 & 3.41e-04  & 2.03e-02 & 2.56e-04  & 2.02e-01 & 1.17e-03\\
 & LS-Chebyshev & \first{2.80e-02} & 7.87e-03  & \first{1.33e-02} & \first{2.72e-03}  & \first{7.72e-03} & \first{9.94e-04}  & \first{3.78e-03} & \first{3.61e-04}  & \first{2.23e-03} & \first{1.29e-04}  & \first{8.58e-04} & \first{4.69e-05}  & \first{4.37e-04} & \first{1.74e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 1.62e-01 & 2.46e-02  & 8.14e-02 & 1.29e-02  & 5.39e-02 & 5.69e-03  & 1.89e-02 & 2.32e-03  & 6.42e-03 & 6.42e-04  & 1.60e-03 & 1.37e-04  & 3.10e-04 & 2.20e-05\\
 & LS-Uniform & \first{9.45e-02} & \first{1.05e-02}  & 6.71e-02 & \first{4.08e-03}  & 2.02e-02 & \first{1.08e-03}  & 8.63e-03 & \first{2.20e-04}  & 6.64e-03 & \first{8.51e-05}  & 1.53e-03 & \first{2.20e-05}  & 3.41e-03 & 2.36e-05\\
 & LS-Chebyshev & 1.14e-01 & 2.12e-02  & \first{4.08e-02} & 7.06e-03  & \first{1.23e-02} & 2.09e-03  & \first{2.51e-03} & 4.46e-04  & \first{7.63e-04} & 1.16e-04  & \first{1.81e-04} & 2.37e-05  & \first{3.76e-05} & \first{4.59e-06}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 2.40e+01 & \first{3.96e+00}  & 3.61e+01 & 3.29e+00  & 3.36e+01 & 2.59e+00  & 2.92e+01 & 1.96e+00  & 2.90e+01 & 1.40e+00  & 3.14e+01 & \first{1.04e+00}  & 3.13e+01 & 7.74e-01\\
 & LS-Uniform & \first{2.27e+01} & 4.40e+00  & \first{2.68e+01} & \first{3.24e+00}  & 5.96e+01 & 3.33e+00  & 4.40e+01 & 3.05e+00  & 1.19e+02 & 2.99e+00  & 5.04e+02 & 5.85e+00  & 1.13e+04 & 6.19e+01\\
 & LS-Chebyshev & 2.49e+01 & 5.10e+00  & 2.99e+01 & 3.74e+00  & \first{2.35e+01} & \first{2.33e+00}  & \first{2.49e+01} & \first{1.78e+00}  & \first{1.98e+01} & \first{1.33e+00}  & \first{1.92e+01} & 1.07e+00  & \first{1.81e+01} & \first{7.73e-01}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 6.42e-01 & 1.75e-01  & 4.80e-01 & 8.93e-02  & 3.24e-01 & 4.70e-02  & 1.98e-01 & 2.07e-02  & 1.04e-01 & 7.66e-03  & 3.94e-02 & 3.36e-03  & 9.55e-03 & 9.78e-04\\
 & LS-Uniform & 8.28e-01 & 1.35e-01  & 1.03e+00 & 7.53e-02  & 1.01e+00 & 5.19e-02  & 1.30e+00 & 2.99e-02  & 3.52e-01 & 9.70e-03  & 3.41e-01 & 4.48e-03  & 1.31e+00 & 7.83e-03\\
 & LS-Chebyshev & \first{5.90e-01} & \first{9.71e-02}  & \first{4.10e-01} & \first{5.53e-02}  & \first{2.14e-01} & \first{2.71e-02}  & \first{1.08e-01} & \first{1.13e-02}  & \first{3.82e-02} & \first{3.73e-03}  & \first{1.68e-02} & \first{1.06e-03}  & \first{5.26e-03} & \first{2.87e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & \first{8.36e-02} & 2.25e-02  & 3.02e-02 & 5.43e-03  & 9.51e-03 & 1.15e-03  & 2.33e-03 & 2.05e-04  & 5.75e-04 & 3.13e-05  & 9.34e-05 & 4.02e-06  & 1.07e-05 & 4.43e-07\\
 & LS-Uniform & 1.03e-01 & \first{1.27e-02}  & \first{2.90e-02} & \first{2.50e-03}  & 1.35e-02 & \first{5.94e-04}  & 5.62e-03 & \first{1.27e-04}  & 8.25e-04 & \first{1.35e-05}  & 1.25e-04 & \first{2.09e-06}  & 1.18e-04 & 9.63e-07\\
 & LS-Chebyshev & 1.03e-01 & 3.31e-02  & 2.91e-02 & 7.40e-03  & \first{5.91e-03} & 1.19e-03  & \first{8.35e-04} & 2.12e-04  & \first{1.92e-04} & 2.86e-05  & \first{1.68e-05} & 2.98e-06  & \first{3.13e-06} & \first{2.92e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 1.65e-06 & 4.23e-07  & 2.09e-06 & 5.18e-07  & 2.63e-06 & 5.34e-07  & 4.27e-06 & 6.76e-07  & 4.65e-06 & 7.53e-07  & 5.81e-06 & 9.02e-07  & 6.78e-06 & 1.02e-06\\
 & LS-Uniform & 1.45e-06 & 1.96e-07  & 1.48e-06 & 1.88e-07  & 3.94e-06 & 2.58e-07  & 6.85e-06 & 2.78e-07  & 1.39e-05 & 4.01e-07  & 7.98e-05 & 9.71e-07  & 2.00e-03 & 1.32e-05\\
 & LS-Chebyshev & \first{6.18e-07} & \first{1.75e-07}  & \first{7.31e-07} & \first{1.71e-07}  & \first{7.82e-07} & \first{1.49e-07}  & \first{8.05e-07} & \first{1.38e-07}  & \first{7.41e-07} & \first{1.39e-07}  & \first{7.44e-07} & \first{1.37e-07}  & \first{7.95e-07} & \first{1.37e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & \first{1.73e+00} & \first{3.71e-01}  & \first{6.40e-01} & 1.27e-01  & 1.47e-01 & 3.57e-02  & 2.27e-02 & 5.91e-03  & 2.29e-03 & 5.81e-04  & 1.65e-04 & 3.36e-05  & 6.86e-06 & 1.18e-06\\
 & LS-Uniform & 2.57e+00 & 4.73e-01  & 1.12e+00 & \first{1.18e-01}  & 3.74e-01 & \first{2.14e-02}  & 8.01e-02 & \first{2.14e-03}  & 6.46e-03 & 1.75e-04  & 8.88e-04 & 1.58e-05  & 4.14e-04 & 3.25e-06\\
 & LS-Chebyshev & 2.99e+00 & 6.38e-01  & 1.04e+00 & 2.00e-01  & \first{1.19e-01} & 2.60e-02  & \first{1.21e-02} & 2.29e-03  & \first{1.06e-03} & \first{1.60e-04}  & \first{6.54e-05} & \first{8.09e-06}  & \first{2.32e-06} & \first{2.84e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & 7.49e-03 & 1.86e-03  & 1.17e-03 & 2.97e-04  & 1.95e-04 & 4.47e-05  & 2.37e-05 & 5.74e-06  & 2.36e-06 & 5.40e-07  & 2.12e-07 & 3.75e-08  & 1.43e-08 & 1.83e-09\\
 & LS-Uniform & 7.81e-03 & \first{1.60e-03}  & 3.43e-03 & \first{1.92e-04}  & 3.59e-04 & \first{2.02e-05}  & 7.85e-05 & 2.11e-06  & 5.35e-06 & \first{1.28e-07}  & 9.85e-07 & 1.64e-08  & 8.28e-07 & 5.47e-09\\
 & LS-Chebyshev & \first{6.16e-03} & 2.04e-03  & \first{1.13e-03} & 2.97e-04  & \first{1.08e-04} & 2.55e-05  & \first{1.09e-05} & \first{2.09e-06}  & \first{1.10e-06} & 1.52e-07  & \first{7.08e-08} & \first{9.16e-09}  & \first{4.38e-09} & \first{4.44e-10}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 1.70e+00 & 3.83e-01  & 1.30e+00 & 2.05e-01  & 7.02e-01 & 8.54e-02  & 3.40e-01 & 3.77e-02  & 2.32e-01 & 1.58e-02  & 1.24e-01 & 6.54e-03  & 4.96e-02 & 2.72e-03\\
 & LS-Uniform & 2.06e+00 & \first{2.88e-01}  & 1.16e+00 & 1.47e-01  & 1.02e+00 & 9.01e-02  & 1.02e+00 & 3.59e-02  & 6.19e-01 & 2.10e-02  & 2.03e+00 & 2.22e-02  & 1.28e+01 & 8.16e-02\\
 & LS-Chebyshev & \first{9.88e-01} & 3.53e-01  & \first{5.30e-01} & \first{1.27e-01}  & \first{2.94e-01} & \first{5.48e-02}  & \first{2.30e-01} & \first{2.59e-02}  & \first{1.19e-01} & \first{9.61e-03}  & \first{6.77e-02} & \first{3.92e-03}  & \first{4.23e-02} & \first{1.60e-03}\\
\bottomrule
\end{tabular}


==> tables/dim5.tex <==
% Created with Python on 2025-06-22 19:31:16
% ..\results\final_results\low_dim\results_numerical_experiments.csv, dim=5, scales = [3, 4, 5, 6, 7, 8]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7} & \multicolumn{2}{c}{Scale 8}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 6.58e-01 & 2.19e-01  & 6.01e-01 & 9.79e-02  & 3.44e-01 & 6.83e-02  & 2.10e-01 & 3.35e-02  & 1.14e-01 & 1.41e-02  & 5.70e-02 & 5.97e-03\\
 & LS-Uniform & 9.73e-01 & 1.46e-01  & 1.01e+00 & 8.20e-02  & 1.05e+00 & 5.14e-02  & 1.27e+00 & 2.76e-02  & 1.21e+00 & 1.35e-02  & 8.27e-01 & 5.01e-03\\
 & LS-Chebyshev & \first{5.92e-01} & \first{1.11e-01}  & \first{4.63e-01} & \first{6.17e-02}  & \first{2.71e-01} & \first{3.30e-02}  & \first{1.56e-01} & \first{1.79e-02}  & \first{6.91e-02} & \first{7.30e-03}  & \first{2.88e-02} & \first{2.14e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 3.24e-02 & \first{6.00e-03}  & 1.60e-02 & 2.55e-03  & 8.41e-03 & 8.77e-04  & 3.68e-03 & 3.27e-04  & 2.18e-03 & 1.31e-04  & 8.40e-04 & 4.66e-05\\
 & LS-Uniform & 3.47e-02 & 7.08e-03  & 2.26e-02 & 3.14e-03  & 1.63e-02 & 1.17e-03  & 1.36e-02 & 4.58e-04  & 6.62e-03 & 2.06e-04  & 7.40e-03 & 1.04e-04\\
 & LS-Chebyshev & \first{2.80e-02} & 6.25e-03  & \first{1.45e-02} & \first{2.23e-03}  & \first{6.89e-03} & \first{7.64e-04}  & \first{3.13e-03} & \first{2.85e-04}  & \first{1.42e-03} & \first{1.02e-04}  & \first{7.27e-04} & \first{3.74e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 1.56e-01 & 2.07e-02  & 2.47e-01 & 1.57e-02  & 1.25e-01 & 1.07e-02  & 7.94e-02 & 5.60e-03  & 3.98e-02 & 2.24e-03  & 1.65e-02 & 1.01e-03\\
 & LS-Uniform & \first{4.36e-02} & \first{5.32e-03}  & 1.21e-01 & \first{4.43e-03}  & 6.88e-02 & \first{1.49e-03}  & 1.91e-02 & \first{4.54e-04}  & 1.51e-02 & \first{1.62e-04}  & 1.39e-02 & \first{6.86e-05}\\
 & LS-Chebyshev & 1.51e-01 & 3.78e-02  & \first{5.15e-02} & 1.30e-02  & \first{2.44e-02} & 4.49e-03  & \first{8.78e-03} & 1.20e-03  & \first{2.72e-03} & 3.57e-04  & \first{1.25e-03} & 1.15e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & \first{4.92e+01} & 7.98e+00  & \first{5.33e+01} & \first{5.79e+00}  & 5.18e+01 & \first{4.33e+00}  & 6.96e+01 & \first{3.59e+00}  & 7.05e+01 & \first{2.61e+00}  & 7.93e+01 & \first{1.92e+00}\\
 & LS-Uniform & 5.05e+01 & 9.25e+00  & 6.57e+01 & 7.68e+00  & 7.06e+01 & 5.40e+00  & 1.27e+02 & 4.79e+00  & 1.84e+02 & 5.00e+00  & 3.20e+02 & 4.61e+00\\
 & LS-Chebyshev & 4.93e+01 & \first{7.89e+00}  & 6.37e+01 & 6.57e+00  & \first{5.03e+01} & 4.62e+00  & \first{5.36e+01} & 3.66e+00  & \first{4.26e+01} & 2.71e+00  & \first{4.79e+01} & 2.04e+00\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 6.92e-01 & 1.18e-01  & 5.59e-01 & 7.81e-02  & 4.13e-01 & 6.14e-02  & 2.36e-01 & 2.39e-02  & 1.11e-01 & 8.48e-03  & 4.50e-02 & 3.53e-03\\
 & LS-Uniform & \first{5.93e-01} & 9.65e-02  & 1.05e+00 & 8.73e-02  & 1.11e+00 & 3.93e-02  & 6.08e-01 & 1.70e-02  & 7.12e-01 & 1.01e-02  & 8.05e-01 & 4.63e-03\\
 & LS-Chebyshev & 6.71e-01 & \first{8.36e-02}  & \first{4.57e-01} & \first{5.40e-02}  & \first{2.64e-01} & \first{2.75e-02}  & \first{1.49e-01} & \first{1.25e-02}  & \first{7.31e-02} & \first{4.62e-03}  & \first{2.69e-02} & \first{1.46e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & \first{2.20e-02} & 5.62e-03  & 5.79e-03 & 9.61e-04  & 1.28e-03 & 1.42e-04  & 1.84e-04 & 1.79e-05  & 3.08e-05 & 1.64e-06  & 3.21e-06 & 1.30e-07\\
 & LS-Uniform & 3.12e-02 & \first{4.22e-03}  & 6.55e-03 & \first{5.47e-04}  & 1.46e-03 & \first{6.65e-05}  & 3.74e-04 & \first{8.14e-06}  & 5.12e-05 & \first{9.06e-07}  & 4.22e-06 & \first{6.83e-08}\\
 & LS-Chebyshev & 2.24e-02 & 8.09e-03  & \first{4.78e-03} & 7.64e-04  & \first{5.93e-04} & 1.02e-04  & \first{6.03e-05} & 1.21e-05  & \first{1.06e-05} & 1.30e-06  & \first{1.13e-06} & 1.03e-07\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 1.86e-06 & 5.11e-07  & 2.72e-06 & 6.52e-07  & 4.71e-06 & 7.87e-07  & 6.50e-06 & 9.68e-07  & 9.92e-06 & 1.21e-06  & 1.06e-05 & 1.47e-06\\
 & LS-Uniform & 1.13e-06 & \first{1.76e-07}  & 1.67e-06 & 1.92e-07  & 3.03e-06 & 1.90e-07  & 7.35e-06 & 2.27e-07  & 1.06e-05 & 2.99e-07  & 3.63e-05 & 4.34e-07\\
 & LS-Chebyshev & \first{8.94e-07} & 1.77e-07  & \first{7.39e-07} & \first{1.51e-07}  & \first{7.12e-07} & \first{1.48e-07}  & \first{8.82e-07} & \first{1.48e-07}  & \first{7.43e-07} & \first{1.42e-07}  & \first{8.45e-07} & \first{1.43e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & \first{3.16e+00} & \first{6.35e-01}  & \first{1.96e+00} & \first{3.25e-01}  & 8.12e-01 & 1.37e-01  & 1.98e-01 & 3.66e-02  & 3.98e-02 & 8.11e-03  & 5.71e-03 & 1.11e-03\\
 & LS-Uniform & 7.47e+00 & 8.13e-01  & 3.53e+00 & 3.44e-01  & 1.87e+00 & \first{8.95e-02}  & 1.44e+00 & \first{2.34e-02}  & 2.71e-01 & 3.65e-03  & 3.33e-02 & 3.65e-04\\
 & LS-Chebyshev & 3.93e+00 & 1.02e+00  & 2.23e+00 & 5.68e-01  & \first{7.15e-01} & 1.66e-01  & \first{1.56e-01} & 3.08e-02  & \first{2.59e-02} & \first{3.41e-03}  & \first{2.31e-03} & \first{2.90e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & 9.44e-03 & 1.67e-03  & \first{1.51e-03} & 3.14e-04  & \first{3.04e-04} & 5.54e-05  & 4.84e-05 & 8.17e-06  & 6.45e-06 & 1.09e-06  & 8.07e-07 & 1.28e-07\\
 & LS-Uniform & \first{7.66e-03} & \first{1.25e-03}  & 2.88e-03 & \first{2.89e-04}  & 1.22e-03 & \first{3.95e-05}  & 2.85e-04 & 5.28e-06  & 2.59e-05 & 4.58e-07  & 5.06e-06 & 4.72e-08\\
 & LS-Chebyshev & 9.17e-03 & 2.19e-03  & 2.11e-03 & 3.67e-04  & 3.62e-04 & 4.76e-05  & \first{4.66e-05} & \first{4.97e-06}  & \first{4.87e-06} & \first{4.37e-07}  & \first{3.99e-07} & \first{3.50e-08}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 2.92e+00 & 6.22e-01  & 2.40e+00 & 3.19e-01  & 1.80e+00 & 1.67e-01  & 8.60e-01 & 8.16e-02  & 4.45e-01 & 3.77e-02  & 3.11e-01 & 1.70e-02\\
 & LS-Uniform & 2.32e+00 & \first{4.64e-01}  & 2.05e+00 & \first{2.24e-01}  & 1.88e+00 & 1.10e-01  & 1.40e+00 & 5.16e-02  & 9.51e-01 & 2.92e-02  & 1.43e+00 & 1.86e-02\\
 & LS-Chebyshev & \first{2.23e+00} & 6.17e-01  & \first{1.26e+00} & 2.63e-01  & \first{9.49e-01} & \first{1.02e-01}  & \first{3.85e-01} & \first{4.24e-02}  & \first{1.92e-01} & \first{1.79e-02}  & \first{1.58e-01} & \first{7.57e-03}\\
\bottomrule
\end{tabular}


==> tables/dim6.tex <==
% Created with Python on 2025-06-22 19:31:16
% ..\results\final_results\low_dim\results_numerical_experiments.csv, dim=6, scales = [3, 4, 5, 6, 7]
\begin{tabular}{ll|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 7.63e-01 & 1.60e-01  & 5.55e-01 & 1.10e-01  & 4.59e-01 & 6.18e-02  & 3.38e-01 & 2.96e-02  & 1.88e-01 & 1.22e-02\\
 & LS-Uniform & 9.79e-01 & \first{1.16e-01}  & 1.28e+00 & 7.12e-02  & 7.96e-01 & 3.72e-02  & 8.97e-01 & 2.03e-02  & 7.20e-01 & 1.21e-02\\
 & LS-Chebyshev & \first{7.01e-01} & 1.23e-01  & \first{5.40e-01} & \first{6.15e-02}  & \first{4.19e-01} & \first{3.47e-02}  & \first{2.04e-01} & \first{1.63e-02}  & \first{1.18e-01} & \first{7.75e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & \first{2.46e-02} & \first{5.14e-03}  & \first{1.37e-02} & \first{1.90e-03}  & 7.75e-03 & 7.71e-04  & \first{3.31e-03} & 3.30e-04  & 1.78e-03 & 1.10e-04\\
 & LS-Uniform & 3.23e-02 & 5.40e-03  & 1.68e-02 & 2.30e-03  & 1.09e-02 & 9.02e-04  & 1.16e-02 & 3.73e-04  & 5.36e-03 & 1.60e-04\\
 & LS-Chebyshev & 2.47e-02 & 5.55e-03  & 1.38e-02 & 2.15e-03  & \first{6.24e-03} & \first{7.46e-04}  & 3.75e-03 & \first{2.59e-04}  & \first{1.58e-03} & \first{9.33e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 2.46e-02 & 2.99e-03  & 1.80e-01 & 8.18e-03  & 2.53e-01 & 8.59e-03  & 1.44e-01 & 5.65e-03  & 1.07e-01 & 4.41e-03\\
 & LS-Uniform & \first{2.41e-02} & \first{2.87e-03}  & 1.03e-01 & \first{2.87e-03}  & 7.82e-02 & \first{1.19e-03}  & 7.77e-02 & \first{6.63e-04}  & 2.75e-02 & \first{1.54e-04}\\
 & LS-Chebyshev & 7.62e-02 & 2.10e-02  & \first{6.89e-02} & 9.41e-03  & \first{2.50e-02} & 4.35e-03  & \first{1.75e-02} & 2.11e-03  & \first{8.05e-03} & 7.55e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 1.19e+02 & \first{1.29e+01}  & 1.67e+02 & 1.14e+01  & 1.38e+02 & \first{7.79e+00}  & 1.31e+02 & \first{5.95e+00}  & 1.75e+02 & \first{4.24e+00}\\
 & LS-Uniform & \first{1.12e+02} & 1.38e+01  & \first{1.27e+02} & \first{1.13e+01}  & 1.42e+02 & 9.37e+00  & 2.74e+02 & 8.39e+00  & 3.37e+02 & 7.03e+00\\
 & LS-Chebyshev & 1.45e+02 & 4.46e+01  & 1.37e+02 & 2.16e+01  & \first{1.01e+02} & 1.07e+01  & \first{1.08e+02} & 7.36e+00  & \first{1.01e+02} & 5.33e+00\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & \first{5.74e-01} & 1.63e-01  & 5.92e-01 & 8.11e-02  & 4.88e-01 & 4.00e-02  & 3.05e-01 & 2.13e-02  & 1.95e-01 & 8.53e-03\\
 & LS-Uniform & 7.27e-01 & 1.11e-01  & 6.73e-01 & 5.92e-02  & 9.13e-01 & 3.42e-02  & 1.40e+00 & 1.85e-02  & 8.09e-01 & 8.80e-03\\
 & LS-Chebyshev & 6.30e-01 & \first{9.58e-02}  & \first{5.16e-01} & \first{5.49e-02}  & \first{3.05e-01} & \first{2.89e-02}  & \first{1.69e-01} & \first{1.34e-02}  & \first{9.95e-02} & \first{5.00e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & \first{9.67e-02} & 2.23e-02  & 3.33e-02 & 4.40e-03  & 6.61e-03 & 6.20e-04  & 1.20e-03 & 1.12e-04  & 3.06e-04 & 1.70e-05\\
 & LS-Uniform & 1.24e-01 & \first{1.62e-02}  & 2.86e-02 & \first{3.13e-03}  & 8.01e-03 & \first{3.48e-04}  & 4.62e-03 & \first{5.96e-05}  & 5.21e-04 & \first{8.06e-06}\\
 & LS-Chebyshev & 1.04e-01 & 2.51e-02  & \first{2.43e-02} & 5.71e-03  & \first{5.20e-03} & 9.03e-04  & \first{7.05e-04} & 9.40e-05  & \first{1.05e-04} & 1.40e-05\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 2.98e-06 & 6.30e-07  & 4.34e-06 & 9.47e-07  & 8.13e-06 & 1.08e-06  & 1.08e-05 & 1.42e-06  & 1.53e-05 & 1.84e-06\\
 & LS-Uniform & 1.09e-06 & \first{1.62e-07}  & 2.38e-06 & \first{1.61e-07}  & 2.97e-06 & 1.74e-07  & 8.25e-06 & 2.14e-07  & 1.15e-05 & 2.52e-07\\
 & LS-Chebyshev & \first{7.27e-07} & 1.73e-07  & \first{7.92e-07} & 1.63e-07  & \first{7.93e-07} & \first{1.57e-07}  & \first{8.30e-07} & \first{1.49e-07}  & \first{9.26e-07} & \first{1.49e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & 8.22e+00 & \first{9.31e-01}  & 5.60e+00 & \first{5.52e-01}  & 2.34e+00 & 2.79e-01  & 9.08e-01 & 1.15e-01  & 2.67e-01 & 3.63e-02\\
 & LS-Uniform & 7.38e+00 & 9.44e-01  & 7.51e+00 & 6.52e-01  & 6.52e+00 & \first{2.55e-01}  & 4.17e+00 & \first{8.02e-02}  & 1.47e+00 & \first{1.98e-02}\\
 & LS-Chebyshev & \first{5.68e+00} & 1.28e+00  & \first{3.63e+00} & 9.07e-01  & \first{2.31e+00} & 4.57e-01  & \first{7.52e-01} & 1.33e-01  & \first{1.63e-01} & 2.75e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & \first{9.11e-03} & \first{1.58e-03}  & \first{2.55e-03} & 2.81e-04  & \first{3.29e-04} & 4.74e-05  & \first{5.42e-05} & 7.37e-06  & \first{8.00e-06} & 1.14e-06\\
 & LS-Uniform & 1.96e-02 & 1.84e-03  & 4.56e-03 & \first{2.72e-04}  & 7.60e-04 & \first{2.89e-05}  & 3.73e-04 & \first{4.33e-06}  & 8.31e-05 & \first{6.08e-07}\\
 & LS-Chebyshev & 1.50e-02 & 2.60e-03  & 3.33e-03 & 3.93e-04  & 4.72e-04 & 4.64e-05  & 8.14e-05 & 5.99e-06  & 1.09e-05 & 6.35e-07\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 6.46e+00 & 9.21e-01  & 6.57e+00 & 5.98e-01  & 4.06e+00 & 3.12e-01  & 1.86e+00 & 1.60e-01  & 1.18e+00 & 7.76e-02\\
 & LS-Uniform & \first{3.24e+00} & \first{5.50e-01}  & 4.09e+00 & \first{2.63e-01}  & 2.21e+00 & \first{1.33e-01}  & 1.91e+00 & \first{7.53e-02}  & 1.10e+00 & 3.85e-02\\
 & LS-Chebyshev & 3.78e+00 & 8.72e-01  & \first{3.10e+00} & 3.98e-01  & \first{1.66e+00} & 1.80e-01  & \first{7.14e-01} & 7.62e-02  & \first{4.85e-01} & \first{3.25e-02}\\
\bottomrule
\end{tabular}


==> tables/dim7.tex <==
% Created with Python on 2025-06-22 19:31:16
% ..\results\final_results\low_dim\results_numerical_experiments.csv, dim=7, scales = [3, 4, 5, 6, 7]
\begin{tabular}{ll|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6} & \multicolumn{2}{c}{Scale 7}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & \first{5.74e-01} & 9.52e-02  & 5.51e-01 & 6.38e-02  & 5.00e-01 & 4.12e-02  & 3.37e-01 & 2.24e-02  & 2.08e-01 & 1.29e-02\\
 & LS-Uniform & 6.72e-01 & \first{7.97e-02}  & 7.04e-01 & 4.92e-02  & 2.33e+00 & 3.49e-02  & 1.17e+00 & 2.44e-02  & 1.85e+00 & 1.71e-02\\
 & LS-Chebyshev & 6.09e-01 & 8.44e-02  & \first{5.50e-01} & \first{4.78e-02}  & \first{4.07e-01} & \first{2.92e-02}  & \first{2.38e-01} & \first{1.64e-02}  & \first{1.49e-01} & \first{9.16e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 3.05e-02 & 6.08e-03  & 1.22e-02 & 1.95e-03  & 7.33e-03 & 7.47e-04  & 4.32e-03 & 2.83e-04  & 1.78e-03 & 1.08e-04\\
 & LS-Uniform & 3.32e-02 & \first{5.12e-03}  & 1.91e-02 & 1.94e-03  & 1.35e-02 & 8.28e-04  & 1.17e-02 & 3.24e-04  & 6.02e-03 & 1.35e-04\\
 & LS-Chebyshev & \first{2.13e-02} & 5.31e-03  & \first{1.13e-02} & \first{1.78e-03}  & \first{5.84e-03} & \first{6.34e-04}  & \first{2.99e-03} & \first{2.35e-04}  & \first{1.74e-03} & \first{8.47e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 1.68e-02 & 1.40e-03  & 3.63e-02 & 2.11e-03  & 1.06e-01 & 3.14e-03  & 1.36e-01 & 3.50e-03  & 1.45e-01 & 3.08e-03\\
 & LS-Uniform & \first{1.49e-02} & \first{7.53e-04}  & \first{2.17e-02} & \first{4.91e-04}  & 3.75e-02 & \first{4.28e-04}  & 6.35e-02 & \first{4.00e-04}  & 4.31e-02 & \first{1.72e-04}\\
 & LS-Chebyshev & 3.82e-02 & 1.26e-02  & 2.98e-02 & 4.26e-03  & \first{2.76e-02} & 3.68e-03  & \first{1.62e-02} & 1.41e-03  & \first{9.84e-03} & 6.83e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 3.16e+02 & \first{3.26e+01}  & 3.15e+02 & \first{2.22e+01}  & 3.21e+02 & \first{1.78e+01}  & 2.93e+02 & \first{1.29e+01}  & 3.78e+02 & \first{9.44e+00}\\
 & LS-Uniform & 5.30e+02 & 3.27e+01  & 3.72e+02 & 2.34e+01  & 4.73e+02 & 1.82e+01  & 3.96e+02 & 1.51e+01  & 7.70e+02 & 1.33e+01\\
 & LS-Chebyshev & \first{2.55e+02} & 5.16e+01  & \first{2.21e+02} & 4.58e+01  & \first{2.45e+02} & 2.90e+01  & \first{2.71e+02} & 2.14e+01  & \first{3.10e+02} & 1.54e+01\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 8.19e-01 & 8.12e-02  & 6.49e-01 & 9.23e-02  & 5.66e-01 & 3.82e-02  & 4.27e-01 & 1.90e-02  & 2.89e-01 & 1.24e-02\\
 & LS-Uniform & \first{6.16e-01} & \first{6.05e-02}  & 6.97e-01 & 3.99e-02  & 9.40e-01 & 2.56e-02  & 1.90e+00 & 1.90e-02  & 1.08e+00 & 9.96e-03\\
 & LS-Chebyshev & 6.45e-01 & 7.00e-02  & \first{5.18e-01} & \first{3.70e-02}  & \first{3.33e-01} & \first{2.22e-02}  & \first{2.45e-01} & \first{1.22e-02}  & \first{1.38e-01} & \first{6.03e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 2.12e-01 & 3.39e-02  & \first{5.98e-02} & 9.17e-03  & 1.69e-02 & 1.66e-03  & 5.02e-03 & 3.01e-04  & 1.22e-03 & 5.36e-05\\
 & LS-Uniform & 2.46e-01 & \first{1.96e-02}  & 6.28e-02 & \first{5.51e-03}  & 2.67e-02 & \first{9.99e-04}  & 5.91e-03 & \first{1.25e-04}  & 1.96e-03 & \first{1.69e-05}\\
 & LS-Chebyshev & \first{1.69e-01} & 4.66e-02  & 7.30e-02 & 1.61e-02  & \first{1.53e-02} & 2.97e-03  & \first{2.32e-03} & 3.96e-04  & \first{4.64e-04} & 5.06e-05\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 3.89e-06 & 7.36e-07  & 7.43e-06 & 1.18e-06  & 1.29e-05 & 1.44e-06  & 1.83e-05 & 1.99e-06  & 2.80e-05 & 2.59e-06\\
 & LS-Uniform & 1.03e-06 & \first{1.40e-07}  & 2.18e-06 & \first{1.50e-07}  & 4.86e-06 & 1.72e-07  & 7.99e-06 & 1.94e-07  & 1.59e-05 & 2.34e-07\\
 & LS-Chebyshev & \first{6.94e-07} & 1.70e-07  & \first{8.48e-07} & 1.70e-07  & \first{9.50e-07} & \first{1.58e-07}  & \first{1.07e-06} & \first{1.55e-07}  & \first{1.12e-06} & \first{1.56e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & 1.07e+01 & 1.22e+00  & 9.41e+00 & 9.07e-01  & 5.95e+00 & 5.23e-01  & 3.24e+00 & 2.56e-01  & 1.26e+00 & 1.05e-01\\
 & LS-Uniform & 1.10e+01 & \first{1.12e+00}  & 1.37e+01 & \first{7.95e-01}  & 2.03e+01 & \first{4.98e-01}  & 1.55e+01 & \first{2.40e-01}  & 8.97e+00 & \first{7.95e-02}\\
 & LS-Chebyshev & \first{6.02e+00} & 1.39e+00  & \first{4.89e+00} & 1.17e+00  & \first{4.09e+00} & 7.94e-01  & \first{2.75e+00} & 4.25e-01  & \first{8.34e-01} & 1.35e-01\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & \first{8.35e-03} & \first{1.62e-03}  & \first{2.36e-03} & 3.25e-04  & \first{5.73e-04} & 6.41e-05  & \first{1.18e-04} & 1.13e-05  & \first{2.85e-05} & 1.87e-06\\
 & LS-Uniform & 1.49e-02 & 1.82e-03  & 4.91e-03 & \first{3.00e-04}  & 8.68e-04 & \first{4.60e-05}  & 3.77e-04 & \first{6.61e-06}  & 1.35e-04 & \first{1.14e-06}\\
 & LS-Chebyshev & 1.38e-02 & 2.93e-03  & 4.36e-03 & 5.51e-04  & 7.29e-04 & 7.56e-05  & 1.61e-04 & 1.14e-05  & 2.90e-05 & 1.40e-06\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 1.64e+01 & 1.22e+00  & 1.34e+01 & 8.31e-01  & 9.61e+00 & 4.93e-01  & 5.26e+00 & 2.66e-01  & 3.23e+00 & 1.35e-01\\
 & LS-Uniform & 7.44e+00 & \first{7.64e-01}  & 5.69e+00 & \first{4.08e-01}  & 3.73e+00 & \first{2.25e-01}  & 3.20e+00 & \first{1.20e-01}  & 2.14e+00 & \first{6.46e-02}\\
 & LS-Chebyshev & \first{6.29e+00} & 1.45e+00  & \first{3.24e+00} & 7.89e-01  & \first{2.17e+00} & 3.60e-01  & \first{1.98e+00} & 1.62e-01  & \first{9.39e-01} & 7.06e-02\\
\bottomrule
\end{tabular}


==> tables/dim8.tex <==
% Created with Python on 2025-06-22 19:31:16
% ..\results\final_results\low_dim\results_numerical_experiments.csv, dim=8, scales = [3, 4, 5, 6]
\begin{tabular}{ll|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 1.27e+00 & 3.51e-01  & 9.95e-01 & 1.66e-01  & 4.83e-01 & 7.72e-02  & 3.37e-01 & 3.80e-02\\
 & LS-Uniform & \first{6.17e-01} & \first{5.79e-02}  & 6.54e-01 & \first{4.06e-02}  & 8.87e-01 & \first{2.64e-02}  & 1.06e+00 & 1.82e-02\\
 & LS-Chebyshev & 6.28e-01 & 6.48e-02  & \first{5.80e-01} & 5.10e-02  & \first{4.61e-01} & 2.74e-02  & \first{2.74e-01} & \first{1.46e-02}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 2.35e-02 & 4.67e-03  & \first{1.13e-02} & 1.89e-03  & 6.45e-03 & 6.21e-04  & 3.25e-03 & 2.40e-04\\
 & LS-Uniform & 2.41e-02 & \first{4.44e-03}  & 1.40e-02 & 1.80e-03  & 9.09e-03 & 7.09e-04  & 5.86e-03 & 2.80e-04\\
 & LS-Chebyshev & \first{2.22e-02} & 4.75e-03  & 1.26e-02 & \first{1.65e-03}  & \first{5.08e-03} & \first{6.01e-04}  & \first{2.85e-03} & \first{2.17e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 1.40e-03 & \first{6.37e-05}  & 7.79e-03 & 5.32e-04  & 4.59e-02 & 9.43e-04  & 4.68e-02 & 1.34e-03\\
 & LS-Uniform & \first{1.29e-03} & 8.69e-05  & \first{1.43e-03} & \first{9.33e-05}  & \first{9.09e-03} & \first{7.55e-05}  & \first{7.43e-03} & \first{7.63e-05}\\
 & LS-Chebyshev & 1.52e-02 & 3.77e-03  & 2.64e-02 & 3.62e-03  & 2.40e-02 & 2.21e-03  & 1.56e-02 & 9.77e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 6.16e+02 & \first{4.12e+01}  & 4.69e+02 & \first{3.33e+01}  & 1.00e+03 & \first{2.78e+01}  & 8.55e+02 & \first{2.15e+01}\\
 & LS-Uniform & \first{4.39e+02} & 4.64e+01  & 5.24e+02 & 4.03e+01  & \first{7.67e+02} & 3.26e+01  & 8.95e+02 & 2.75e+01\\
 & LS-Chebyshev & 5.56e+02 & 8.63e+01  & \first{4.46e+02} & 6.56e+01  & 8.71e+02 & 4.60e+01  & \first{8.14e+02} & 3.56e+01\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & \first{5.52e-01} & 1.32e-01  & 6.66e-01 & 7.20e-02  & 5.10e-01 & 4.32e-02  & 3.42e-01 & 2.35e-02\\
 & LS-Uniform & 5.90e-01 & \first{5.49e-02}  & 9.57e-01 & \first{3.33e-02}  & 7.75e-01 & 2.12e-02  & 8.86e-01 & 1.30e-02\\
 & LS-Chebyshev & 6.10e-01 & 7.08e-02  & \first{5.32e-01} & 3.60e-02  & \first{4.23e-01} & \first{2.02e-02}  & \first{2.45e-01} & \first{1.11e-02}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & \first{7.50e-02} & 1.68e-02  & 2.32e-02 & 3.01e-03  & 6.07e-03 & 5.67e-04  & 1.60e-03 & 1.05e-04\\
 & LS-Uniform & 8.86e-02 & \first{1.09e-02}  & 2.59e-02 & \first{1.87e-03}  & \first{3.50e-03} & \first{2.15e-04}  & 1.94e-03 & \first{2.84e-05}\\
 & LS-Chebyshev & 1.03e-01 & 2.53e-02  & \first{2.16e-02} & 4.55e-03  & 4.17e-03 & 5.71e-04  & \first{3.78e-04} & 6.69e-05\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 5.30e-06 & 8.86e-07  & 1.10e-05 & 1.46e-06  & 1.77e-05 & 1.94e-06  & 2.64e-05 & 2.67e-06\\
 & LS-Uniform & 9.18e-07 & \first{1.34e-07}  & 1.41e-06 & \first{1.42e-07}  & 3.08e-06 & \first{1.58e-07}  & 6.80e-06 & 1.81e-07\\
 & LS-Chebyshev & \first{7.69e-07} & 1.75e-07  & \first{8.40e-07} & 1.63e-07  & \first{9.82e-07} & 1.61e-07  & \first{1.08e-06} & \first{1.61e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & 1.74e+01 & 1.53e+00  & 1.66e+01 & 1.13e+00  & 1.42e+01 & 7.29e-01  & 1.29e+01 & 4.34e-01\\
 & LS-Uniform & 1.07e+01 & \first{1.20e+00}  & 1.22e+01 & \first{9.90e-01}  & 1.71e+01 & \first{7.00e-01}  & 2.00e+01 & \first{4.00e-01}\\
 & LS-Chebyshev & \first{5.75e+00} & 1.45e+00  & \first{5.84e+00} & 1.27e+00  & \first{5.79e+00} & 1.09e+00  & \first{4.52e+00} & 7.55e-01\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & \first{1.07e-02} & 1.34e-03  & \first{3.01e-03} & 2.86e-04  & \first{1.05e-03} & 6.48e-05  & \first{2.19e-04} & 1.16e-05\\
 & LS-Uniform & 1.70e-02 & \first{1.32e-03}  & 4.71e-03 & \first{2.49e-04}  & 1.48e-03 & \first{4.39e-05}  & 1.19e-03 & \first{7.35e-06}\\
 & LS-Chebyshev & 1.87e-02 & 2.34e-03  & 5.39e-03 & 4.65e-04  & 1.11e-03 & 8.02e-05  & 2.30e-04 & 1.16e-05\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 2.29e+01 & 1.85e+00  & 2.60e+01 & 1.40e+00  & 1.89e+01 & 9.00e-01  & 1.10e+01 & 5.33e-01\\
 & LS-Uniform & \first{7.92e+00} & \first{1.30e+00}  & \first{6.54e+00} & \first{7.10e-01}  & 5.65e+00 & \first{3.95e-01}  & 5.08e+00 & \first{2.09e-01}\\
 & LS-Chebyshev & 9.91e+00 & 2.75e+00  & 6.68e+00 & 1.61e+00  & \first{4.08e+00} & 7.55e-01  & \first{2.58e+00} & 3.53e-01\\
\bottomrule
\end{tabular}


==> tables/dim9.tex <==
% Created with Python on 2025-06-22 19:31:17
% ..\results\final_results\low_dim\results_numerical_experiments.csv, dim=9, scales = [3, 4, 5, 6]
\begin{tabular}{ll|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Scale 3} & \multicolumn{2}{c}{Scale 4} & \multicolumn{2}{c}{Scale 5} & \multicolumn{2}{c}{Scale 6}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 8.64e-01 & 2.63e-01  & 8.49e-01 & 1.23e-01  & 7.20e-01 & 5.77e-02  & 3.17e-01 & 2.91e-02\\
 & LS-Uniform & \first{5.65e-01} & \first{6.83e-02}  & 1.42e+00 & \first{4.23e-02}  & 1.13e+00 & 2.90e-02  & 1.43e+00 & 1.83e-02\\
 & LS-Chebyshev & 6.50e-01 & 7.35e-02  & \first{5.48e-01} & 4.42e-02  & \first{4.36e-01} & \first{2.71e-02}  & \first{2.98e-01} & \first{1.59e-02}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & \first{2.08e-02} & \first{4.22e-03}  & 1.26e-02 & \first{1.74e-03}  & \first{4.71e-03} & 7.08e-04  & 3.44e-03 & 2.55e-04\\
 & LS-Uniform & 2.26e-02 & 4.27e-03  & 1.56e-02 & 1.86e-03  & 1.33e-02 & 7.18e-04  & 9.70e-03 & 2.93e-04\\
 & LS-Chebyshev & 2.09e-02 & 4.60e-03  & \first{9.93e-03} & 1.86e-03  & 5.37e-03 & \first{6.31e-04}  & \first{2.60e-03} & \first{2.33e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & \first{1.30e-03} & \first{4.80e-05}  & 1.49e-02 & 4.24e-04  & 3.07e-02 & 6.85e-04  & 4.38e-02 & 8.63e-04\\
 & LS-Uniform & 1.46e-03 & 5.45e-05  & \first{6.29e-03} & \first{8.21e-05}  & \first{5.84e-03} & \first{3.80e-05}  & 2.55e-02 & \first{8.50e-05}\\
 & LS-Chebyshev & 3.56e-02 & 8.37e-03  & 2.21e-02 & 3.34e-03  & 1.46e-02 & 1.54e-03  & \first{1.97e-02} & 1.03e-03\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 1.11e+03 & \first{7.78e+01}  & 1.84e+03 & \first{5.96e+01}  & 1.62e+03 & \first{4.44e+01}  & 2.28e+03 & \first{3.75e+01}\\
 & LS-Uniform & 1.25e+03 & 9.28e+01  & \first{1.59e+03} & 7.37e+01  & \first{1.57e+03} & 5.85e+01  & \first{1.85e+03} & 4.80e+01\\
 & LS-Chebyshev & \first{1.06e+03} & 1.61e+02  & 1.98e+03 & 1.45e+02  & 1.73e+03 & 9.91e+01  & 2.05e+03 & 7.17e+01\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 5.85e-01 & 1.46e-01  & 9.05e-01 & 8.47e-02  & 5.07e-01 & 4.52e-02  & 3.81e-01 & 2.74e-02\\
 & LS-Uniform & \first{5.43e-01} & 4.69e-02  & 8.32e-01 & 3.36e-02  & 8.26e-01 & 2.38e-02  & 1.39e+00 & 1.49e-02\\
 & LS-Chebyshev & 5.99e-01 & \first{4.31e-02}  & \first{5.93e-01} & \first{3.13e-02}  & \first{4.24e-01} & \first{2.10e-02}  & \first{2.95e-01} & \first{1.27e-02}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 1.54e-01 & 3.18e-02  & \first{5.70e-02} & 8.03e-03  & \first{1.56e-02} & 1.37e-03  & 3.57e-03 & 1.52e-04\\
 & LS-Uniform & \first{1.28e-01} & \first{1.48e-02}  & 7.95e-02 & \first{4.52e-03}  & 2.44e-02 & \first{8.86e-04}  & 4.25e-03 & \first{8.22e-05}\\
 & LS-Chebyshev & 1.58e-01 & 4.58e-02  & 6.94e-02 & 1.42e-02  & 1.70e-02 & 2.74e-03  & \first{2.24e-03} & 2.98e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 5.41e-06 & 1.18e-06  & 1.23e-05 & 1.76e-06  & 2.59e-05 & 2.62e-06  & 3.88e-05 & 3.57e-06\\
 & LS-Uniform & 1.03e-06 & \first{1.31e-07}  & 1.69e-06 & \first{1.39e-07}  & 3.67e-06 & \first{1.53e-07}  & 1.05e-05 & 1.74e-07\\
 & LS-Chebyshev & \first{7.20e-07} & 1.85e-07  & \first{9.39e-07} & 1.73e-07  & \first{1.14e-06} & 1.65e-07  & \first{1.33e-06} & \first{1.65e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & 2.42e+01 & 2.27e+00  & 3.33e+01 & 1.48e+00  & 2.19e+01 & 1.12e+00  & 2.13e+01 & 7.17e-01\\
 & LS-Uniform & 8.54e+00 & \first{1.15e+00}  & 1.69e+01 & \first{1.07e+00}  & 3.41e+01 & \first{8.90e-01}  & 4.13e+01 & \first{6.09e-01}\\
 & LS-Chebyshev & \first{6.95e+00} & 1.52e+00  & \first{6.84e+00} & 1.41e+00  & \first{6.82e+00} & 1.24e+00  & \first{6.29e+00} & 9.71e-01\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & \first{1.05e-02} & 1.84e-03  & \first{3.58e-03} & 3.43e-04  & \first{9.39e-04} & 6.33e-05  & \first{1.40e-04} & 1.04e-05\\
 & LS-Uniform & 1.62e-02 & \first{1.52e-03}  & 8.66e-03 & \first{3.02e-04}  & 2.92e-03 & \first{4.69e-05}  & 9.15e-04 & \first{7.01e-06}\\
 & LS-Chebyshev & 2.39e-02 & 3.22e-03  & 6.19e-03 & 5.25e-04  & 1.35e-03 & 8.90e-05  & 2.73e-04 & 1.25e-05\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 4.61e+01 & 2.46e+00  & 4.11e+01 & 1.85e+00  & 3.73e+01 & 1.30e+00  & 2.35e+01 & 7.50e-01\\
 & LS-Uniform & 1.93e+01 & \first{1.52e+00}  & 1.51e+01 & \first{8.92e-01}  & 1.48e+01 & \first{4.86e-01}  & 8.80e+00 & \first{2.75e-01}\\
 & LS-Chebyshev & \first{1.54e+01} & 4.25e+00  & \first{1.39e+01} & 2.17e+00  & \first{8.35e+00} & 1.18e+00  & \first{4.76e+00} & 5.52e-01\\
\bottomrule
\end{tabular}


==> tables/scale1.tex <==
% Created with Python on 2025-06-22 19:31:17
% ..\results\final_results\low_dim\results_numerical_experiments.csv, scale=1, dims = [2, 3, 4, 5, 6, 7, 8, 9, 10]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Dim2} & \multicolumn{2}{c}{Dim3} & \multicolumn{2}{c}{Dim4} & \multicolumn{2}{c}{Dim5} & \multicolumn{2}{c}{Dim6} & \multicolumn{2}{c}{Dim7} & \multicolumn{2}{c}{Dim8} & \multicolumn{2}{c}{Dim9} & \multicolumn{2}{c}{Dim10}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 1.56e+00 & 1.17e+00  & 1.26e+00 & 9.13e-01  & 8.30e-01 & 5.01e-01  & 7.70e-01 & 3.53e-01  & 8.31e-01 & 3.12e-01  & \first{5.45e-01} & 2.53e-01  & 1.90e+00 & 9.58e-01  & 1.35e+00 & 7.58e-01  & 1.66e+00 & 1.03e+00\\
 & LS-Uniform & 8.30e-01 & 5.13e-01  & \first{8.92e-01} & \first{4.68e-01}  & 9.11e-01 & 4.84e-01  & 8.47e-01 & \first{2.98e-01}  & 6.41e-01 & \first{2.77e-01}  & 5.46e-01 & \first{1.48e-01}  & 5.41e-01 & 2.04e-01  & 5.23e-01 & 1.85e-01  & \first{4.65e-01} & 1.36e-01\\
 & LS-Chebyshev & \first{8.21e-01} & \first{5.01e-01}  & 9.06e-01 & 5.05e-01  & \first{8.11e-01} & \first{4.50e-01}  & \first{7.59e-01} & 3.26e-01  & \first{5.69e-01} & 2.96e-01  & 5.57e-01 & 1.55e-01  & \first{5.28e-01} & \first{1.29e-01}  & \first{5.08e-01} & \first{1.35e-01}  & 5.64e-01 & \first{1.26e-01}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 1.51e-01 & 9.80e-02  & 1.24e-01 & 7.13e-02  & 1.07e-01 & 6.20e-02  & 9.92e-02 & 4.83e-02  & 1.01e-01 & 4.96e-02  & 1.08e-01 & 4.83e-02  & \first{7.43e-02} & \first{3.34e-02}  & 1.02e-01 & 3.70e-02  & 6.79e-02 & 2.61e-02\\
 & LS-Uniform & \first{1.49e-01} & \first{8.37e-02}  & \first{7.27e-02} & \first{4.13e-02}  & \first{8.20e-02} & \first{3.55e-02}  & 1.05e-01 & \first{3.63e-02}  & \first{9.53e-02} & \first{3.92e-02}  & \first{6.57e-02} & \first{2.86e-02}  & 1.25e-01 & 4.13e-02  & \first{8.14e-02} & \first{2.78e-02}  & \first{6.67e-02} & \first{2.56e-02}\\
 & LS-Chebyshev & 1.72e-01 & 1.16e-01  & 1.02e-01 & 7.02e-02  & 1.42e-01 & 8.05e-02  & \first{9.50e-02} & 5.25e-02  & 1.36e-01 & 6.13e-02  & 8.03e-02 & 3.56e-02  & 1.16e-01 & 4.64e-02  & 9.66e-02 & 4.22e-02  & 7.51e-02 & 3.70e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 1.62e-01 & 1.09e-01  & 7.14e-02 & 4.19e-02  & \first{1.62e-02} & \first{8.75e-03}  & \first{3.53e-03} & \first{1.19e-03}  & 4.65e-03 & 1.30e-03  & \first{7.44e-04} & \first{1.93e-04}  & \first{1.77e-05} & \first{4.38e-06}  & \first{3.77e-06} & \first{8.70e-07}  & \first{4.72e-07} & \first{1.03e-07}\\
 & LS-Uniform & \first{7.50e-02} & \first{5.15e-02}  & \first{5.46e-02} & \first{2.65e-02}  & 2.84e-02 & 1.75e-02  & 6.28e-03 & 3.11e-03  & \first{4.31e-03} & \first{1.20e-03}  & 3.37e-03 & 1.65e-03  & 1.01e-03 & 4.34e-04  & 2.11e-05 & 1.05e-05  & 8.99e-06 & 3.24e-06\\
 & LS-Chebyshev & 1.64e-01 & 1.34e-01  & 2.58e-01 & 1.66e-01  & 1.23e-01 & 8.61e-02  & 9.38e-02 & 5.55e-02  & 2.53e-02 & 1.46e-02  & 2.89e-03 & 1.25e-03  & 6.04e-03 & 3.30e-03  & 1.74e-04 & 8.03e-05  & 2.19e-05 & 9.86e-06\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 5.76e+00 & 3.90e+00  & 9.16e+00 & 3.81e+00  & \first{2.14e+01} & \first{8.82e+00}  & 3.28e+01 & 1.46e+01  & \first{6.95e+01} & \first{2.62e+01}  & 2.82e+02 & 7.46e+01  & \first{4.02e+02} & \first{1.12e+02}  & 6.82e+02 & 2.02e+02  & 1.45e+03 & 4.41e+02\\
 & LS-Uniform & \first{3.88e+00} & \first{2.19e+00}  & 8.99e+00 & \first{3.81e+00}  & 2.76e+01 & 1.02e+01  & \first{2.72e+01} & \first{1.26e+01}  & 1.08e+02 & 3.79e+01  & 2.66e+02 & \first{7.08e+01}  & 4.73e+02 & 1.98e+02  & \first{6.67e+02} & \first{1.94e+02}  & \first{1.39e+03} & \first{4.05e+02}\\
 & LS-Chebyshev & 3.99e+00 & 2.47e+00  & \first{8.12e+00} & 4.07e+00  & 2.41e+01 & 1.43e+01  & 4.34e+01 & 1.37e+01  & 8.30e+01 & 5.26e+01  & \first{2.65e+02} & 8.08e+01  & 6.62e+02 & 3.50e+02  & 6.90e+02 & 2.58e+02  & 4.46e+03 & 2.03e+03\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 9.42e-01 & 5.40e-01  & 8.93e-01 & 3.63e-01  & 7.46e-01 & \first{2.63e-01}  & 7.47e-01 & 2.26e-01  & 7.16e-01 & 2.52e-01  & 5.71e-01 & \first{1.48e-01}  & \first{6.26e-01} & 1.86e-01  & 6.44e-01 & 3.07e-01  & 4.33e-01 & 1.30e-01\\
 & LS-Uniform & 7.55e-01 & \first{4.41e-01}  & \first{7.07e-01} & \first{3.02e-01}  & \first{6.51e-01} & 2.68e-01  & \first{7.28e-01} & \first{2.24e-01}  & \first{6.79e-01} & \first{2.13e-01}  & \first{4.88e-01} & 2.35e-01  & 6.36e-01 & \first{1.55e-01}  & \first{4.72e-01} & 1.19e-01  & 4.34e-01 & \first{9.47e-02}\\
 & LS-Chebyshev & \first{7.42e-01} & 4.46e-01  & 8.76e-01 & 3.48e-01  & 7.72e-01 & 3.11e-01  & 7.62e-01 & 2.82e-01  & 7.37e-01 & 2.38e-01  & 5.72e-01 & 1.56e-01  & 6.64e-01 & 1.62e-01  & 4.96e-01 & \first{1.18e-01}  & \first{3.64e-01} & 1.08e-01\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & \first{9.72e-02} & \first{6.88e-02}  & 2.08e-01 & 1.18e-01  & 3.00e-01 & 1.62e-01  & 2.81e-01 & 1.18e-01  & 5.64e-01 & 2.25e-01  & 4.49e-01 & 1.87e-01  & 4.66e-01 & 1.90e-01  & 4.10e-01 & 2.14e-01  & 5.39e-01 & 1.83e-01\\
 & LS-Uniform & 1.05e-01 & 8.56e-02  & \first{1.07e-01} & \first{5.74e-02}  & \first{2.05e-01} & \first{8.07e-02}  & \first{1.54e-01} & \first{6.13e-02}  & \first{2.47e-01} & \first{8.69e-02}  & \first{2.08e-01} & \first{1.03e-01}  & \first{2.36e-01} & \first{8.88e-02}  & 3.98e-01 & \first{9.98e-02}  & \first{2.92e-01} & \first{1.15e-01}\\
 & LS-Chebyshev & 3.97e-01 & 3.17e-01  & 3.59e-01 & 2.48e-01  & 6.79e-01 & 4.06e-01  & 2.58e-01 & 1.48e-01  & 4.18e-01 & 1.62e-01  & 9.24e-01 & 4.18e-01  & 5.16e-01 & 2.02e-01  & \first{3.95e-01} & 2.73e-01  & 6.54e-01 & 2.75e-01\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 2.32e-07 & 1.59e-07  & 2.67e-07 & \first{1.50e-07}  & \first{3.05e-07} & 1.73e-07  & 6.41e-07 & 2.74e-07  & 5.38e-07 & 2.69e-07  & 6.13e-07 & 2.74e-07  & 1.03e-06 & 5.85e-07  & 8.62e-07 & 5.42e-07  & 1.29e-06 & 7.66e-07\\
 & LS-Uniform & \first{1.65e-07} & \first{1.09e-07}  & \first{2.38e-07} & 1.54e-07  & 3.25e-07 & \first{1.64e-07}  & \first{2.86e-07} & \first{1.33e-07}  & \first{3.30e-07} & \first{1.49e-07}  & \first{4.68e-07} & \first{2.02e-07}  & \first{5.57e-07} & \first{2.16e-07}  & \first{4.21e-07} & \first{1.62e-07}  & \first{4.00e-07} & \first{1.67e-07}\\
 & LS-Chebyshev & 3.58e-07 & 2.39e-07  & 3.55e-07 & 2.54e-07  & 4.30e-07 & 3.13e-07  & 4.29e-07 & 2.78e-07  & 4.34e-07 & 2.37e-07  & 5.77e-07 & 2.90e-07  & 8.21e-07 & 3.00e-07  & 5.59e-07 & 3.33e-07  & 6.60e-07 & 3.07e-07\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & 1.01e+00 & 8.27e-01  & 1.78e+00 & 1.26e+00  & 2.86e+00 & \first{1.17e+00}  & 3.57e+00 & \first{1.60e+00}  & 4.41e+00 & 1.88e+00  & 4.28e+00 & 2.09e+00  & 4.37e+00 & 2.43e+00  & 4.87e+00 & 2.65e+00  & 5.40e+00 & 2.99e+00\\
 & LS-Uniform & \first{8.24e-01} & \first{5.85e-01}  & \first{1.72e+00} & \first{8.66e-01}  & \first{2.48e+00} & 1.24e+00  & \first{2.73e+00} & 1.66e+00  & \first{3.08e+00} & \first{1.32e+00}  & \first{2.88e+00} & \first{1.52e+00}  & 5.25e+00 & 2.43e+00  & \first{4.19e+00} & \first{1.92e+00}  & \first{3.00e+00} & \first{1.50e+00}\\
 & LS-Chebyshev & 1.57e+00 & 1.23e+00  & 2.23e+00 & 1.69e+00  & 3.20e+00 & 2.07e+00  & 2.80e+00 & 1.66e+00  & 3.98e+00 & 2.47e+00  & 4.47e+00 & 1.96e+00  & \first{3.95e+00} & \first{2.12e+00}  & 4.43e+00 & 1.99e+00  & 4.82e+00 & 2.32e+00\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & 6.39e-02 & 4.59e-02  & 9.24e-02 & 4.24e-02  & \first{8.15e-02} & \first{3.78e-02}  & \first{5.67e-02} & \first{2.84e-02}  & 8.65e-02 & 3.76e-02  & 8.63e-02 & \first{2.90e-02}  & \first{6.25e-02} & \first{2.62e-02}  & 1.17e-01 & 4.51e-02  & 1.59e-01 & 5.87e-02\\
 & LS-Uniform & \first{5.23e-02} & \first{3.46e-02}  & \first{6.36e-02} & \first{3.14e-02}  & 1.31e-01 & 5.50e-02  & 5.94e-02 & 3.26e-02  & \first{7.01e-02} & \first{3.26e-02}  & \first{6.97e-02} & 3.13e-02  & 1.01e-01 & 2.96e-02  & \first{5.76e-02} & \first{2.67e-02}  & 8.94e-02 & \first{3.06e-02}\\
 & LS-Chebyshev & 8.50e-02 & 6.00e-02  & 1.02e-01 & 7.39e-02  & 8.30e-02 & 5.09e-02  & 9.35e-02 & 5.07e-02  & 1.63e-01 & 1.11e-01  & 1.54e-01 & 8.57e-02  & 1.04e-01 & 4.06e-02  & 9.06e-02 & 3.65e-02  & \first{7.97e-02} & 4.10e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & \first{6.43e-01} & 5.07e-01  & 9.88e-01 & 6.60e-01  & 2.00e+00 & 7.96e-01  & 2.83e+00 & 1.08e+00  & 5.23e+00 & 1.86e+00  & 5.53e+00 & \first{1.59e+00}  & \first{8.78e+00} & \first{2.77e+00}  & 1.52e+01 & \first{3.62e+00}  & \first{1.89e+01} & \first{5.07e+00}\\
 & LS-Uniform & 7.26e-01 & \first{3.64e-01}  & \first{7.44e-01} & \first{4.11e-01}  & \first{1.54e+00} & \first{6.40e-01}  & \first{2.49e+00} & \first{9.43e-01}  & \first{4.08e+00} & \first{1.47e+00}  & \first{4.61e+00} & 1.96e+00  & 1.49e+01 & 6.40e+00  & \first{1.04e+01} & 5.43e+00  & 2.34e+01 & 8.50e+00\\
 & LS-Chebyshev & 7.28e-01 & 5.03e-01  & 1.66e+00 & 1.24e+00  & 2.26e+00 & 1.42e+00  & 5.11e+00 & 2.77e+00  & 7.61e+00 & 4.43e+00  & 1.21e+01 & 6.04e+00  & 1.49e+01 & 7.31e+00  & 1.89e+01 & 9.40e+00  & 5.86e+01 & 2.52e+01\\
\bottomrule
\end{tabular}


==> tables/scale2.tex <==
% Created with Python on 2025-06-22 19:31:17
% ..\results\final_results\low_dim\results_numerical_experiments.csv, scale=2, dims = [2, 3, 4, 5, 6, 7, 8, 9, 10]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Dim2} & \multicolumn{2}{c}{Dim3} & \multicolumn{2}{c}{Dim4} & \multicolumn{2}{c}{Dim5} & \multicolumn{2}{c}{Dim6} & \multicolumn{2}{c}{Dim7} & \multicolumn{2}{c}{Dim8} & \multicolumn{2}{c}{Dim9} & \multicolumn{2}{c}{Dim10}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 1.12e+00 & 7.34e-01  & 1.22e+00 & 5.84e-01  & \first{7.47e-01} & 3.33e-01  & \first{6.75e-01} & 3.07e-01  & \first{6.69e-01} & 2.27e-01  & 5.97e-01 & \first{1.05e-01}  & 1.77e+00 & 4.40e-01  & 1.96e+00 & 4.06e-01  & 2.32e+00 & 5.01e-01\\
 & LS-Uniform & 1.17e+00 & \first{4.40e-01}  & 1.92e+00 & 6.81e-01  & 1.50e+00 & 4.65e-01  & 7.46e-01 & \first{1.82e-01}  & 6.86e-01 & \first{1.62e-01}  & \first{5.79e-01} & 1.14e-01  & \first{5.83e-01} & 1.01e-01  & \first{5.77e-01} & 9.53e-02  & \first{5.11e-01} & 7.66e-02\\
 & LS-Chebyshev & \first{8.38e-01} & 5.24e-01  & \first{8.34e-01} & \first{3.32e-01}  & 8.28e-01 & \first{2.32e-01}  & 7.32e-01 & 2.23e-01  & 6.88e-01 & 1.65e-01  & 5.98e-01 & 1.15e-01  & 6.20e-01 & \first{8.95e-02}  & 6.06e-01 & \first{7.13e-02}  & 6.10e-01 & \first{7.28e-02}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 8.77e-02 & 4.16e-02  & 7.72e-02 & \first{2.60e-02}  & 6.14e-02 & 2.25e-02  & 6.47e-02 & 1.80e-02  & 4.88e-02 & 1.71e-02  & 4.45e-02 & 1.47e-02  & 3.57e-02 & \first{1.10e-02}  & 3.91e-02 & 1.13e-02  & 4.08e-02 & 1.05e-02\\
 & LS-Uniform & \first{6.10e-02} & \first{2.48e-02}  & 1.36e-01 & 4.56e-02  & 9.02e-02 & 2.33e-02  & \first{5.54e-02} & \first{1.74e-02}  & \first{3.87e-02} & \first{1.30e-02}  & 5.09e-02 & \first{1.22e-02}  & 3.73e-02 & 1.11e-02  & 4.07e-02 & \first{1.07e-02}  & \first{4.01e-02} & \first{9.15e-03}\\
 & LS-Chebyshev & 8.10e-02 & 3.51e-02  & \first{7.45e-02} & 2.80e-02  & \first{5.80e-02} & \first{2.18e-02}  & 6.01e-02 & 1.87e-02  & 5.21e-02 & 1.59e-02  & \first{3.99e-02} & 1.25e-02  & \first{3.43e-02} & 1.19e-02  & \first{3.60e-02} & 1.23e-02  & 4.85e-02 & 1.41e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 3.31e-02 & 1.75e-02  & 1.10e-01 & 3.52e-02  & 1.03e-01 & 2.78e-02  & 4.69e-02 & 9.05e-03  & \first{1.78e-02} & \first{1.96e-03}  & \first{2.10e-03} & \first{2.56e-04}  & \first{7.72e-04} & \first{6.41e-05}  & \first{1.10e-04} & \first{9.74e-06}  & \first{1.40e-05} & \first{9.42e-07}\\
 & LS-Uniform & \first{1.25e-02} & \first{6.21e-03}  & \first{3.65e-02} & \first{1.04e-02}  & \first{5.57e-02} & \first{1.94e-02}  & \first{2.16e-02} & \first{6.89e-03}  & 1.84e-02 & 4.50e-03  & 7.17e-03 & 1.46e-03  & 1.17e-03 & 2.09e-04  & 2.34e-04 & 3.07e-05  & 1.41e-05 & 2.73e-06\\
 & LS-Chebyshev & 4.52e-02 & 3.37e-02  & 7.97e-02 & 3.29e-02  & 1.81e-01 & 6.51e-02  & 2.39e-01 & 8.54e-02  & 2.85e-02 & 8.20e-03  & 3.86e-02 & 1.22e-02  & 1.90e-02 & 6.72e-03  & 4.50e-03 & 1.19e-03  & 3.34e-04 & 1.13e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 4.39e+00 & \first{1.86e+00}  & \first{7.58e+00} & 2.60e+00  & 2.47e+01 & \first{6.15e+00}  & 4.73e+01 & \first{9.99e+00}  & \first{8.60e+01} & \first{1.47e+01}  & 3.34e+02 & \first{4.17e+01}  & 5.68e+02 & 6.72e+01  & 8.03e+02 & \first{9.31e+01}  & \first{2.17e+03} & \first{2.49e+02}\\
 & LS-Uniform & 3.86e+00 & 1.90e+00  & 1.48e+01 & 5.39e+00  & \first{2.38e+01} & 6.72e+00  & \first{3.92e+01} & 1.03e+01  & 9.21e+01 & 1.83e+01  & \first{2.54e+02} & 4.19e+01  & 5.13e+02 & \first{6.42e+01}  & \first{6.11e+02} & 9.97e+01  & 3.42e+03 & 2.97e+02\\
 & LS-Chebyshev & \first{3.73e+00} & 2.11e+00  & 7.78e+00 & \first{2.29e+00}  & 2.48e+01 & 9.69e+00  & 4.00e+01 & 1.99e+01  & 1.25e+02 & 4.44e+01  & 2.86e+02 & 7.86e+01  & \first{4.12e+02} & 1.43e+02  & 7.27e+02 & 2.15e+02  & 3.39e+03 & 1.00e+03\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 8.29e-01 & 3.55e-01  & 8.19e-01 & 3.79e-01  & \first{7.22e-01} & 2.78e-01  & 7.24e-01 & 1.58e-01  & 7.04e-01 & 2.18e-01  & 5.82e-01 & 1.27e-01  & 6.50e-01 & 1.44e-01  & 7.17e-01 & 1.92e-01  & 4.59e-01 & 1.15e-01\\
 & LS-Uniform & \first{6.07e-01} & \first{2.45e-01}  & 1.12e+00 & 3.96e-01  & 7.90e-01 & 2.51e-01  & \first{6.01e-01} & \first{1.28e-01}  & \first{5.87e-01} & \first{1.20e-01}  & \first{5.03e-01} & \first{8.79e-02}  & \first{5.95e-01} & \first{6.32e-02}  & \first{5.36e-01} & \first{5.22e-02}  & \first{3.84e-01} & \first{6.36e-02}\\
 & LS-Chebyshev & 8.86e-01 & 3.60e-01  & \first{6.98e-01} & \first{2.04e-01}  & 7.65e-01 & \first{1.76e-01}  & 7.16e-01 & 1.72e-01  & 7.45e-01 & 1.20e-01  & 6.43e-01 & 8.92e-02  & 6.58e-01 & 8.67e-02  & 6.07e-01 & 5.76e-02  & 5.38e-01 & 7.31e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 5.07e-02 & 2.31e-02  & 1.00e-01 & 4.38e-02  & 2.20e-01 & 6.19e-02  & 1.03e-01 & 3.22e-02  & 2.54e-01 & 7.21e-02  & 3.54e-01 & 9.83e-02  & \first{1.90e-01} & 6.85e-02  & 3.34e-01 & 8.64e-02  & 2.70e-01 & 8.91e-02\\
 & LS-Uniform & \first{6.79e-03} & \first{3.55e-03}  & \first{5.60e-02} & \first{2.09e-02}  & \first{1.16e-01} & \first{2.86e-02}  & 1.24e-01 & \first{2.71e-02}  & \first{2.49e-01} & \first{4.65e-02}  & 3.20e-01 & \first{5.84e-02}  & 2.02e-01 & \first{3.86e-02}  & \first{1.95e-01} & \first{3.54e-02}  & \first{1.80e-01} & \first{3.85e-02}\\
 & LS-Chebyshev & 6.96e-02 & 3.74e-02  & 5.71e-02 & 2.38e-02  & 2.83e-01 & 9.10e-02  & \first{9.36e-02} & 4.05e-02  & 2.79e-01 & 1.19e-01  & \first{2.82e-01} & 1.14e-01  & 3.34e-01 & 9.70e-02  & 2.58e-01 & 9.87e-02  & 2.92e-01 & 9.64e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 4.78e-07 & 2.29e-07  & 9.14e-07 & 3.15e-07  & 9.27e-07 & 3.96e-07  & 9.73e-07 & 4.44e-07  & 1.36e-06 & 4.85e-07  & 2.06e-06 & 6.14e-07  & 1.95e-06 & 5.86e-07  & 3.21e-06 & 8.84e-07  & 3.91e-06 & 1.11e-06\\
 & LS-Uniform & \first{2.28e-07} & \first{1.29e-07}  & 8.45e-07 & 3.02e-07  & 6.35e-07 & 1.76e-07  & \first{6.01e-07} & \first{1.92e-07}  & \first{6.19e-07} & \first{1.57e-07}  & \first{5.99e-07} & \first{1.54e-07}  & 7.64e-07 & \first{1.37e-07}  & 6.75e-07 & \first{1.28e-07}  & \first{5.19e-07} & \first{1.30e-07}\\
 & LS-Chebyshev & 4.69e-07 & 2.54e-07  & \first{4.11e-07} & \first{1.98e-07}  & \first{5.34e-07} & \first{1.69e-07}  & 6.42e-07 & 2.15e-07  & 6.44e-07 & 2.55e-07  & 6.30e-07 & 2.19e-07  & \first{5.83e-07} & 1.97e-07  & \first{6.07e-07} & 2.01e-07  & 9.23e-07 & 2.57e-07\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & 2.96e-01 & 1.89e-01  & \first{1.01e+00} & \first{5.23e-01}  & \first{1.94e+00} & \first{7.97e-01}  & \first{2.83e+00} & \first{9.29e-01}  & 5.13e+00 & \first{1.20e+00}  & 8.23e+00 & 1.68e+00  & 1.17e+01 & 2.08e+00  & 1.40e+01 & 2.74e+00  & 1.72e+01 & 3.44e+00\\
 & LS-Uniform & \first{1.37e-01} & \first{7.05e-02}  & 2.64e+00 & 8.48e-01  & 4.16e+00 & 1.14e+00  & 3.58e+00 & 1.11e+00  & 4.73e+00 & 1.25e+00  & \first{5.14e+00} & \first{1.20e+00}  & 4.87e+00 & \first{1.21e+00}  & 5.45e+00 & \first{1.16e+00}  & \first{4.12e+00} & \first{1.14e+00}\\
 & LS-Chebyshev & 4.80e-01 & 3.20e-01  & 1.79e+00 & 6.39e-01  & 2.86e+00 & 9.75e-01  & 4.75e+00 & 1.57e+00  & \first{4.18e+00} & 1.61e+00  & 5.29e+00 & 1.57e+00  & \first{4.63e+00} & 1.56e+00  & \first{5.26e+00} & 1.67e+00  & 6.11e+00 & 1.71e+00\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & 8.69e-03 & 5.74e-03  & \first{1.78e-02} & \first{8.89e-03}  & \first{3.46e-02} & \first{9.59e-03}  & 3.36e-02 & \first{7.94e-03}  & 2.46e-02 & \first{6.68e-03}  & \first{2.25e-02} & \first{6.94e-03}  & \first{2.79e-02} & \first{5.45e-03}  & \first{2.28e-02} & \first{7.06e-03}  & 8.27e-02 & 9.52e-03\\
 & LS-Uniform & \first{3.95e-03} & \first{2.33e-03}  & 2.85e-02 & 9.77e-03  & 6.57e-02 & 1.75e-02  & \first{3.02e-02} & 9.87e-03  & \first{2.37e-02} & 8.88e-03  & 2.50e-02 & 7.56e-03  & 3.70e-02 & 6.13e-03  & 2.86e-02 & 9.01e-03  & \first{4.57e-02} & \first{7.12e-03}\\
 & LS-Chebyshev & 1.31e-02 & 8.38e-03  & 1.84e-02 & 9.91e-03  & 4.16e-02 & 1.13e-02  & 5.68e-02 & 1.97e-02  & 4.80e-02 & 1.20e-02  & 5.09e-02 & 1.81e-02  & 6.07e-02 & 1.05e-02  & 7.38e-02 & 1.50e-02  & 8.08e-02 & 1.35e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 4.40e-01 & 2.59e-01  & 1.17e+00 & 3.91e-01  & 2.44e+00 & 6.04e-01  & 3.69e+00 & 8.58e-01  & 8.20e+00 & 1.27e+00  & 6.92e+00 & \first{1.39e+00}  & 1.45e+01 & 2.23e+00  & 3.03e+01 & 3.30e+00  & 2.35e+01 & 3.30e+00\\
 & LS-Uniform & \first{3.26e-01} & \first{1.59e-01}  & 1.67e+00 & 5.49e-01  & \first{1.77e+00} & \first{4.15e-01}  & \first{2.65e+00} & \first{6.98e-01}  & \first{4.82e+00} & \first{1.05e+00}  & \first{6.86e+00} & 1.63e+00  & \first{1.24e+01} & \first{1.96e+00}  & \first{1.38e+01} & \first{2.87e+00}  & \first{1.44e+01} & \first{2.79e+00}\\
 & LS-Chebyshev & 3.80e-01 & 2.03e-01  & \first{7.31e-01} & \first{2.36e-01}  & 1.77e+00 & 5.16e-01  & 5.16e+00 & 1.80e+00  & 5.27e+00 & 2.04e+00  & 1.49e+01 & 5.01e+00  & 1.75e+01 & 5.55e+00  & 3.42e+01 & 1.01e+01  & 3.09e+01 & 1.02e+01\\
\bottomrule
\end{tabular}


==> tables/scale3.tex <==
% Created with Python on 2025-06-22 19:31:17
% ..\results\final_results\low_dim\results_numerical_experiments.csv, scale=3, dims = [2, 3, 4, 5, 6, 7, 8, 9, 10]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Dim2} & \multicolumn{2}{c}{Dim3} & \multicolumn{2}{c}{Dim4} & \multicolumn{2}{c}{Dim5} & \multicolumn{2}{c}{Dim6} & \multicolumn{2}{c}{Dim7} & \multicolumn{2}{c}{Dim8} & \multicolumn{2}{c}{Dim9} & \multicolumn{2}{c}{Dim10}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & \first{5.71e-01} & \first{2.69e-01}  & 7.17e-01 & 2.93e-01  & \first{6.34e-01} & 1.76e-01  & 6.58e-01 & 2.19e-01  & 7.63e-01 & 1.60e-01  & \first{5.74e-01} & 9.52e-02  & 1.27e+00 & 3.51e-01  & 8.64e-01 & 2.63e-01  & 1.21e+00 & 2.73e-01\\
 & LS-Uniform & 3.51e+00 & 8.16e-01  & 2.47e+00 & 4.44e-01  & 1.40e+00 & 1.86e-01  & 9.73e-01 & 1.46e-01  & 9.79e-01 & \first{1.16e-01}  & 6.72e-01 & \first{7.97e-02}  & \first{6.17e-01} & \first{5.79e-02}  & \first{5.65e-01} & \first{6.83e-02}  & \first{5.24e-01} & \first{6.01e-02}\\
 & LS-Chebyshev & 7.40e-01 & 2.89e-01  & \first{6.04e-01} & \first{1.77e-01}  & 7.14e-01 & \first{1.56e-01}  & \first{5.92e-01} & \first{1.11e-01}  & \first{7.01e-01} & 1.23e-01  & 6.09e-01 & 8.44e-02  & 6.28e-01 & 6.48e-02  & 6.50e-01 & 7.35e-02  & 6.88e-01 & 6.53e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & \first{4.40e-02} & \first{1.49e-02}  & 4.54e-02 & 1.16e-02  & 3.06e-02 & \first{7.22e-03}  & 3.24e-02 & \first{6.00e-03}  & \first{2.46e-02} & \first{5.14e-03}  & 3.05e-02 & 6.08e-03  & 2.35e-02 & 4.67e-03  & \first{2.08e-02} & \first{4.22e-03}  & 2.33e-02 & 4.16e-03\\
 & LS-Uniform & 2.66e-01 & 7.08e-02  & 9.00e-02 & 1.51e-02  & 6.82e-02 & 8.94e-03  & 3.47e-02 & 7.08e-03  & 3.23e-02 & 5.40e-03  & 3.32e-02 & \first{5.12e-03}  & 2.41e-02 & \first{4.44e-03}  & 2.26e-02 & 4.27e-03  & 2.36e-02 & \first{3.73e-03}\\
 & LS-Chebyshev & 4.80e-02 & 2.21e-02  & \first{3.30e-02} & \first{9.08e-03}  & \first{2.80e-02} & 7.87e-03  & \first{2.80e-02} & 6.25e-03  & 2.47e-02 & 5.55e-03  & \first{2.13e-02} & 5.31e-03  & \first{2.22e-02} & 4.75e-03  & 2.09e-02 & 4.60e-03  & \first{2.23e-02} & 4.08e-03\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & \first{8.78e-03} & 4.52e-03  & 5.78e-02 & 1.58e-02  & 1.62e-01 & 2.46e-02  & 1.56e-01 & 2.07e-02  & 2.46e-02 & 2.99e-03  & 1.68e-02 & 1.40e-03  & 1.40e-03 & \first{6.37e-05}  & \first{1.30e-03} & \first{4.80e-05}  & 4.08e-04 & \first{1.11e-05}\\
 & LS-Uniform & 1.54e-02 & 3.24e-03  & 7.11e-02 & \first{1.33e-02}  & \first{9.45e-02} & \first{1.05e-02}  & \first{4.36e-02} & \first{5.32e-03}  & \first{2.41e-02} & \first{2.87e-03}  & \first{1.49e-02} & \first{7.53e-04}  & \first{1.29e-03} & 8.69e-05  & 1.46e-03 & 5.45e-05  & \first{3.87e-04} & 2.09e-05\\
 & LS-Chebyshev & 8.88e-03 & \first{3.12e-03}  & \first{3.38e-02} & 1.34e-02  & 1.14e-01 & 2.12e-02  & 1.51e-01 & 3.78e-02  & 7.62e-02 & 2.10e-02  & 3.82e-02 & 1.26e-02  & 1.52e-02 & 3.77e-03  & 3.56e-02 & 8.37e-03  & 1.62e-03 & 2.92e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 4.73e+00 & \first{1.26e+00}  & 7.08e+00 & \first{1.73e+00}  & 2.40e+01 & \first{3.96e+00}  & \first{4.92e+01} & 7.98e+00  & 1.19e+02 & \first{1.29e+01}  & 3.16e+02 & \first{3.26e+01}  & 6.16e+02 & \first{4.12e+01}  & 1.11e+03 & \first{7.78e+01}  & 4.14e+03 & 2.24e+02\\
 & LS-Uniform & 3.46e+01 & 8.99e+00  & 1.70e+01 & 3.87e+00  & \first{2.27e+01} & 4.40e+00  & 5.05e+01 & 9.25e+00  & \first{1.12e+02} & 1.38e+01  & 5.30e+02 & 3.27e+01  & \first{4.39e+02} & 4.64e+01  & 1.25e+03 & 9.28e+01  & \first{3.36e+03} & \first{1.93e+02}\\
 & LS-Chebyshev & \first{3.47e+00} & 1.27e+00  & \first{6.97e+00} & 1.75e+00  & 2.49e+01 & 5.10e+00  & 4.93e+01 & \first{7.89e+00}  & 1.45e+02 & 4.46e+01  & \first{2.55e+02} & 5.16e+01  & 5.56e+02 & 8.63e+01  & \first{1.06e+03} & 1.61e+02  & 3.79e+03 & 4.90e+02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 5.81e-01 & 2.39e-01  & 6.32e-01 & 2.17e-01  & 6.42e-01 & 1.75e-01  & 6.92e-01 & 1.18e-01  & \first{5.74e-01} & 1.63e-01  & 8.19e-01 & 8.12e-02  & \first{5.52e-01} & 1.32e-01  & 5.85e-01 & 1.46e-01  & 7.29e-01 & 8.59e-02\\
 & LS-Uniform & 3.13e+00 & 7.97e-01  & 1.66e+00 & 2.82e-01  & 8.28e-01 & 1.35e-01  & \first{5.93e-01} & 9.65e-02  & 7.27e-01 & 1.11e-01  & \first{6.16e-01} & \first{6.05e-02}  & 5.90e-01 & \first{5.49e-02}  & \first{5.43e-01} & 4.69e-02  & \first{5.32e-01} & \first{4.63e-02}\\
 & LS-Chebyshev & \first{4.84e-01} & \first{1.75e-01}  & \first{4.91e-01} & \first{1.28e-01}  & \first{5.90e-01} & \first{9.71e-02}  & 6.71e-01 & \first{8.36e-02}  & 6.30e-01 & \first{9.58e-02}  & 6.45e-01 & 7.00e-02  & 6.10e-01 & 7.08e-02  & 5.99e-01 & \first{4.31e-02}  & 7.05e-01 & 5.57e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 1.09e-02 & 5.50e-03  & 2.27e-02 & 7.18e-03  & \first{8.36e-02} & 2.25e-02  & \first{2.20e-02} & 5.62e-03  & \first{9.67e-02} & 2.23e-02  & 2.12e-01 & 3.39e-02  & \first{7.50e-02} & 1.68e-02  & 1.54e-01 & 3.18e-02  & 2.11e-01 & 3.30e-02\\
 & LS-Uniform & \first{7.18e-03} & \first{1.52e-03}  & 4.56e-02 & \first{6.02e-03}  & 1.03e-01 & \first{1.27e-02}  & 3.12e-02 & \first{4.22e-03}  & 1.24e-01 & \first{1.62e-02}  & 2.46e-01 & \first{1.96e-02}  & 8.86e-02 & \first{1.09e-02}  & \first{1.28e-01} & \first{1.48e-02}  & \first{1.33e-01} & \first{1.46e-02}\\
 & LS-Chebyshev & 9.32e-03 & 4.52e-03  & \first{2.22e-02} & 6.15e-03  & 1.03e-01 & 3.31e-02  & 2.24e-02 & 8.09e-03  & 1.04e-01 & 2.51e-02  & \first{1.69e-01} & 4.66e-02  & 1.03e-01 & 2.53e-02  & 1.58e-01 & 4.58e-02  & 1.70e-01 & 3.77e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 6.00e-07 & 3.07e-07  & 9.86e-07 & 3.43e-07  & 1.65e-06 & 4.23e-07  & 1.86e-06 & 5.11e-07  & 2.98e-06 & 6.30e-07  & 3.89e-06 & 7.36e-07  & 5.30e-06 & 8.86e-07  & 5.41e-06 & 1.18e-06  & 1.06e-05 & 1.74e-06\\
 & LS-Uniform & 4.11e-06 & 1.04e-06  & 1.75e-06 & 3.59e-07  & 1.45e-06 & 1.96e-07  & 1.13e-06 & \first{1.76e-07}  & 1.09e-06 & \first{1.62e-07}  & 1.03e-06 & \first{1.40e-07}  & 9.18e-07 & \first{1.34e-07}  & 1.03e-06 & \first{1.31e-07}  & 7.99e-07 & \first{1.25e-07}\\
 & LS-Chebyshev & \first{5.59e-07} & \first{2.36e-07}  & \first{6.16e-07} & \first{1.70e-07}  & \first{6.18e-07} & \first{1.75e-07}  & \first{8.94e-07} & 1.77e-07  & \first{7.27e-07} & 1.73e-07  & \first{6.94e-07} & 1.70e-07  & \first{7.69e-07} & 1.75e-07  & \first{7.20e-07} & 1.85e-07  & \first{7.85e-07} & 1.77e-07\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & \first{3.97e-02} & 2.52e-02  & \first{4.60e-01} & \first{1.54e-01}  & \first{1.73e+00} & \first{3.71e-01}  & \first{3.16e+00} & \first{6.35e-01}  & 8.22e+00 & \first{9.31e-01}  & 1.07e+01 & 1.22e+00  & 1.74e+01 & 1.53e+00  & 2.42e+01 & 2.27e+00  & 4.10e+01 & 3.10e+00\\
 & LS-Uniform & 1.69e-01 & 3.71e-02  & 1.12e+00 & 2.40e-01  & 2.57e+00 & 4.73e-01  & 7.47e+00 & 8.13e-01  & 7.38e+00 & 9.44e-01  & 1.10e+01 & \first{1.12e+00}  & 1.07e+01 & \first{1.20e+00}  & 8.54e+00 & \first{1.15e+00}  & 6.72e+00 & \first{1.12e+00}\\
 & LS-Chebyshev & 4.57e-02 & \first{1.78e-02}  & 6.95e-01 & 1.94e-01  & 2.99e+00 & 6.38e-01  & 3.93e+00 & 1.02e+00  & \first{5.68e+00} & 1.28e+00  & \first{6.02e+00} & 1.39e+00  & \first{5.75e+00} & 1.45e+00  & \first{6.95e+00} & 1.52e+00  & \first{6.05e+00} & 1.46e+00\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & \first{1.04e-03} & 6.17e-04  & 3.13e-03 & 1.28e-03  & 7.49e-03 & 1.86e-03  & 9.44e-03 & 1.67e-03  & \first{9.11e-03} & \first{1.58e-03}  & \first{8.35e-03} & \first{1.62e-03}  & \first{1.07e-02} & 1.34e-03  & \first{1.05e-02} & 1.84e-03  & \first{1.53e-02} & 1.89e-03\\
 & LS-Uniform & 4.27e-03 & 9.86e-04  & 9.12e-03 & 1.56e-03  & 7.81e-03 & \first{1.60e-03}  & \first{7.66e-03} & \first{1.25e-03}  & 1.96e-02 & 1.84e-03  & 1.49e-02 & 1.82e-03  & 1.70e-02 & \first{1.32e-03}  & 1.62e-02 & \first{1.52e-03}  & 3.22e-02 & \first{1.41e-03}\\
 & LS-Chebyshev & 1.05e-03 & \first{5.03e-04}  & \first{2.53e-03} & \first{1.04e-03}  & \first{6.16e-03} & 2.04e-03  & 9.17e-03 & 2.19e-03  & 1.50e-02 & 2.60e-03  & 1.38e-02 & 2.93e-03  & 1.87e-02 & 2.34e-03  & 2.39e-02 & 3.22e-03  & 1.99e-02 & 2.59e-03\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 2.48e-01 & 1.05e-01  & 6.03e-01 & 1.98e-01  & 1.70e+00 & 3.83e-01  & 2.92e+00 & 6.22e-01  & 6.46e+00 & 9.21e-01  & 1.64e+01 & 1.22e+00  & 2.29e+01 & 1.85e+00  & 4.61e+01 & 2.46e+00  & 4.96e+01 & 2.83e+00\\
 & LS-Uniform & 1.29e+00 & 3.18e-01  & 1.09e+00 & 2.25e-01  & 2.06e+00 & \first{2.88e-01}  & 2.32e+00 & \first{4.64e-01}  & \first{3.24e+00} & \first{5.50e-01}  & 7.44e+00 & \first{7.64e-01}  & \first{7.92e+00} & \first{1.30e+00}  & 1.93e+01 & \first{1.52e+00}  & \first{1.98e+01} & \first{1.64e+00}\\
 & LS-Chebyshev & \first{1.94e-01} & \first{6.80e-02}  & \first{5.43e-01} & \first{1.53e-01}  & \first{9.88e-01} & 3.53e-01  & \first{2.23e+00} & 6.17e-01  & 3.78e+00 & 8.72e-01  & \first{6.29e+00} & 1.45e+00  & 9.91e+00 & 2.75e+00  & \first{1.54e+01} & 4.25e+00  & 2.68e+01 & 6.33e+00\\
\bottomrule
\end{tabular}


==> tables/scale4.tex <==
% Created with Python on 2025-06-22 19:31:17
% ..\results\final_results\low_dim\results_numerical_experiments.csv, scale=4, dims = [2, 3, 4, 5, 6, 7, 8, 9, 10]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Dim2} & \multicolumn{2}{c}{Dim3} & \multicolumn{2}{c}{Dim4} & \multicolumn{2}{c}{Dim5} & \multicolumn{2}{c}{Dim6} & \multicolumn{2}{c}{Dim7} & \multicolumn{2}{c}{Dim8} & \multicolumn{2}{c}{Dim9} & \multicolumn{2}{c}{Dim10}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & \first{3.66e-01} & 1.55e-01  & \first{4.04e-01} & 1.43e-01  & 6.14e-01 & 1.27e-01  & 6.01e-01 & 9.79e-02  & 5.55e-01 & 1.10e-01  & 5.51e-01 & 6.38e-02  & 9.95e-01 & 1.66e-01  & 8.49e-01 & 1.23e-01  & 9.42e-01 & 1.45e-01\\
 & LS-Uniform & 5.12e+00 & 7.82e-01  & 1.33e+00 & 2.13e-01  & 1.15e+00 & 1.23e-01  & 1.01e+00 & 8.20e-02  & 1.28e+00 & 7.12e-02  & 7.04e-01 & 4.92e-02  & 6.54e-01 & \first{4.06e-02}  & 1.42e+00 & \first{4.23e-02}  & \first{4.85e-01} & \first{4.17e-02}\\
 & LS-Chebyshev & 4.20e-01 & \first{1.35e-01}  & 5.85e-01 & \first{1.25e-01}  & \first{5.03e-01} & \first{8.22e-02}  & \first{4.63e-01} & \first{6.17e-02}  & \first{5.40e-01} & \first{6.15e-02}  & \first{5.50e-01} & \first{4.78e-02}  & \first{5.80e-01} & 5.10e-02  & \first{5.48e-01} & 4.42e-02  & 5.97e-01 & 4.47e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 2.22e-02 & 5.15e-03  & \first{1.57e-02} & \first{3.66e-03}  & 1.51e-02 & 3.07e-03  & 1.60e-02 & 2.55e-03  & \first{1.37e-02} & \first{1.90e-03}  & 1.22e-02 & 1.95e-03  & \first{1.13e-02} & 1.89e-03  & 1.26e-02 & \first{1.74e-03}  & \first{9.30e-03} & 1.55e-03\\
 & LS-Uniform & 5.19e-01 & 7.51e-02  & 2.57e-02 & 4.94e-03  & 3.20e-02 & 3.45e-03  & 2.26e-02 & 3.14e-03  & 1.68e-02 & 2.30e-03  & 1.91e-02 & 1.94e-03  & 1.40e-02 & 1.80e-03  & 1.56e-02 & 1.86e-03  & 1.20e-02 & 1.48e-03\\
 & LS-Chebyshev & \first{1.84e-02} & \first{4.06e-03}  & 1.90e-02 & 4.16e-03  & \first{1.33e-02} & \first{2.72e-03}  & \first{1.45e-02} & \first{2.23e-03}  & 1.38e-02 & 2.15e-03  & \first{1.13e-02} & \first{1.78e-03}  & 1.26e-02 & \first{1.65e-03}  & \first{9.93e-03} & 1.86e-03  & 1.03e-02 & \first{1.45e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 1.48e-03 & 5.81e-04  & 3.03e-02 & 5.80e-03  & 8.14e-02 & 1.29e-02  & 2.47e-01 & 1.57e-02  & 1.80e-01 & 8.18e-03  & 3.63e-02 & 2.11e-03  & 7.79e-03 & 5.32e-04  & 1.49e-02 & 4.24e-04  & 5.66e-04 & \first{1.08e-05}\\
 & LS-Uniform & 3.50e-03 & 5.50e-04  & \first{8.54e-03} & \first{1.65e-03}  & 6.71e-02 & \first{4.08e-03}  & 1.21e-01 & \first{4.43e-03}  & 1.03e-01 & \first{2.87e-03}  & \first{2.17e-02} & \first{4.91e-04}  & \first{1.43e-03} & \first{9.33e-05}  & \first{6.29e-03} & \first{8.21e-05}  & \first{5.40e-04} & 1.26e-05\\
 & LS-Chebyshev & \first{1.42e-03} & \first{4.44e-04}  & 9.19e-03 & 2.33e-03  & \first{4.08e-02} & 7.06e-03  & \first{5.15e-02} & 1.30e-02  & \first{6.89e-02} & 9.41e-03  & 2.98e-02 & 4.26e-03  & 2.64e-02 & 3.62e-03  & 2.21e-02 & 3.34e-03  & 1.33e-03 & 2.53e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 3.82e+00 & 1.08e+00  & 1.11e+01 & \first{1.33e+00}  & 3.61e+01 & 3.29e+00  & \first{5.33e+01} & \first{5.79e+00}  & 1.67e+02 & 1.14e+01  & 3.15e+02 & \first{2.22e+01}  & 4.69e+02 & \first{3.33e+01}  & 1.84e+03 & \first{5.96e+01}  & 4.14e+03 & \first{1.37e+02}\\
 & LS-Uniform & 7.48e+01 & 1.09e+01  & 1.11e+01 & 1.66e+00  & \first{2.68e+01} & \first{3.24e+00}  & 6.57e+01 & 7.68e+00  & \first{1.27e+02} & \first{1.13e+01}  & 3.72e+02 & 2.34e+01  & 5.24e+02 & 4.03e+01  & \first{1.59e+03} & 7.37e+01  & \first{2.89e+03} & 1.43e+02\\
 & LS-Chebyshev & \first{3.59e+00} & \first{7.15e-01}  & \first{6.09e+00} & 1.37e+00  & 2.99e+01 & 3.74e+00  & 6.37e+01 & 6.57e+00  & 1.37e+02 & 2.16e+01  & \first{2.21e+02} & 4.58e+01  & \first{4.46e+02} & 6.56e+01  & 1.98e+03 & 1.45e+02  & 3.60e+03 & 3.37e+02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 3.51e-01 & 9.72e-02  & 4.54e-01 & 9.92e-02  & 4.80e-01 & 8.93e-02  & 5.59e-01 & 7.81e-02  & 5.92e-01 & 8.11e-02  & 6.49e-01 & 9.23e-02  & 6.66e-01 & 7.20e-02  & 9.05e-01 & 8.47e-02  & 6.10e-01 & 5.78e-02\\
 & LS-Uniform & 3.83e+00 & 5.77e-01  & 7.59e-01 & 9.70e-02  & 1.03e+00 & 7.53e-02  & 1.05e+00 & 8.73e-02  & 6.73e-01 & 5.92e-02  & 6.97e-01 & 3.99e-02  & 9.57e-01 & \first{3.33e-02}  & 8.32e-01 & 3.36e-02  & \first{5.28e-01} & \first{2.98e-02}\\
 & LS-Chebyshev & \first{3.40e-01} & \first{8.12e-02}  & \first{3.66e-01} & \first{7.08e-02}  & \first{4.10e-01} & \first{5.53e-02}  & \first{4.57e-01} & \first{5.40e-02}  & \first{5.16e-01} & \first{5.49e-02}  & \first{5.18e-01} & \first{3.70e-02}  & \first{5.32e-01} & 3.60e-02  & \first{5.93e-01} & \first{3.13e-02}  & 5.66e-01 & 3.15e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 2.80e-03 & \first{7.19e-04}  & \first{3.20e-03} & 8.34e-04  & 3.02e-02 & 5.43e-03  & 5.79e-03 & 9.61e-04  & 3.33e-02 & 4.40e-03  & \first{5.98e-02} & 9.17e-03  & 2.32e-02 & 3.01e-03  & \first{5.70e-02} & 8.03e-03  & 1.24e-01 & 1.11e-02\\
 & LS-Uniform & 5.70e-03 & 1.08e-03  & 4.19e-03 & \first{5.11e-04}  & \first{2.90e-02} & \first{2.50e-03}  & 6.55e-03 & \first{5.47e-04}  & 2.86e-02 & \first{3.13e-03}  & 6.28e-02 & \first{5.51e-03}  & 2.59e-02 & \first{1.87e-03}  & 7.95e-02 & \first{4.52e-03}  & 7.36e-02 & \first{4.07e-03}\\
 & LS-Chebyshev & \first{2.45e-03} & 9.90e-04  & 3.75e-03 & 1.06e-03  & 2.91e-02 & 7.40e-03  & \first{4.78e-03} & 7.64e-04  & \first{2.43e-02} & 5.71e-03  & 7.30e-02 & 1.61e-02  & \first{2.16e-02} & 4.55e-03  & 6.94e-02 & 1.42e-02  & \first{5.84e-02} & 1.26e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 6.46e-07 & 2.64e-07  & 1.25e-06 & 3.48e-07  & 2.09e-06 & 5.18e-07  & 2.72e-06 & 6.52e-07  & 4.34e-06 & 9.47e-07  & 7.43e-06 & 1.18e-06  & 1.10e-05 & 1.46e-06  & 1.23e-05 & 1.76e-06  & 2.09e-05 & 2.14e-06\\
 & LS-Uniform & 2.12e-05 & 3.07e-06  & 1.39e-06 & 2.47e-07  & 1.48e-06 & 1.88e-07  & 1.67e-06 & 1.92e-07  & 2.38e-06 & \first{1.61e-07}  & 2.18e-06 & \first{1.50e-07}  & 1.41e-06 & \first{1.42e-07}  & 1.69e-06 & \first{1.39e-07}  & 1.42e-06 & \first{1.31e-07}\\
 & LS-Chebyshev & \first{5.80e-07} & \first{1.97e-07}  & \first{6.21e-07} & \first{1.59e-07}  & \first{7.31e-07} & \first{1.71e-07}  & \first{7.39e-07} & \first{1.51e-07}  & \first{7.92e-07} & 1.63e-07  & \first{8.48e-07} & 1.70e-07  & \first{8.40e-07} & 1.63e-07  & \first{9.39e-07} & 1.73e-07  & \first{1.01e-06} & 1.76e-07\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & \first{2.12e-03} & 1.06e-03  & \first{8.77e-02} & 3.12e-02  & \first{6.40e-01} & 1.27e-01  & \first{1.96e+00} & \first{3.25e-01}  & 5.60e+00 & \first{5.52e-01}  & 9.41e+00 & 9.07e-01  & 1.66e+01 & 1.13e+00  & 3.33e+01 & 1.48e+00  & 4.89e+01 & 2.10e+00\\
 & LS-Uniform & 9.31e-03 & 1.42e-03  & 1.43e-01 & \first{1.71e-02}  & 1.12e+00 & \first{1.18e-01}  & 3.53e+00 & 3.44e-01  & 7.51e+00 & 6.52e-01  & 1.37e+01 & \first{7.95e-01}  & 1.22e+01 & \first{9.90e-01}  & 1.69e+01 & \first{1.07e+00}  & 1.70e+01 & \first{1.13e+00}\\
 & LS-Chebyshev & 2.53e-03 & \first{8.35e-04}  & 9.86e-02 & 2.25e-02  & 1.04e+00 & 2.00e-01  & 2.23e+00 & 5.68e-01  & \first{3.63e+00} & 9.07e-01  & \first{4.89e+00} & 1.17e+00  & \first{5.84e+00} & 1.27e+00  & \first{6.84e+00} & 1.41e+00  & \first{7.55e+00} & 1.44e+00\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & \first{8.63e-05} & 3.77e-05  & 4.30e-04 & 1.57e-04  & 1.17e-03 & 2.97e-04  & \first{1.51e-03} & 3.14e-04  & \first{2.55e-03} & 2.81e-04  & \first{2.36e-03} & 3.25e-04  & \first{3.01e-03} & 2.86e-04  & \first{3.58e-03} & 3.43e-04  & \first{4.83e-03} & 4.05e-04\\
 & LS-Uniform & 4.65e-04 & 7.06e-05  & 5.74e-04 & \first{7.52e-05}  & 3.43e-03 & \first{1.92e-04}  & 2.88e-03 & \first{2.89e-04}  & 4.56e-03 & \first{2.72e-04}  & 4.91e-03 & \first{3.00e-04}  & 4.71e-03 & \first{2.49e-04}  & 8.66e-03 & \first{3.02e-04}  & 8.72e-03 & \first{2.71e-04}\\
 & LS-Chebyshev & 1.01e-04 & \first{3.20e-05}  & \first{4.28e-04} & 1.07e-04  & \first{1.13e-03} & 2.97e-04  & 2.11e-03 & 3.67e-04  & 3.33e-03 & 3.93e-04  & 4.36e-03 & 5.51e-04  & 5.39e-03 & 4.65e-04  & 6.19e-03 & 5.25e-04  & 8.62e-03 & 5.31e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & \first{1.14e-01} & \first{3.85e-02}  & 4.75e-01 & 8.99e-02  & 1.30e+00 & 2.05e-01  & 2.40e+00 & 3.19e-01  & 6.57e+00 & 5.98e-01  & 1.34e+01 & 8.31e-01  & 2.60e+01 & 1.40e+00  & 4.11e+01 & 1.85e+00  & 6.16e+01 & 2.16e+00\\
 & LS-Uniform & 2.37e+00 & 3.45e-01  & 4.55e-01 & 9.45e-02  & 1.16e+00 & 1.47e-01  & 2.05e+00 & \first{2.24e-01}  & 4.09e+00 & \first{2.63e-01}  & 5.69e+00 & \first{4.08e-01}  & \first{6.54e+00} & \first{7.10e-01}  & 1.51e+01 & \first{8.92e-01}  & \first{1.61e+01} & \first{9.34e-01}\\
 & LS-Chebyshev & 1.17e-01 & 4.08e-02  & \first{3.43e-01} & \first{7.47e-02}  & \first{5.30e-01} & \first{1.27e-01}  & \first{1.26e+00} & 2.63e-01  & \first{3.10e+00} & 3.98e-01  & \first{3.24e+00} & 7.89e-01  & 6.68e+00 & 1.61e+00  & \first{1.39e+01} & 2.17e+00  & 1.98e+01 & 3.37e+00\\
\bottomrule
\end{tabular}


==> tables/scale5.tex <==
% Created with Python on 2025-06-22 19:31:17
% ..\results\final_results\low_dim\results_numerical_experiments.csv, scale=5, dims = [2, 3, 4, 5, 6, 7, 8, 9, 10]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Dim2} & \multicolumn{2}{c}{Dim3} & \multicolumn{2}{c}{Dim4} & \multicolumn{2}{c}{Dim5} & \multicolumn{2}{c}{Dim6} & \multicolumn{2}{c}{Dim7} & \multicolumn{2}{c}{Dim8} & \multicolumn{2}{c}{Dim9} & \multicolumn{2}{c}{Dim10}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 1.91e-01 & 7.14e-02  & 2.98e-01 & 8.74e-02  & 3.43e-01 & 8.48e-02  & 3.44e-01 & 6.83e-02  & 4.59e-01 & 6.18e-02  & 5.00e-01 & 4.12e-02  & 4.83e-01 & 7.72e-02  & 7.20e-01 & 5.77e-02  & 8.41e-01 & 6.38e-02\\
 & LS-Uniform & 3.56e+00 & 3.27e-01  & 8.83e-01 & 1.27e-01  & 1.10e+00 & 9.00e-02  & 1.05e+00 & 5.14e-02  & 7.96e-01 & 3.72e-02  & 2.33e+00 & 3.49e-02  & 8.87e-01 & \first{2.64e-02}  & 1.13e+00 & 2.90e-02  & 1.13e+00 & 2.66e-02\\
 & LS-Chebyshev & \first{1.87e-01} & \first{4.82e-02}  & \first{2.25e-01} & \first{5.65e-02}  & \first{2.35e-01} & \first{4.60e-02}  & \first{2.71e-01} & \first{3.30e-02}  & \first{4.19e-01} & \first{3.47e-02}  & \first{4.07e-01} & \first{2.92e-02}  & \first{4.61e-01} & 2.74e-02  & \first{4.36e-01} & \first{2.71e-02}  & \first{4.92e-01} & \first{2.57e-02}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 1.10e-02 & 1.58e-03  & 1.17e-02 & 1.68e-03  & 9.36e-03 & 1.03e-03  & 8.41e-03 & 8.77e-04  & 7.75e-03 & 7.71e-04  & 7.33e-03 & 7.47e-04  & 6.45e-03 & 6.21e-04  & \first{4.71e-03} & 7.08e-04  & \first{5.37e-03} & 6.20e-04\\
 & LS-Uniform & 3.64e-01 & 3.24e-02  & 3.90e-02 & 2.89e-03  & 1.81e-02 & 1.67e-03  & 1.63e-02 & 1.17e-03  & 1.09e-02 & 9.02e-04  & 1.35e-02 & 8.28e-04  & 9.09e-03 & 7.09e-04  & 1.33e-02 & 7.18e-04  & 1.07e-02 & 6.01e-04\\
 & LS-Chebyshev & \first{9.43e-03} & \first{1.45e-03}  & \first{7.98e-03} & \first{1.43e-03}  & \first{7.72e-03} & \first{9.94e-04}  & \first{6.89e-03} & \first{7.64e-04}  & \first{6.24e-03} & \first{7.46e-04}  & \first{5.84e-03} & \first{6.34e-04}  & \first{5.08e-03} & \first{6.01e-04}  & 5.37e-03 & \first{6.31e-04}  & 5.61e-03 & \first{5.39e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 1.04e-04 & 3.31e-05  & 7.48e-03 & 1.46e-03  & 5.39e-02 & 5.69e-03  & 1.25e-01 & 1.07e-02  & 2.53e-01 & 8.59e-03  & 1.06e-01 & 3.14e-03  & 4.59e-02 & 9.43e-04  & 3.07e-02 & 6.85e-04  & 1.16e-02 & 1.67e-04\\
 & LS-Uniform & 4.92e-04 & 5.98e-05  & 6.77e-03 & \first{3.90e-04}  & 2.02e-02 & \first{1.08e-03}  & 6.88e-02 & \first{1.49e-03}  & 7.82e-02 & \first{1.19e-03}  & 3.75e-02 & \first{4.28e-04}  & \first{9.09e-03} & \first{7.55e-05}  & \first{5.84e-03} & \first{3.80e-05}  & \first{9.89e-04} & \first{9.84e-06}\\
 & LS-Chebyshev & \first{8.77e-05} & \first{2.65e-05}  & \first{2.31e-03} & 4.72e-04  & \first{1.23e-02} & 2.09e-03  & \first{2.44e-02} & 4.49e-03  & \first{2.50e-02} & 4.35e-03  & \first{2.76e-02} & 3.68e-03  & 2.40e-02 & 2.21e-03  & 1.46e-02 & 1.54e-03  & 4.98e-03 & 3.72e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 4.82e+00 & 8.42e-01  & 7.35e+00 & \first{1.03e+00}  & 3.36e+01 & 2.59e+00  & 5.18e+01 & \first{4.33e+00}  & 1.38e+02 & \first{7.79e+00}  & 3.21e+02 & \first{1.78e+01}  & 1.00e+03 & \first{2.78e+01}  & 1.62e+03 & \first{4.44e+01}  & 2.92e+03 & \first{1.00e+02}\\
 & LS-Uniform & 6.02e+01 & 6.33e+00  & 2.38e+01 & 1.67e+00  & 5.96e+01 & 3.33e+00  & 7.06e+01 & 5.40e+00  & 1.42e+02 & 9.37e+00  & 4.73e+02 & 1.82e+01  & \first{7.67e+02} & 3.26e+01  & \first{1.57e+03} & 5.85e+01  & 2.62e+03 & 1.13e+02\\
 & LS-Chebyshev & \first{4.24e+00} & \first{6.58e-01}  & \first{5.86e+00} & 1.04e+00  & \first{2.35e+01} & \first{2.33e+00}  & \first{5.03e+01} & 4.62e+00  & \first{1.01e+02} & 1.07e+01  & \first{2.45e+02} & 2.90e+01  & 8.71e+02 & 4.60e+01  & 1.73e+03 & 9.91e+01  & \first{2.60e+03} & 2.30e+02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 1.18e-01 & 3.11e-02  & \first{2.21e-01} & 3.99e-02  & 3.24e-01 & 4.70e-02  & 4.13e-01 & 6.14e-02  & 4.88e-01 & 4.00e-02  & 5.66e-01 & 3.82e-02  & 5.10e-01 & 4.32e-02  & 5.07e-01 & 4.52e-02  & 5.69e-01 & 3.47e-02\\
 & LS-Uniform & 3.44e+00 & 2.92e-01  & 7.69e-01 & 6.15e-02  & 1.01e+00 & 5.19e-02  & 1.11e+00 & 3.93e-02  & 9.13e-01 & 3.42e-02  & 9.40e-01 & 2.56e-02  & 7.75e-01 & 2.12e-02  & 8.26e-01 & 2.38e-02  & 1.01e+00 & \first{1.82e-02}\\
 & LS-Chebyshev & \first{6.74e-02} & \first{1.90e-02}  & 2.59e-01 & \first{2.74e-02}  & \first{2.14e-01} & \first{2.71e-02}  & \first{2.64e-01} & \first{2.75e-02}  & \first{3.05e-01} & \first{2.89e-02}  & \first{3.33e-01} & \first{2.22e-02}  & \first{4.23e-01} & \first{2.02e-02}  & \first{4.24e-01} & \first{2.10e-02}  & \first{4.67e-01} & 1.96e-02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & \first{3.70e-04} & \first{7.25e-05}  & 3.76e-04 & 6.70e-05  & 9.51e-03 & 1.15e-03  & 1.28e-03 & 1.42e-04  & 6.61e-03 & 6.20e-04  & 1.69e-02 & 1.66e-03  & 6.07e-03 & 5.67e-04  & \first{1.56e-02} & 1.37e-03  & 5.30e-02 & 3.61e-03\\
 & LS-Uniform & 1.33e-03 & 1.36e-04  & 5.38e-04 & \first{4.27e-05}  & 1.35e-02 & \first{5.94e-04}  & 1.46e-03 & \first{6.65e-05}  & 8.01e-03 & \first{3.48e-04}  & 2.67e-02 & \first{9.99e-04}  & \first{3.50e-03} & \first{2.15e-04}  & 2.44e-02 & \first{8.86e-04}  & 2.87e-02 & \first{8.66e-04}\\
 & LS-Chebyshev & 5.63e-04 & 9.85e-05  & \first{2.48e-04} & 7.25e-05  & \first{5.91e-03} & 1.19e-03  & \first{5.93e-04} & 1.02e-04  & \first{5.20e-03} & 9.03e-04  & \first{1.53e-02} & 2.97e-03  & 4.17e-03 & 5.71e-04  & 1.70e-02 & 2.74e-03  & \first{1.60e-02} & 2.92e-03\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 7.78e-07 & 2.43e-07  & 1.44e-06 & 4.06e-07  & 2.63e-06 & 5.34e-07  & 4.71e-06 & 7.87e-07  & 8.13e-06 & 1.08e-06  & 1.29e-05 & 1.44e-06  & 1.77e-05 & 1.94e-06  & 2.59e-05 & 2.62e-06  & 3.98e-05 & 3.22e-06\\
 & LS-Uniform & 1.98e-05 & 2.30e-06  & 3.84e-06 & 3.29e-07  & 3.94e-06 & 2.58e-07  & 3.03e-06 & 1.90e-07  & 2.97e-06 & 1.74e-07  & 4.86e-06 & 1.72e-07  & 3.08e-06 & \first{1.58e-07}  & 3.67e-06 & \first{1.53e-07}  & 3.67e-06 & \first{1.47e-07}\\
 & LS-Chebyshev & \first{7.30e-07} & \first{1.51e-07}  & \first{6.35e-07} & \first{1.49e-07}  & \first{7.82e-07} & \first{1.49e-07}  & \first{7.12e-07} & \first{1.48e-07}  & \first{7.93e-07} & \first{1.57e-07}  & \first{9.50e-07} & \first{1.58e-07}  & \first{9.82e-07} & 1.61e-07  & \first{1.14e-06} & 1.65e-07  & \first{1.15e-06} & 1.70e-07\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & \first{4.48e-05} & 1.87e-05  & 9.48e-03 & 3.25e-03  & 1.47e-01 & 3.57e-02  & 8.12e-01 & 1.37e-01  & 2.34e+00 & 2.79e-01  & 5.95e+00 & 5.23e-01  & 1.42e+01 & 7.29e-01  & 2.19e+01 & 1.12e+00  & 4.38e+01 & 1.44e+00\\
 & LS-Uniform & 1.97e-04 & 3.00e-05  & 2.46e-02 & 1.93e-03  & 3.74e-01 & \first{2.14e-02}  & 1.87e+00 & \first{8.95e-02}  & 6.52e+00 & \first{2.55e-01}  & 2.03e+01 & \first{4.98e-01}  & 1.71e+01 & \first{7.00e-01}  & 3.41e+01 & \first{8.90e-01}  & 4.13e+01 & \first{1.09e+00}\\
 & LS-Chebyshev & 5.56e-05 & \first{1.33e-05}  & \first{8.00e-03} & \first{1.65e-03}  & \first{1.19e-01} & 2.60e-02  & \first{7.15e-01} & 1.66e-01  & \first{2.31e+00} & 4.57e-01  & \first{4.09e+00} & 7.94e-01  & \first{5.79e+00} & 1.09e+00  & \first{6.82e+00} & 1.24e+00  & \first{7.39e+00} & 1.34e+00\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & 3.51e-06 & 1.24e-06  & 4.39e-05 & 1.56e-05  & 1.95e-04 & 4.47e-05  & \first{3.04e-04} & 5.54e-05  & \first{3.29e-04} & 4.74e-05  & \first{5.73e-04} & 6.41e-05  & \first{1.05e-03} & 6.48e-05  & \first{9.39e-04} & 6.33e-05  & \first{1.79e-03} & 6.80e-05\\
 & LS-Uniform & 1.99e-05 & 2.55e-06  & 8.01e-05 & \first{8.11e-06}  & 3.59e-04 & \first{2.02e-05}  & 1.22e-03 & \first{3.95e-05}  & 7.60e-04 & \first{2.89e-05}  & 8.68e-04 & \first{4.60e-05}  & 1.48e-03 & \first{4.39e-05}  & 2.92e-03 & \first{4.69e-05}  & 3.74e-03 & \first{5.71e-05}\\
 & LS-Chebyshev & \first{3.45e-06} & \first{8.70e-07}  & \first{3.82e-05} & 8.14e-06  & \first{1.08e-04} & 2.55e-05  & 3.62e-04 & 4.76e-05  & 4.72e-04 & 4.64e-05  & 7.29e-04 & 7.56e-05  & 1.11e-03 & 8.02e-05  & 1.35e-03 & 8.90e-05  & 2.12e-03 & 9.73e-05\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & \first{6.89e-02} & 1.54e-02  & 2.08e-01 & 4.03e-02  & 7.02e-01 & 8.54e-02  & 1.80e+00 & 1.67e-01  & 4.06e+00 & 3.12e-01  & 9.61e+00 & 4.93e-01  & 1.89e+01 & 9.00e-01  & 3.73e+01 & 1.30e+00  & 4.62e+01 & 1.64e+00\\
 & LS-Uniform & 1.61e+00 & 1.67e-01  & 4.46e-01 & 4.71e-02  & 1.02e+00 & 9.01e-02  & 1.88e+00 & 1.10e-01  & 2.21e+00 & \first{1.33e-01}  & 3.73e+00 & \first{2.25e-01}  & 5.65e+00 & \first{3.95e-01}  & 1.48e+01 & \first{4.86e-01}  & 1.40e+01 & \first{5.31e-01}\\
 & LS-Chebyshev & 8.27e-02 & \first{1.14e-02}  & \first{1.98e-01} & \first{3.08e-02}  & \first{2.94e-01} & \first{5.48e-02}  & \first{9.49e-01} & \first{1.02e-01}  & \first{1.66e+00} & 1.80e-01  & \first{2.17e+00} & 3.60e-01  & \first{4.08e+00} & 7.55e-01  & \first{8.35e+00} & 1.18e+00  & \first{1.00e+01} & 1.63e+00\\
\bottomrule
\end{tabular}


==> tables/scale6.tex <==
% Created with Python on 2025-06-22 19:31:18
% ..\results\final_results\low_dim\results_numerical_experiments.csv, scale=6, dims = [2, 3, 4, 5, 6, 7, 8, 9, 10]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Dim2} & \multicolumn{2}{c}{Dim3} & \multicolumn{2}{c}{Dim4} & \multicolumn{2}{c}{Dim5} & \multicolumn{2}{c}{Dim6} & \multicolumn{2}{c}{Dim7} & \multicolumn{2}{c}{Dim8} & \multicolumn{2}{c}{Dim9} & \multicolumn{2}{c}{Dim10}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 3.33e-02 & 9.39e-03  & 1.06e-01 & 2.28e-02  & 1.77e-01 & 4.25e-02  & 2.10e-01 & 3.35e-02  & 3.38e-01 & 2.96e-02  & 3.37e-01 & 2.24e-02  & 3.37e-01 & 3.80e-02  & 3.17e-01 & 2.91e-02  & 4.33e-01 & 4.68e-02\\
 & LS-Uniform & 8.19e+00 & 7.13e-01  & 1.37e+00 & 6.60e-02  & 7.49e-01 & 3.09e-02  & 1.27e+00 & 2.76e-02  & 8.97e-01 & 2.03e-02  & 1.17e+00 & 2.44e-02  & 1.06e+00 & 1.82e-02  & 1.43e+00 & 1.83e-02  & 1.52e+00 & 1.71e-02\\
 & LS-Chebyshev & \first{2.24e-02} & \first{6.11e-03}  & \first{7.17e-02} & \first{1.27e-02}  & \first{1.18e-01} & \first{1.95e-02}  & \first{1.56e-01} & \first{1.79e-02}  & \first{2.04e-01} & \first{1.63e-02}  & \first{2.38e-01} & \first{1.64e-02}  & \first{2.74e-01} & \first{1.46e-02}  & \first{2.98e-01} & \first{1.59e-02}  & \first{3.66e-01} & \first{1.55e-02}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 5.23e-03 & 6.18e-04  & \first{4.17e-03} & \first{4.94e-04}  & 4.98e-03 & 4.84e-04  & 3.68e-03 & 3.27e-04  & \first{3.31e-03} & 3.30e-04  & 4.32e-03 & 2.83e-04  & 3.25e-03 & 2.40e-04  & 3.44e-03 & 2.55e-04  & 2.79e-03 & \first{1.92e-04}\\
 & LS-Uniform & 6.88e-01 & 6.27e-02  & 5.98e-02 & 2.11e-03  & 1.81e-02 & 7.44e-04  & 1.36e-02 & 4.58e-04  & 1.16e-02 & 3.73e-04  & 1.17e-02 & 3.24e-04  & 5.86e-03 & 2.80e-04  & 9.70e-03 & 2.93e-04  & 6.48e-03 & 2.37e-04\\
 & LS-Chebyshev & \first{4.69e-03} & \first{4.91e-04}  & 5.42e-03 & 5.28e-04  & \first{3.78e-03} & \first{3.61e-04}  & \first{3.13e-03} & \first{2.85e-04}  & 3.75e-03 & \first{2.59e-04}  & \first{2.99e-03} & \first{2.35e-04}  & \first{2.85e-03} & \first{2.17e-04}  & \first{2.60e-03} & \first{2.33e-04}  & \first{2.34e-03} & 1.95e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & 8.90e-07 & 2.61e-07  & 1.44e-03 & 2.55e-04  & 1.89e-02 & 2.32e-03  & 7.94e-02 & 5.60e-03  & 1.44e-01 & 5.65e-03  & 1.36e-01 & 3.50e-03  & 4.68e-02 & 1.34e-03  & 4.38e-02 & 8.63e-04  & 2.88e-02 & 4.11e-04\\
 & LS-Uniform & 2.30e-04 & 2.04e-05  & 2.03e-03 & 1.02e-04  & 8.63e-03 & \first{2.20e-04}  & 1.91e-02 & \first{4.54e-04}  & 7.77e-02 & \first{6.63e-04}  & 6.35e-02 & \first{4.00e-04}  & \first{7.43e-03} & \first{7.63e-05}  & 2.55e-02 & \first{8.50e-05}  & \first{2.38e-03} & \first{8.90e-06}\\
 & LS-Chebyshev & \first{6.13e-07} & \first{1.70e-07}  & \first{3.68e-04} & \first{8.59e-05}  & \first{2.51e-03} & 4.46e-04  & \first{8.78e-03} & 1.20e-03  & \first{1.75e-02} & 2.11e-03  & \first{1.62e-02} & 1.41e-03  & 1.56e-02 & 9.77e-04  & \first{1.97e-02} & 1.03e-03  & 6.19e-03 & 3.31e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 4.56e+00 & 6.75e-01  & 9.26e+00 & 8.10e-01  & 2.92e+01 & 1.96e+00  & 6.96e+01 & \first{3.59e+00}  & 1.31e+02 & \first{5.95e+00}  & 2.93e+02 & \first{1.29e+01}  & 8.55e+02 & \first{2.15e+01}  & 2.28e+03 & \first{3.75e+01}  & 5.01e+03 & \first{7.81e+01}\\
 & LS-Uniform & 3.07e+02 & 2.72e+01  & 6.09e+01 & 2.57e+00  & 4.40e+01 & 3.05e+00  & 1.27e+02 & 4.79e+00  & 2.74e+02 & 8.39e+00  & 3.96e+02 & 1.51e+01  & 8.95e+02 & 2.75e+01  & \first{1.85e+03} & 4.80e+01  & 4.37e+03 & 9.03e+01\\
 & LS-Chebyshev & \first{3.44e+00} & \first{4.35e-01}  & \first{7.10e+00} & \first{7.63e-01}  & \first{2.49e+01} & \first{1.78e+00}  & \first{5.36e+01} & 3.66e+00  & \first{1.08e+02} & 7.36e+00  & \first{2.71e+02} & 2.14e+01  & \first{8.14e+02} & 3.56e+01  & 2.05e+03 & 7.17e+01  & \first{3.39e+03} & 1.75e+02\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 2.17e-02 & 5.03e-03  & 1.20e-01 & 1.72e-02  & 1.98e-01 & 2.07e-02  & 2.36e-01 & 2.39e-02  & 3.05e-01 & 2.13e-02  & 4.27e-01 & 1.90e-02  & 3.42e-01 & 2.35e-02  & 3.81e-01 & 2.74e-02  & 4.24e-01 & 2.04e-02\\
 & LS-Uniform & 7.53e+00 & 6.71e-01  & 6.03e-01 & 3.04e-02  & 1.30e+00 & 2.99e-02  & 6.08e-01 & 1.70e-02  & 1.40e+00 & 1.85e-02  & 1.90e+00 & 1.90e-02  & 8.86e-01 & 1.30e-02  & 1.39e+00 & 1.49e-02  & 9.98e-01 & 1.08e-02\\
 & LS-Chebyshev & \first{1.67e-02} & \first{3.37e-03}  & \first{9.23e-02} & \first{8.81e-03}  & \first{1.08e-01} & \first{1.13e-02}  & \first{1.49e-01} & \first{1.25e-02}  & \first{1.69e-01} & \first{1.34e-02}  & \first{2.45e-01} & \first{1.22e-02}  & \first{2.45e-01} & \first{1.11e-02}  & \first{2.95e-01} & \first{1.27e-02}  & \first{3.04e-01} & \first{1.07e-02}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 4.84e-05 & 8.72e-06  & 2.58e-05 & 4.08e-06  & 2.33e-03 & 2.05e-04  & 1.84e-04 & 1.79e-05  & 1.20e-03 & 1.12e-04  & 5.02e-03 & 3.01e-04  & 1.60e-03 & 1.05e-04  & 3.57e-03 & 1.52e-04  & 1.45e-02 & 1.10e-03\\
 & LS-Uniform & 3.29e-03 & 2.95e-04  & 5.83e-05 & 3.24e-06  & 5.62e-03 & \first{1.27e-04}  & 3.74e-04 & \first{8.14e-06}  & 4.62e-03 & \first{5.96e-05}  & 5.91e-03 & \first{1.25e-04}  & 1.94e-03 & \first{2.84e-05}  & 4.25e-03 & \first{8.22e-05}  & 1.27e-02 & \first{1.82e-04}\\
 & LS-Chebyshev & \first{3.23e-05} & \first{7.11e-06}  & \first{1.39e-05} & \first{3.05e-06}  & \first{8.35e-04} & 2.12e-04  & \first{6.03e-05} & 1.21e-05  & \first{7.05e-04} & 9.40e-05  & \first{2.32e-03} & 3.96e-04  & \first{3.78e-04} & 6.69e-05  & \first{2.24e-03} & 2.98e-04  & \first{7.23e-03} & 8.24e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & \first{8.85e-07} & 2.38e-07  & 1.80e-06 & 4.04e-07  & 4.27e-06 & 6.76e-07  & 6.50e-06 & 9.68e-07  & 1.08e-05 & 1.42e-06  & 1.83e-05 & 1.99e-06  & 2.64e-05 & 2.67e-06  & 3.88e-05 & 3.57e-06  & 6.21e-05 & 4.71e-06\\
 & LS-Uniform & 2.21e-04 & 2.00e-05  & 2.20e-05 & 8.19e-07  & 6.85e-06 & 2.78e-07  & 7.35e-06 & 2.27e-07  & 8.25e-06 & 2.14e-07  & 7.99e-06 & 1.94e-07  & 6.80e-06 & 1.81e-07  & 1.05e-05 & 1.74e-07  & 5.65e-06 & \first{1.65e-07}\\
 & LS-Chebyshev & 1.13e-06 & \first{1.47e-07}  & \first{8.77e-07} & \first{1.46e-07}  & \first{8.05e-07} & \first{1.38e-07}  & \first{8.82e-07} & \first{1.48e-07}  & \first{8.30e-07} & \first{1.49e-07}  & \first{1.07e-06} & \first{1.55e-07}  & \first{1.08e-06} & \first{1.61e-07}  & \first{1.33e-06} & \first{1.65e-07}  & \first{1.29e-06} & 1.68e-07\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & 9.42e-09 & 3.35e-09  & 5.94e-04 & 1.77e-04  & 2.27e-02 & 5.91e-03  & 1.98e-01 & 3.66e-02  & 9.08e-01 & 1.15e-01  & 3.24e+00 & 2.56e-01  & 1.29e+01 & 4.34e-01  & 2.13e+01 & 7.17e-01  & 4.67e+01 & 9.71e-01\\
 & LS-Uniform & 2.71e-06 & 2.40e-07  & 2.61e-03 & 1.24e-04  & 8.01e-02 & \first{2.14e-03}  & 1.44e+00 & \first{2.34e-02}  & 4.17e+00 & \first{8.02e-02}  & 1.55e+01 & \first{2.40e-01}  & 2.00e+01 & \first{4.00e-01}  & 4.13e+01 & \first{6.09e-01}  & 6.83e+01 & \first{8.65e-01}\\
 & LS-Chebyshev & \first{7.69e-09} & \first{2.20e-09}  & \first{3.41e-04} & \first{7.41e-05}  & \first{1.21e-02} & 2.29e-03  & \first{1.56e-01} & 3.08e-02  & \first{7.52e-01} & 1.33e-01  & \first{2.75e+00} & 4.25e-01  & \first{4.52e+00} & 7.55e-01  & \first{6.29e+00} & 9.71e-01  & \first{8.18e+00} & 1.20e+00\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & 2.27e-08 & 7.41e-09  & 3.80e-06 & 1.11e-06  & 2.37e-05 & 5.74e-06  & 4.84e-05 & 8.17e-06  & \first{5.42e-05} & 7.37e-06  & \first{1.18e-04} & 1.13e-05  & \first{2.19e-04} & 1.16e-05  & \first{1.40e-04} & 1.04e-05  & \first{2.96e-04} & 1.34e-05\\
 & LS-Uniform & 7.28e-06 & 6.43e-07  & 1.44e-05 & 7.00e-07  & 7.85e-05 & 2.11e-06  & 2.85e-04 & 5.28e-06  & 3.73e-04 & \first{4.33e-06}  & 3.77e-04 & \first{6.61e-06}  & 1.19e-03 & \first{7.35e-06}  & 9.15e-04 & \first{7.01e-06}  & 1.61e-03 & \first{1.08e-05}\\
 & LS-Chebyshev & \first{1.81e-08} & \first{4.66e-09}  & \first{2.77e-06} & \first{5.03e-07}  & \first{1.09e-05} & \first{2.09e-06}  & \first{4.66e-05} & \first{4.97e-06}  & 8.14e-05 & 5.99e-06  & 1.61e-04 & 1.14e-05  & 2.30e-04 & 1.16e-05  & 2.73e-04 & 1.25e-05  & 5.25e-04 & 1.85e-05\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & \first{3.42e-02} & 5.39e-03  & 1.18e-01 & 1.54e-02  & 3.40e-01 & 3.77e-02  & 8.60e-01 & 8.16e-02  & 1.86e+00 & 1.60e-01  & 5.26e+00 & 2.66e-01  & 1.10e+01 & 5.33e-01  & 2.35e+01 & 7.50e-01  & 5.71e+01 & 1.08e+00\\
 & LS-Uniform & 9.01e+00 & 7.85e-01  & 9.80e-01 & 3.95e-02  & 1.02e+00 & 3.59e-02  & 1.40e+00 & 5.16e-02  & 1.91e+00 & \first{7.53e-02}  & 3.20e+00 & \first{1.20e-01}  & 5.08e+00 & \first{2.09e-01}  & 8.80e+00 & \first{2.75e-01}  & 1.15e+01 & \first{2.94e-01}\\
 & LS-Chebyshev & 4.75e-02 & \first{4.39e-03}  & \first{9.31e-02} & \first{1.15e-02}  & \first{2.30e-01} & \first{2.59e-02}  & \first{3.85e-01} & \first{4.24e-02}  & \first{7.14e-01} & 7.62e-02  & \first{1.98e+00} & 1.62e-01  & \first{2.58e+00} & 3.53e-01  & \first{4.76e+00} & 5.52e-01  & \first{7.43e+00} & 7.75e-01\\
\bottomrule
\end{tabular}


==> tables/scale7.tex <==
% Created with Python on 2025-06-22 19:31:18
% ..\results\final_results\low_dim\results_numerical_experiments.csv, scale=7, dims = [2, 3, 4, 5, 6, 7]
\begin{tabular}{ll|rr|rr|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Dim2} & \multicolumn{2}{c}{Dim3} & \multicolumn{2}{c}{Dim4} & \multicolumn{2}{c}{Dim5} & \multicolumn{2}{c}{Dim6} & \multicolumn{2}{c}{Dim7}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 2.47e-03 & 6.16e-04  & 2.71e-02 & 5.99e-03  & 1.01e-01 & 1.36e-02  & 1.14e-01 & 1.41e-02  & 1.88e-01 & 1.22e-02  & 2.08e-01 & 1.29e-02\\
 & LS-Uniform & 3.15e+02 & 1.41e+01  & 7.62e-01 & 2.36e-02  & 4.71e-01 & 1.36e-02  & 1.21e+00 & 1.35e-02  & 7.20e-01 & 1.21e-02  & 1.85e+00 & 1.71e-02\\
 & LS-Chebyshev & \first{1.52e-03} & \first{4.10e-04}  & \first{2.26e-02} & \first{2.86e-03}  & \first{4.77e-02} & \first{6.20e-03}  & \first{6.91e-02} & \first{7.30e-03}  & \first{1.18e-01} & \first{7.75e-03}  & \first{1.49e-01} & \first{9.16e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 2.68e-03 & 2.17e-04  & 3.22e-03 & 1.92e-04  & 2.80e-03 & 1.64e-04  & 2.18e-03 & 1.31e-04  & 1.78e-03 & 1.10e-04  & 1.78e-03 & 1.08e-04\\
 & LS-Uniform & 5.86e+02 & 2.69e+01  & 5.33e-02 & 1.49e-03  & 1.05e-02 & 3.41e-04  & 6.62e-03 & 2.06e-04  & 5.36e-03 & 1.60e-04  & 6.02e-03 & 1.35e-04\\
 & LS-Chebyshev & \first{2.08e-03} & \first{1.85e-04}  & \first{2.11e-03} & \first{1.81e-04}  & \first{2.23e-03} & \first{1.29e-04}  & \first{1.42e-03} & \first{1.02e-04}  & \first{1.58e-03} & \first{9.33e-05}  & \first{1.74e-03} & \first{8.47e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & \first{6.08e-09} & 1.75e-09  & 1.98e-04 & 2.96e-05  & 6.42e-03 & 6.42e-04  & 3.98e-02 & 2.24e-03  & 1.07e-01 & 4.41e-03  & 1.45e-01 & 3.08e-03\\
 & LS-Uniform & 6.80e-04 & 3.05e-05  & 1.40e-03 & 3.23e-05  & 6.64e-03 & \first{8.51e-05}  & 1.51e-02 & \first{1.62e-04}  & 2.75e-02 & \first{1.54e-04}  & 4.31e-02 & \first{1.72e-04}\\
 & LS-Chebyshev & 6.32e-09 & \first{1.30e-09}  & \first{6.43e-05} & \first{1.07e-05}  & \first{7.63e-04} & 1.16e-04  & \first{2.72e-03} & 3.57e-04  & \first{8.05e-03} & 7.55e-04  & \first{9.84e-03} & 6.83e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 4.07e+00 & 4.26e-01  & 9.99e+00 & 5.76e-01  & 2.90e+01 & 1.40e+00  & 7.05e+01 & \first{2.61e+00}  & 1.75e+02 & \first{4.24e+00}  & 3.78e+02 & \first{9.44e+00}\\
 & LS-Uniform & 6.62e+05 & 2.77e+04  & 2.28e+02 & 5.88e+00  & 1.19e+02 & 2.99e+00  & 1.84e+02 & 5.00e+00  & 3.37e+02 & 7.03e+00  & 7.70e+02 & 1.33e+01\\
 & LS-Chebyshev & \first{3.25e+00} & \first{2.92e-01}  & \first{9.30e+00} & \first{5.30e-01}  & \first{1.98e+01} & \first{1.33e+00}  & \first{4.26e+01} & 2.71e+00  & \first{1.01e+02} & 5.33e+00  & \first{3.10e+02} & 1.54e+01\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 1.93e-03 & 4.27e-04  & 3.31e-02 & 5.10e-03  & 1.04e-01 & 7.66e-03  & 1.11e-01 & 8.48e-03  & 1.95e-01 & 8.53e-03  & 2.89e-01 & 1.24e-02\\
 & LS-Uniform & 2.27e+02 & 1.11e+01  & 6.14e-01 & 1.82e-02  & 3.52e-01 & 9.70e-03  & 7.12e-01 & 1.01e-02  & 8.09e-01 & 8.80e-03  & 1.08e+00 & 9.96e-03\\
 & LS-Chebyshev & \first{1.19e-03} & \first{2.87e-04}  & \first{1.72e-02} & \first{2.09e-03}  & \first{3.82e-02} & \first{3.73e-03}  & \first{7.31e-02} & \first{4.62e-03}  & \first{9.95e-02} & \first{5.00e-03}  & \first{1.38e-01} & \first{6.03e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 3.65e-06 & 6.94e-07  & 2.11e-06 & 2.89e-07  & 5.75e-04 & 3.13e-05  & 3.08e-05 & 1.64e-06  & 3.06e-04 & 1.70e-05  & 1.22e-03 & 5.36e-05\\
 & LS-Uniform & 1.07e-01 & 4.54e-03  & 3.39e-05 & 9.23e-07  & 8.25e-04 & \first{1.35e-05}  & 5.12e-05 & \first{9.06e-07}  & 5.21e-04 & \first{8.06e-06}  & 1.96e-03 & \first{1.69e-05}\\
 & LS-Chebyshev & \first{3.08e-06} & \first{5.99e-07}  & \first{9.97e-07} & \first{1.49e-07}  & \first{1.92e-04} & 2.86e-05  & \first{1.06e-05} & 1.30e-06  & \first{1.05e-04} & 1.40e-05  & \first{4.64e-04} & 5.06e-05\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 9.21e-07 & 2.39e-07  & 2.24e-06 & 4.56e-07  & 4.65e-06 & 7.53e-07  & 9.92e-06 & 1.21e-06  & 1.53e-05 & 1.84e-06  & 2.80e-05 & 2.59e-06\\
 & LS-Uniform & 5.97e-01 & 2.69e-02  & 6.91e-05 & 1.80e-06  & 1.39e-05 & 4.01e-07  & 1.06e-05 & 2.99e-07  & 1.15e-05 & 2.52e-07  & 1.59e-05 & 2.34e-07\\
 & LS-Chebyshev & \first{8.96e-07} & \first{1.35e-07}  & \first{9.05e-07} & \first{1.43e-07}  & \first{7.41e-07} & \first{1.39e-07}  & \first{7.43e-07} & \first{1.42e-07}  & \first{9.26e-07} & \first{1.49e-07}  & \first{1.12e-06} & \first{1.56e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & 5.70e-13 & 1.95e-13  & 2.01e-05 & 4.99e-06  & 2.29e-03 & 5.81e-04  & 3.98e-02 & 8.11e-03  & 2.67e-01 & 3.63e-02  & 1.26e+00 & 1.05e-01\\
 & LS-Uniform & 7.01e-08 & 3.60e-09  & 2.75e-04 & 7.39e-06  & 6.46e-03 & 1.75e-04  & 2.71e-01 & 3.65e-03  & 1.47e+00 & \first{1.98e-02}  & 8.97e+00 & \first{7.95e-02}\\
 & LS-Chebyshev & \first{5.26e-13} & \first{1.40e-13}  & \first{1.38e-05} & \first{2.08e-06}  & \first{1.06e-03} & \first{1.60e-04}  & \first{2.59e-02} & \first{3.41e-03}  & \first{1.63e-01} & 2.75e-02  & \first{8.34e-01} & 1.35e-01\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & 3.03e-11 & 8.55e-12  & 2.04e-07 & 4.59e-08  & 2.36e-06 & 5.40e-07  & 6.45e-06 & 1.09e-06  & \first{8.00e-06} & 1.14e-06  & \first{2.85e-05} & 1.87e-06\\
 & LS-Uniform & 3.65e-06 & 1.54e-07  & 2.28e-06 & 6.98e-08  & 5.35e-06 & \first{1.28e-07}  & 2.59e-05 & 4.58e-07  & 8.31e-05 & \first{6.08e-07}  & 1.35e-04 & \first{1.14e-06}\\
 & LS-Chebyshev & \first{2.75e-11} & \first{6.14e-12}  & \first{1.50e-07} & \first{2.05e-08}  & \first{1.10e-06} & 1.52e-07  & \first{4.87e-06} & \first{4.37e-07}  & 1.09e-05 & 6.35e-07  & 2.90e-05 & 1.40e-06\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & \first{2.39e-02} & 2.13e-03  & 7.33e-02 & 6.44e-03  & 2.32e-01 & 1.58e-02  & 4.45e-01 & 3.77e-02  & 1.18e+00 & 7.76e-02  & 3.23e+00 & 1.35e-01\\
 & LS-Uniform & 6.36e+03 & 2.86e+02  & 2.31e+00 & 5.32e-02  & 6.19e-01 & 2.10e-02  & 9.51e-01 & 2.92e-02  & 1.10e+00 & 3.85e-02  & 2.14e+00 & \first{6.46e-02}\\
 & LS-Chebyshev & 2.72e-02 & \first{1.68e-03}  & \first{4.65e-02} & \first{4.66e-03}  & \first{1.19e-01} & \first{9.61e-03}  & \first{1.92e-01} & \first{1.79e-02}  & \first{4.85e-01} & \first{3.25e-02}  & \first{9.39e-01} & 7.06e-02\\
\bottomrule
\end{tabular}


==> tables/scale8.tex <==
% Created with Python on 2025-06-22 19:31:18
% ..\results\final_results\low_dim\results_numerical_experiments.csv, scale=8, dims = [2, 3, 4, 5]
\begin{tabular}{ll|rr|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Dim2} & \multicolumn{2}{c}{Dim3} & \multicolumn{2}{c}{Dim4} & \multicolumn{2}{c}{Dim5}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 8.96e-06 & 2.44e-06  & 5.82e-03 & 9.34e-04  & 3.60e-02 & 3.18e-03  & 5.70e-02 & 5.97e-03\\
 & LS-Uniform & 1.93e+00 & 6.95e-02  & 1.42e+00 & 2.36e-02  & 3.80e-01 & 5.27e-03  & 8.27e-01 & 5.01e-03\\
 & LS-Chebyshev & \first{6.78e-06} & \first{1.50e-06}  & \first{3.83e-03} & \first{4.99e-04}  & \first{1.29e-02} & \first{1.29e-03}  & \first{2.88e-02} & \first{2.14e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 1.46e-03 & 8.93e-05  & 1.32e-03 & 6.54e-05  & 1.13e-03 & 5.73e-05  & 8.40e-04 & 4.66e-05\\
 & LS-Uniform & 7.77e+02 & 3.19e+01  & 2.74e-01 & 4.00e-03  & 2.03e-02 & 2.56e-04  & 7.40e-03 & 1.04e-04\\
 & LS-Chebyshev & \first{1.20e-03} & \first{6.72e-05}  & \first{1.04e-03} & \first{6.09e-05}  & \first{8.58e-04} & \first{4.69e-05}  & \first{7.27e-04} & \first{3.74e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & \first{2.77e-13} & 8.54e-14  & 1.35e-05 & 2.06e-06  & 1.60e-03 & 1.37e-04  & 1.65e-02 & 1.01e-03\\
 & LS-Uniform & 7.93e-08 & 2.70e-09  & 6.45e-04 & 1.13e-05  & 1.53e-03 & \first{2.20e-05}  & 1.39e-02 & \first{6.86e-05}\\
 & LS-Chebyshev & 2.79e-13 & \first{5.98e-14}  & \first{5.24e-06} & \first{9.96e-07}  & \first{1.81e-04} & 2.37e-05  & \first{1.25e-03} & 1.15e-04\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 3.57e+00 & 3.28e-01  & 8.40e+00 & 4.81e-01  & 3.14e+01 & \first{1.04e+00}  & 7.93e+01 & \first{1.92e+00}\\
 & LS-Uniform & 1.79e+06 & 6.20e+04  & 1.29e+03 & 2.70e+01  & 5.04e+02 & 5.85e+00  & 3.20e+02 & 4.61e+00\\
 & LS-Chebyshev & \first{2.36e+00} & \first{2.04e-01}  & \first{6.44e+00} & \first{3.77e-01}  & \first{1.92e+01} & 1.07e+00  & \first{4.79e+01} & 2.04e+00\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 7.40e-06 & 1.88e-06  & 7.56e-03 & 8.69e-04  & 3.94e-02 & 3.36e-03  & 4.50e-02 & 3.53e-03\\
 & LS-Uniform & 2.62e+00 & 8.97e-02  & 9.04e-01 & 1.65e-02  & 3.41e-01 & 4.48e-03  & 8.05e-01 & 4.63e-03\\
 & LS-Chebyshev & \first{5.39e-06} & \first{1.22e-06}  & \first{2.88e-03} & \first{3.73e-04}  & \first{1.68e-02} & \first{1.06e-03}  & \first{2.69e-02} & \first{1.46e-03}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 1.36e-07 & 2.22e-08  & 1.44e-07 & 1.55e-08  & 9.34e-05 & 4.02e-06  & 3.21e-06 & 1.30e-07\\
 & LS-Uniform & 3.88e-03 & 1.23e-04  & 1.81e-06 & 4.77e-08  & 1.25e-04 & \first{2.09e-06}  & 4.22e-06 & \first{6.83e-08}\\
 & LS-Chebyshev & \first{9.87e-08} & \first{2.00e-08}  & \first{4.43e-08} & \first{6.60e-09}  & \first{1.68e-05} & 2.98e-06  & \first{1.13e-06} & 1.03e-07\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 1.21e-06 & 2.51e-07  & 2.73e-06 & 4.96e-07  & 5.81e-06 & 9.02e-07  & 1.06e-05 & 1.47e-06\\
 & LS-Uniform & 1.65e+00 & 5.52e-02  & 6.26e-04 & 1.09e-05  & 7.98e-05 & 9.71e-07  & 3.63e-05 & 4.34e-07\\
 & LS-Chebyshev & \first{7.56e-07} & \first{1.28e-07}  & \first{7.14e-07} & \first{1.38e-07}  & \first{7.44e-07} & \first{1.37e-07}  & \first{8.45e-07} & \first{1.43e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & \first{9.44e-15} & \first{2.26e-15}  & 2.82e-07 & 6.29e-08  & 1.65e-04 & 3.36e-05  & 5.71e-03 & 1.11e-03\\
 & LS-Uniform & 7.54e-09 & 2.53e-10  & 4.31e-05 & 7.63e-07  & 8.88e-04 & 1.58e-05  & 3.33e-02 & 3.65e-04\\
 & LS-Chebyshev & 3.43e-14 & 2.88e-15  & \first{1.45e-07} & \first{2.87e-08}  & \first{6.54e-05} & \first{8.09e-06}  & \first{2.31e-03} & \first{2.90e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & \first{7.77e-15} & 2.15e-15  & 5.45e-09 & 9.51e-10  & 2.12e-07 & 3.75e-08  & 8.07e-07 & 1.28e-07\\
 & LS-Uniform & 3.19e-09 & 1.14e-10  & 9.92e-07 & 1.61e-08  & 9.85e-07 & 1.64e-08  & 5.06e-06 & 4.72e-08\\
 & LS-Chebyshev & 1.55e-14 & \first{1.79e-15}  & \first{2.57e-09} & \first{4.36e-10}  & \first{7.08e-08} & \first{9.16e-09}  & \first{3.99e-07} & \first{3.50e-08}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 1.18e-02 & 9.11e-04  & \first{3.25e-02} & 2.47e-03  & 1.24e-01 & 6.54e-03  & 3.11e-01 & 1.70e-02\\
 & LS-Uniform & 5.10e+03 & 1.54e+02  & 1.25e+01 & 2.04e-01  & 2.03e+00 & 2.22e-02  & 1.43e+00 & 1.86e-02\\
 & LS-Chebyshev & \first{1.14e-02} & \first{6.19e-04}  & 3.39e-02 & \first{1.74e-03}  & \first{6.77e-02} & \first{3.92e-03}  & \first{1.58e-01} & \first{7.57e-03}\\
\bottomrule
\end{tabular}


==> tables/scale9.tex <==
% Created with Python on 2025-06-22 19:31:18
% ..\results\final_results\low_dim\results_numerical_experiments.csv, scale=9, dims = [2, 3, 4]
\begin{tabular}{ll|rr|rr|rr|}
 &   \multicolumn{1}{c}{} & \multicolumn{2}{c}{Dim2} & \multicolumn{2}{c}{Dim3} & \multicolumn{2}{c}{Dim4}\\
 &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm max}^{\rm wc}$} & \multicolumn{1}{c}{$e_{\rm mean}^{\rm wc}$}\\
\toprule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Bim. Gauss.}\\$Q=50$}} & Smolyak & 7.95e-09 & 2.19e-09  & 6.64e-04 & 1.12e-04  & 9.18e-03 & 8.39e-04\\
 & LS-Uniform & 3.03e+04 & 5.31e+02  & 4.05e+01 & 4.14e-01  & 1.39e+00 & 7.92e-03\\
 & LS-Chebyshev & \first{7.27e-09} & \first{1.52e-09}  & \first{3.65e-04} & \first{5.14e-05}  & \first{3.03e-03} & \first{2.47e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Cont.}\\$Q=50$}} & Smolyak & 7.65e-04 & 2.95e-05  & 6.66e-04 & 2.43e-05  & 6.76e-04 & 1.81e-05\\
 & LS-Uniform & 8.46e+08 & 1.50e+07  & 3.04e+01 & 3.14e-01  & 2.02e-01 & 1.17e-03\\
 & LS-Chebyshev & \first{6.47e-04} & \first{2.71e-05}  & \first{5.69e-04} & \first{2.19e-05}  & \first{4.37e-04} & \first{1.74e-05}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Corner Peak}\\$Q=50$}} & Smolyak & \first{6.99e-15} & \first{9.35e-16}  & 3.16e-07 & 4.17e-08  & 3.10e-04 & 2.20e-05\\
 & LS-Uniform & 1.66e-02 & 2.92e-04  & 5.31e-03 & 5.72e-05  & 3.41e-03 & 2.36e-05\\
 & LS-Chebyshev & 1.39e-14 & 1.17e-15  & \first{1.16e-07} & \first{2.05e-08}  & \first{3.76e-05} & \first{4.59e-06}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Discont.}\\$Q=50$}} & Smolyak & 4.70e+00 & 2.16e-01  & 1.07e+01 & 3.28e-01  & 3.13e+01 & 7.74e-01\\
 & LS-Uniform & 6.27e+12 & 1.10e+11  & 4.47e+05 & 4.45e+03  & 1.13e+04 & 6.19e+01\\
 & LS-Chebyshev & \first{2.92e+00} & \first{1.46e-01}  & \first{6.29e+00} & \first{2.59e-01}  & \first{1.81e+01} & \first{7.73e-01}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Gauss.}\\$Q=50$}} & Smolyak & 6.31e-09 & 1.51e-09  & 9.87e-04 & 1.01e-04  & 9.55e-03 & 9.78e-04\\
 & LS-Uniform & 1.88e+04 & 3.30e+02  & 5.56e+01 & 5.23e-01  & 1.31e+00 & 7.83e-03\\
 & LS-Chebyshev & \first{5.51e-09} & \first{1.08e-09}  & \first{3.26e-04} & \first{4.46e-05}  & \first{5.26e-03} & \first{2.87e-04}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Geo. Mean}\\$Q=50$}} & Smolyak & 2.19e-09 & 3.61e-10  & 6.94e-09 & 7.03e-10  & 1.07e-05 & 4.43e-07\\
 & LS-Uniform & 2.26e+02 & 3.95e+00  & 6.44e-05 & 6.38e-07  & 1.18e-04 & 9.63e-07\\
 & LS-Chebyshev & \first{2.06e-09} & \first{3.03e-10}  & \first{2.38e-09} & \first{3.29e-10}  & \first{3.13e-06} & \first{2.92e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{NOISE}\\$Q=50$}} & Smolyak & 1.25e-06 & 2.57e-07  & 3.06e-06 & 5.57e-07  & 6.78e-06 & 1.02e-06\\
 & LS-Uniform & 1.05e+07 & 1.84e+05  & 2.51e-01 & 2.57e-03  & 2.00e-03 & 1.32e-05\\
 & LS-Chebyshev & \first{7.61e-07} & \first{1.27e-07}  & \first{7.36e-07} & \first{1.31e-07}  & \first{7.95e-07} & \first{1.37e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Osci.}\\$Q=50$}} & Smolyak & \first{1.97e-14} & 3.65e-15  & 7.89e-11 & 1.71e-11  & 6.86e-06 & 1.18e-06\\
 & LS-Uniform & 5.83e-02 & 1.02e-03  & 4.07e-06 & 3.67e-08  & 4.14e-04 & 3.25e-06\\
 & LS-Chebyshev & 2.81e-14 & \first{2.41e-15}  & \first{4.98e-11} & \first{7.59e-12}  & \first{2.32e-06} & \first{2.84e-07}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Prod. Peak}\\$Q=50$}} & Smolyak & \first{1.80e-14} & 3.63e-15  & 4.20e-11 & 7.27e-12  & 1.43e-08 & 1.83e-09\\
 & LS-Uniform & 2.16e-02 & 3.83e-04  & 1.46e-06 & 1.47e-08  & 8.28e-07 & 5.47e-09\\
 & LS-Chebyshev & 2.56e-14 & \first{1.73e-15}  & \first{2.47e-11} & \first{3.23e-12}  & \first{4.38e-09} & \first{4.44e-10}\\
\midrule
\multirow{3}{*}{\thead[l]{\tiny\textbf{Ridge Prod.}\\$Q=50$}} & Smolyak & 7.14e-03 & 3.33e-04  & 3.06e-02 & 9.64e-04  & 4.96e-02 & 2.72e-03\\
 & LS-Uniform & 1.57e+10 & 2.75e+08  & 2.03e+03 & 1.87e+01  & 1.28e+01 & 8.16e-02\\
 & LS-Chebyshev & \first{5.41e-03} & \first{2.38e-04}  & \first{1.99e-02} & \first{6.82e-04}  & \first{4.23e-02} & \first{1.60e-03}\\
\bottomrule
\end{tabular}

